Identifying Best Interventions through Online Importance Sampling

Motivated by applications in computational advertising and systems biology, we consider the problem of identifying the best out of several possible soft interventions at a source node $V$ in an acyclic causal directed graph, to maximize the expected value of a target node $Y$ (located downstream of $V$). Our setting imposes a fixed total budget for sampling under various interventions, along with cost constraints on different types of interventions. We pose this as a best arm identification bandit problem with $K$ arms where each arm is a soft intervention at $V,$ and leverage the information leakage among the arms to provide the first gap dependent error and simple regret bounds for this problem. Our results are a significant improvement over the traditional best arm identification results. We empirically show that our algorithms outperform the state of the art in the Flow Cytometry data-set, and also apply our algorithm for model interpretation of the Inception-v3 deep net that classifies images.

==> Introductionv10.tex <==
\label{sec:intro}


Causal graphs \cite{pearl2009causality} are useful for representing
causal relationships among interacting variables in large systems
\cite{bottou2013counterfactual}. Over the last few decades, causal
models have found use in computational
advertising~\cite{bottou2013counterfactual}, biological
systems~\cite{meinshausen2016methods},
sociology~\cite{blalock1985causal},
agriculture~\cite{splawa1990application} and epidemiology
\cite{joffe2012causal}.
%
There are two important questions commonly studied with causal graphs: {\em
(i)} How to learn a directed causal graph that encodes that pattern of
interaction among components in a system (\textit{casual structure
learning})?~\cite{pearl2009causality}~, and {\em (ii)} Using
previously acquired (partial) knowledge about the causal graph
structure, how to estimate and/or to optimize the effect of a new
\textit{intervention} on other variables (\textit{optimization})~\cite{bottou2013counterfactual,joffe2012causal,kemmeren2014large,bonneau2007predictive,krouk2013gene}?
Here, an \textit{intervention} is a forcible change to the value of one of
the variables in a system. The change either alters the relationship
between the parental causes and the variable, or decouples it from the
parental causes entirely. In this work, our focus is on optimizing over a set of given interventions.

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{Bottou_example.pdf}
	\caption{ \small Computational advertising example borrowed from
		\cite{bottou2013counterfactual}. Various observable and hidden variables are shown. The topology of the causal graph is known;
		however the strengths of most interactions are unknown. A click-rate
		scoring algorithm predicts future user click-rates from users' search
		queries and the set of ads relevant to the user query chosen
		from an ad inventory. The algorithm's output determines the ads
		displayed (as well as the display style), and through a complex causal
		graph, finally determines actual revenue. The part of the network in
		bold -- distribution of user queries and matching ad keywords is known
		(including strengths), and the input output characteristics of several
		candidate (randomized) click-rate scoring algorithms are known. The
		objective is to choose the best algorithm that maximizes the revenue
		(target in bold red).\normalsize} \label{fig:Bottou}
\end{figure}

 
 %
An illustrative example includes online advertising
\cite{bottou2013counterfactual}, where there is a collection of
click-through rate scoring algorithms that provide an estimate of the
probability that a user clicks on an ad displayed at a specific
position. The interventions occur through the choice of click-through
rate scoring algorithm; the algorithm choice directly impacts ad
placement and pricing, and through a complex network of interactions,
affects the revenue generated through advertisements. The revenue
%(downstream node in a causal
%graph)
 is used to determine the best scoring algorithm (optimize for the
best intervention); see Figure~\ref{fig:Bottou}. Another example is in
biological gene-regulatory networks \cite{bonneau2007predictive},
where a large number of genomes interact amongst each other and also
interact with environmental factors. The objective here is to
understand the best perturbation of some genomes in terms of its
effect on the expression of another subset of genomes (target) in
cellular systems. %(the downstream node).

%\begin{figure*}
%	\centering
%	\subfloat[][]{\includegraphics[width = 0.3\linewidth]{Bottou_example.pdf}\label{fig:Bottou}} \hfill
%	\subfloat[][]{\includegraphics[width = 0.3\linewidth]{./figs/illustrate.pdf}\label{fig:illustrate}} \hfill
%	%\subfloat[][]{\includegraphics[width = 0.3\linewidth]{./figs/illustrate2.pdf}\label{fig:illustrate2}}
%	\caption{{\small (a) Example of computational advertising borrowed from
%			\cite{bottou2013counterfactual}. Various observable variables and
%			hidden variables are shown. The topology of the causal graph is known;
%			however the strengths of most interactions are unknown. A click-rate
%			scoring algorithm predicts future user click-rates from users' search
%			queries and the set of ads relevant to the user query chosen
%			from an ad inventory. The algorithm's output determines the ads
%			displayed (as well as the display style), and through a complex causal
%			graph, finally determines actual revenue. The part of the network in
%			bold -- distribution of user queries and matching ad keywords is known
%			(including strengths), and the input output characteristics of several
%			candidate (randomized) click-rate scoring algorithms are known. The
%			objective is to choose the best algorithm that maximizes the revenue
%			(target in bold red). (b) Illustration of our causal setting. The soft interventions modify $\mathrm{P}(V | pa(V)$. The various conditionals and the marginal of $pa(V)$ is assumed to be known from prior data. The \textit{target} variable $Y$ lies further downstream in the unknown portions of the causal graph. }}%(c) Illustration of a more general causal setting where the arms are induced distributions on a directed cut separating the sources of intervention and the target variable $Y$. } }
%	\label{fig:allthree}
%\end{figure*}

This paper focuses on the following setting: We are given apriori
knowledge about the structure and strength of interactions over a
small part of the causal graph.  In addition, there is freedom to
intervene (from a set of allowable interventions) at a certain node in
the known part of the graph, and collect data under the chosen
intervention; further we can alter the interventions over time and
observe the corresponding effects. Given a set of potential
interventions to optimize over, the key question of interest is: How
to choose the best sequence of $T$ allowable interventions in order to
discover which intervention maximizes the expectation of the
downstream target node.

Determining the best intervention in the above setting can be cast as
a best arm identification bandit problem, as noted in
\cite{lattimore2016causal}. The possible interventions to optimize over are the arms of the bandit, while the sample value of the \textit{target} node under an intervention is the \textit{reward}.

 More formally, suppose that $V$ is a node in a causal graph
$\mathcal{G}(\mathcal{V}, \mathcal{E})$ (as shown in Fig.~\ref{fig:illustrate}), with the parents of $V$
denoted by $pa(V).$ In Fig.~\ref{fig:Bottou}, $V$ corresponds to the \textit{click-through rate} and its parents are \textit{user-query} and \textit{ads-chosen}. This essentially means that $V$ is causally
determined by a function of $pa(V)$ and some exogenous random
noise. This dependence is characterized by the conditional
$\mathrm{P}(V | pa(V))$. Then a (soft) intervention mathematically
corresponds to changing this conditional probability distribution
i.e. probabilistically forcing $V$ to certain states given its
parents\footnote{These changes through the conditional distributions
	are also called \textit{soft
		interventions}~\cite{pearl2009causality}.Note that our algorithm is
	also applicable to the more general case when the set of interventions
	to optimize over is much larger than the set of interventions
	available to sample from. This 'transfer of knowledge' to an unseen
	but informationally related situation is also an important
	motivation. Formally, it is possible to choose the best soft intervention in $\{0,1 \cdots , K-1 \}$ by only observing samples under interventions in the set $\mathcal{S}$, where $\mathcal{S} \subset [K]$.}. In the computational advertising example, the interventions correspond to changing the click through rate scoring algorithm (i.e $\mathrm{P}(click~through~rate \vert ads~chosen,user~query)$, whose input-output characteristics are well-studied. Further, suppose that the effect of an intervention is
observed at a node $Y$ which is downstream of $V$ in the topological
order (w.r.t $\mathcal{G}$) -refer to Fig.~\ref{fig:illustrate}.  Then, our key question is stated as
follows: \textit{Given a collection of interventions $\{\mathrm{P}_0
	(V| pa(V)),\ldots \mathrm{P}_{K-1}(V |
	pa(V))\},$ find the best intervention among these $K$ possibilites
	that maximizes $E[Y]$ under a fixed budget of $T$ (intervention,
	observation) pairs.}

%The key difference from the classical best arm setting is that there is \textit{information leakage} among the arms through the shared causal graph. In the next section we list our main contributions, where we elaborate on the advantages of leveraging this information leakage. 

%A key property we use is that these interventions are correlated,
%i.e. there is information leakage that informs us about how good one
%arm is by observing the performance of another. Classical best arm
%identification~\cite{audibert2010best} does not model such information
%leakage among arms; our goal is to extend the theory for this regime
%and quantify the benefits of information leakage. Information leakage
%effects are natural for various problems. For example, Bottou et
%al.~\cite{bottou2013counterfactual} show that the performance of
%untested ad scoring algorithms can be predicted from different scoring
%models.  Recent work \cite{lattimore2016causal} has leveraged this
%information leakage and developed algorithms for approximating the
%best possible sequence of interventions for discovering the optimal
%policy.

\begin{figure}
	\centering
	\includegraphics[width=0.6\linewidth]{./figs/illustrate.pdf}
	\caption{\small Illustration of our setting. The soft interventions modify $\mathrm{P}(V | pa(V)$. The various conditionals and the marginal of $pa(V)$ is assumed to be known from prior data. The \textit{target} variable $Y$ lies further downstream in the unknown portions of the causal graph. \normalsize} \label{fig:illustrate}
	%\setlength{\belowcaptionskip}{-30pt}
\end{figure}


%Our main result in this paper is a \textit{successive rejects bandit
%algorithm} for selecting the sequence of interventions, to determine
%the best one that has the maximum desired effect on a downstream
%node. Our algorithm uses past observations along with information
%leakage across interventions to sequentially eliminate sub-optimal
%interventions. We provide the first \textit{gap-dependent} simple
%regret and error bounds for this problem. Further, our solution
%explicitly accounts for possible cost constraints on using
%interventions. As a special case, we recover the gap-independent
%result in \cite{lattimore2016causal} (orderwise).







 \subsection{Main Contributions}
 
 Our main contributions are the following:


{\noindent \bf (Gap Dependent Error Guarantees under budget constraints)}
 We derive the first \textit{gap dependent} (gaps between the
 expectations of the target under different interventions unknown to
 our algorithm) bounds on the probability of misidentification in
 terms of the number of samples $T$, cost budget $B$ on the relative
 fraction of times various arms are sampled and the divergences
 between different conditional probability distributions underlying
 the changes. 
 
 A fundamental difference from the classical best arm setting~\cite{audibert2010best} is the \textit{information leakage} among the arms i.e sampling from one arm can inform us about the mean of other arms because of  the shared causal graph. We show that leveraging this information leakage yields significant improvement both in theory and practice.
 
 Our result generalizes that of \cite{audibert2010best}
 which derives that the number of samples needed is (upto poly
 log factors) $\max_i (i/\Delta_{(i)}^2)$ where $\Delta_{(i)}$ is the
 $i$-th smallest gap from the optimal (for the classic best arm
 identification problem with no information leakage). We obtain a similar result (upto poly log factors) where the the
factor $i$ is replaced by the 'effective variance' of the estimator
for arm $(i)$, i.e. we obtain (with informal notation) $\max_i
\sigma_i^2/\Delta_{(i)}^2$. $\sigma_i$ can be much smaller than $\sqrt{i}$ (the corresponding term in the results of~\cite{audibert2010best}). Our theoretical guarantees quantify the improvement obtained by leveraging information leakage, which have been empirically observed in~\cite{bottou2013counterfactual}. We discuss in more detail in Sections~\ref{sec:guarantee} and~\ref{sec:detcontri} (in the appendix), about how these guarantees can be exponentially better than the classical ones.
We derive simple regret (refer to Section~\ref{sec:def}) bounds analogous to
 the gap dependent bounds on the probability of misidentification.
 
 We provide a novel analysis of \textit{clipped importance sampling} estimators, where pairwise $f$-divergences between the distributions
 $\{\mathrm{P}_{k}(V \vert pa(V))\}$, for a carefully chosen function $f(.)$
 (see Section~\ref{sec:divergence}) act as the `effective variance'
 terms in the analysis for the estimators (similar to Bernstein's bound~\cite{bennett1962probability}).
 
 {\noindent \bf (Successive Rejects Algorithm leveraging Information
Leakage)} We provide an efficient \textit{successive rejects} multi-phase
algorithm that achieves these guarantees. The algorithm uses
\textit{clipped importance sampling} where the clipper level is set adaptively in each phase. Our procedure yields a major improvement over the algorithm in~\cite{lattimore2016causal} (both in theoretical guarantees and in
practice), which sets the clippers and allocates samples in a static
manner. Please refer to Section~\ref{sec:detcontri} for more details.


{\noindent \bf (Extensive Empirical Validation)} We demonstrate that our algorithm outperforms the prior works~\cite{lattimore2016causal,audibert2010best} on the Flow Cytometry data-set~\cite{sachs2005causal} (in Section~\ref{sec:cytometry}). We also exhibit an innovative application of our algorithm in the context of model interpretation of the Inception Deep Network~\cite{szegedy2015going} for classification of images (refer to Section~\ref{sec:inception}).

\begin{remark}
The techniques in this paper can be directly applied to more general settings like (i) the intervention source ($V$) can be a collection of nodes ($\mathcal{V}$) and the changes affect the distribution $P(\mathcal{V} \vert pa(\mathcal{V}))$, where  $pa(\mathcal{V})$ is the union of all the parents; (ii) the importance sampling can be applied at a directed cut separating the sources and the targets, provided the effect of the interventions, on the nodes forming the cut can be estimated. Moreover, our techniques can be applied without the complete knowledge of the source distributions. We explain the variations in more detail in Section~\ref{sec:variation} in the appendix.
\end{remark} 

 
%  \begin{figure}
%\centering
%\includegraphics[width=\linewidth]{Bottou_example.pdf}
%\caption{{\small Example of computational advertising borrowed from
%\cite{bottou2013counterfactual}. Various observable variables and
%hidden variables are shown. The topology of the causal graph is known;
%however the strengths of most interactions are unknown. A click-rate
%scoring algorithm predicts future user click-rates from users' search
%queries and the set of ads relevant to the user query chosen
%from an ad inventory. The algorithm's output determines the ads
%displayed (as well as the display style), and through a complex causal
%graph, finally determines actual revenue. The part of the network in
%bold -- distribution of user queries and matching ad keywords is known
%(including strengths), and the input output characteristics of several
%candidate (randomized) click-rate scoring algorithms are known. The
%objective is to choose the best algorithm that maximizes the revenue
%(target in bold red).}} \label{fig:Bottou}
%\end{figure}
 
% \subsection{An Example in Computational Advertising
%~\cite{bottou2013counterfactual}} 
%
%To illustrate our model, we revisit the computational advertisement example~\cite{bottou2013counterfactual} in more detail. In
%this example, the causal graph among various observable entities in a
%computational advertising system is known (however, the strengths of
%various interactions are not known). The corresponding causal graph is
%illustrated in Figure~\ref{fig:Bottou} (borrowed
%from~\cite{bottou2013counterfactual}).
%
%The overall goal of the system is to maximize the expected value of the \textit{target} variable \textit{revenue} (this is the target $Y$ in our causal system). In the advertisement system, a click-rate scoring algorithm is employed to predict future user
%\textit{click-through rate score} (an intermediate variable in the causal graph). This algorithm takes as input, the \textit{user query} word and the
%set of ad keywords (\textit{ads chosen}) that match the query word, and outputs a click-through rate
%score. This score in-turn influences the pricing and ad placement
%strategies, which in turn affects the revenue (see
%Figure~\ref{fig:Bottou}). In this example we are concerned with choosing the best scoring algorithm, that influences the causal relation between the predicted click-through rate score (equivalent to $V$ in our causal system) and its parents user query word and ad keywords in the causal graph (equivalent to $pa(V)$ in our causal system). 
%There are many candidate randomized scoring algorithms, and the input -
%output characteristics of each one are well studied. This means that
%for each of these algorithms, the conditionals
%$\mathrm{P}_k(\mathrm{Click-through~rate~score} |
%\mathrm{User~Query},\mathrm{Ads~chosen})$ are known. In the causal
%model, this is equivalent to knowing $\mathrm{P}_k (V | pa (V) ),$ where $V$ is
%identified with $\mathrm{click-through~rate~score}$. The task then is to find
%the best algorithm (arms or mechanisms determining $\mathrm{P}(V | pa (V) )$) that maximizes the revenue (target $Y$). This has a natural interpretation as a \textit{best arm identification} problem in bandits~\cite{audibert2010best}. Each of the mechanisms influencing the conditional $\mathrm{P}(V | pa(V))$ (eg. click rate prediction algorithms) can be thought of as the arms of the bandit. The expectation of the target $Y$ under arm/mechanism $i$ (revenue when algorithm $i$ is deployed) is considered to be the reward from arm $i$. The task is to identify the best arm with maximum certainty given a sample budget of $T$ interventions. The crucial difference from the classic best arm setting is that there is information leakage among the arms of the bandit through the shared causal graph.
%
%It should be noted that the level of difficulty to obtain samples from various algorithms can be very different in practice. For instance some of the algorithms above, may be default and easy to engineer and deploy, while others require a lot of engineering effort. Therefore, it is natural to expect a lot of samples from the default algorithms as compared to the more difficult ones. We model this is into our setting through a budget on the relative fractions of samples from different interventions (in addition to the total sample budget $T$). It is assumed that the cost associated with mechanism $i$ is $c_i$ ($c_i$ is high for an algorithm that is difficult to implement). Then we require that $\sum_{i \in [K]} c_i\nu_i \leq B$, where $\nu_i$ is the fraction of times arm $i$ is sampled and $B$ is the total fractional budget constraint.  Thus, it is evident that our causal setting is adequate in handling all the design issues in the optimization problem in the above example. In fact, it can be applied to a wide range of similar best arm identification settings with an underlying causal graph. 
 
 \subsection{Related Work}
    The problem lies at the intersection of causal inference and best
arm identification in bandits, similar in spirit
to~\cite{lattimore2016causal}. %We will review some of the relevant work in these areas and finally distinguish ourcontribution from that of \cite{lattimore2016causal}. 

The classical \textit{best arm identification} problem has been studied extensively in the bandit literature, both in the fixed confidence regime~\cite{gabillon2012best} and in the fixed budget setting~\cite{audibert2010best,chen2015optimal,jamieson2014lil,carpentier2016tight}. It was shown recently in
\cite{carpentier2016tight} that the results of \cite{audibert2010best}
are optimal.  The key difference from our work is that, in these
models, there is no information leakage among the arms.

There has been a lot of work \cite{mooij2016distinguishing,Hyttinen2013,Eberhardt2008X,Hauser2012b,Spirtes2001,Pearl2009}
on \textit{learning casual models} from data and/or experiments and using it to
\textit{estimate causal strength} questions of the \textit{counterfactual} nature. One
notable work that partially inspired our work is
\cite{bottou2013counterfactual} where the causal graph underlying a
computational advertising system (like in Bing, Google etc.) is known
and the primary interest is to find out how a change in the system
would affect some other variable.
  
At the intersection of \textit{causality and bandits}, \cite{lattimore2016causal} is perhaps most
relevant to our setting. The authors study the problem of identifying the best hard interventions on multiple variables (among many), provided the distribution of the parents of the target is known under those interventions. Simple regret bound of order $O(1/\sqrt{T})$ was derived. We assume soft interventions that affect the mechanism between
a 'source' node and its parents far away from the target (similar to
the case of computational advertising considered in
\cite{bottou2013counterfactual}). Further, we derive the first
\textit{gap dependent} bounds (that can be exponentially small in $T$),
generalizing the results of \cite{audibert2010best}. Our formulation can handle general budget constraints on the bandit arms and also recover the problem independent bounds of~\cite{lattimore2016causal} (orderwise).

In the context of machine learning, \textit{importance sampling} has been mostly used to recondition input data to adhere to conditions imposed by learning algorithms~\cite{sugiyama2007covariate,li2011unbiased,zhang2014stochastic}.


 
 
 




==> Introductionv11.tex <==
\label{sec:intro}


Causal graphs \cite{pearl2009causality} are useful for representing
causal relationships among interacting variables in large systems
\cite{bottou2013counterfactual}. Over the last few decades, causal
models have found use in computational
advertising~\cite{bottou2013counterfactual}, biological
systems~\cite{meinshausen2016methods},
sociology~\cite{blalock1985causal},
agriculture~\cite{splawa1990application} and epidemiology
\cite{joffe2012causal}.
%
There are two important questions commonly studied with causal graphs: {\em
(i)} How to learn a directed causal graph that encodes that pattern of
interaction among components in a system (\textit{casual structure
learning})?~\cite{pearl2009causality}~, and {\em (ii)} Using
previously acquired (partial) knowledge about the causal graph
structure, how to estimate and/or to optimize the effect of a new
\textit{intervention} on other variables (\textit{optimization})~\cite{bottou2013counterfactual,joffe2012causal,kemmeren2014large,bonneau2007predictive,krouk2013gene}?
Here, an \textit{intervention} is a forcible change to the value of one of
the variables in a system. The change either alters the relationship
between the parental causes and the variable, or decouples it from the
parental causes entirely. In this work, our focus is on optimizing over a set of given interventions.

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{Bottou_example.pdf}
	\caption{ \small Computational advertising example borrowed from
		\cite{bottou2013counterfactual}. Various observable and hidden variables are shown. The topology of the causal graph is known;
		however the strengths of most interactions are unknown. A click-rate
		scoring algorithm predicts future user click-rates from users' search
		queries and the set of ads relevant to the user query chosen
		from an ad inventory. The algorithm's output determines the ads
		displayed (as well as the display style), and through a complex causal
		graph, finally determines actual revenue. The part of the network in
		bold -- distribution of user queries and matching ad keywords is known
		(including strengths), and the input output characteristics of several
		candidate (randomized) click-rate scoring algorithms are known. The
		objective is to choose the best algorithm that maximizes the revenue
		(target in bold red).\normalsize} \label{fig:Bottou}
\end{figure}

 
 %
An illustrative example includes online advertising
\cite{bottou2013counterfactual}, where there is a collection of
click-through rate scoring algorithms that provide an estimate of the
probability that a user clicks on an ad displayed at a specific
position. The interventions occur through the choice of click-through
rate scoring algorithm; the algorithm choice directly impacts ad
placement and pricing, and through a complex network of interactions,
affects the revenue generated through advertisements. The revenue
%(downstream node in a causal
%graph)
 is used to determine the best scoring algorithm (optimize for the
best intervention); see Figure~\ref{fig:Bottou}. Another example is in
biological gene-regulatory networks \cite{bonneau2007predictive},
where a large number of genomes interact amongst each other and also
interact with environmental factors. The objective here is to
understand the best perturbation of some genomes in terms of its
effect on the expression of another subset of genomes (target) in
cellular systems. %(the downstream node).

%\begin{figure*}
%	\centering
%	\subfloat[][]{\includegraphics[width = 0.3\linewidth]{Bottou_example.pdf}\label{fig:Bottou}} \hfill
%	\subfloat[][]{\includegraphics[width = 0.3\linewidth]{./figs/illustrate.pdf}\label{fig:illustrate}} \hfill
%	%\subfloat[][]{\includegraphics[width = 0.3\linewidth]{./figs/illustrate2.pdf}\label{fig:illustrate2}}
%	\caption{{\small (a) Example of computational advertising borrowed from
%			\cite{bottou2013counterfactual}. Various observable variables and
%			hidden variables are shown. The topology of the causal graph is known;
%			however the strengths of most interactions are unknown. A click-rate
%			scoring algorithm predicts future user click-rates from users' search
%			queries and the set of ads relevant to the user query chosen
%			from an ad inventory. The algorithm's output determines the ads
%			displayed (as well as the display style), and through a complex causal
%			graph, finally determines actual revenue. The part of the network in
%			bold -- distribution of user queries and matching ad keywords is known
%			(including strengths), and the input output characteristics of several
%			candidate (randomized) click-rate scoring algorithms are known. The
%			objective is to choose the best algorithm that maximizes the revenue
%			(target in bold red). (b) Illustration of our causal setting. The soft interventions modify $\mathrm{P}(V | pa(V)$. The various conditionals and the marginal of $pa(V)$ is assumed to be known from prior data. The \textit{target} variable $Y$ lies further downstream in the unknown portions of the causal graph. }}%(c) Illustration of a more general causal setting where the arms are induced distributions on a directed cut separating the sources of intervention and the target variable $Y$. } }
%	\label{fig:allthree}
%\end{figure*}

This paper focuses on the following setting: We are given apriori
knowledge about the structure and strength of interactions over a
small part of the causal graph.  In addition, there is freedom to
intervene (from a set of allowable interventions) at a certain node in
the known part of the graph, and collect data under the chosen
intervention; further we can alter the interventions over time and
observe the corresponding effects. Given a set of potential
interventions to optimize over, the key question of interest is: How
to choose the best sequence of $T$ allowable interventions in order to
discover which intervention maximizes the expectation of the
downstream target node.

Determining the best intervention in the above setting can be cast as
a best arm identification bandit problem, as noted in
\cite{lattimore2016causal}. The possible interventions to optimize over are the arms of the bandit, while the sample value of the \textit{target} node under an intervention is the \textit{reward}.

 More formally, suppose that $V$ is a node in a causal graph
$\mathcal{G}(\mathcal{V}, \mathcal{E})$ (as shown in Fig.~\ref{fig:illustrate}), with the parents of $V$
denoted by $pa(V).$ In Fig.~\ref{fig:Bottou}, $V$ corresponds to the \textit{click-through rate} and its parents are \textit{user-query} and \textit{ads-chosen}. This essentially means that $V$ is causally
determined by a function of $pa(V)$ and some exogenous random
noise. This dependence is characterized by the conditional
$\mathrm{P}(V | pa(V))$. Then a (soft) intervention mathematically
corresponds to changing this conditional probability distribution
i.e. probabilistically forcing $V$ to certain states given its
parents\footnote{These changes through the conditional distributions
	are also called \textit{soft
		interventions}~\cite{pearl2009causality}.Note that our algorithm is
	also applicable to the more general case when the set of interventions
	to optimize over is much larger than the set of interventions
	available to sample from. This 'transfer of knowledge' to an unseen
	but informationally related situation is also an important
	motivation. Formally, it is possible to choose the best soft intervention in $\{0,1 \cdots , K-1 \}$ by only observing samples under interventions in the set $\mathcal{S}$, where $\mathcal{S} \subset [K]$.}. In the computational advertising example, the interventions correspond to changing the click through rate scoring algorithm (i.e $\mathrm{P}(click~through~rate \vert ads~chosen,user~query)$, whose input-output characteristics are well-studied. Further, suppose that the effect of an intervention is
observed at a node $Y$ which is downstream of $V$ in the topological
order (w.r.t $\mathcal{G}$) -refer to Fig.~\ref{fig:illustrate}.  Then, our key question is stated as
follows: \textit{Given a collection of interventions $\{\mathrm{P}_0
	(V| pa(V)),\ldots \mathrm{P}_{K-1}(V |
	pa(V))\},$ find the best intervention among these $K$ possibilites
	that maximizes $E[Y]$ under a fixed budget of $T$ (intervention,
	observation) pairs.}

%The key difference from the classical best arm setting is that there is \textit{information leakage} among the arms through the shared causal graph. In the next section we list our main contributions, where we elaborate on the advantages of leveraging this information leakage. 

%A key property we use is that these interventions are correlated,
%i.e. there is information leakage that informs us about how good one
%arm is by observing the performance of another. Classical best arm
%identification~\cite{audibert2010best} does not model such information
%leakage among arms; our goal is to extend the theory for this regime
%and quantify the benefits of information leakage. Information leakage
%effects are natural for various problems. For example, Bottou et
%al.~\cite{bottou2013counterfactual} show that the performance of
%untested ad scoring algorithms can be predicted from different scoring
%models.  Recent work \cite{lattimore2016causal} has leveraged this
%information leakage and developed algorithms for approximating the
%best possible sequence of interventions for discovering the optimal
%policy.

\begin{figure}
	\centering
	\includegraphics[width=0.6\linewidth]{./figs/illustrate.pdf}
	\caption{\small Illustration of our setting. The soft interventions modify $\mathrm{P}(V | pa(V)$. The various conditionals and the marginal of $pa(V)$ is assumed to be known from prior data. The \textit{target} variable $Y$ lies further downstream in the unknown portions of the causal graph. \normalsize} \label{fig:illustrate}
	%\setlength{\belowcaptionskip}{-30pt}
\end{figure}


%Our main result in this paper is a \textit{successive rejects bandit
%algorithm} for selecting the sequence of interventions, to determine
%the best one that has the maximum desired effect on a downstream
%node. Our algorithm uses past observations along with information
%leakage across interventions to sequentially eliminate sub-optimal
%interventions. We provide the first \textit{gap-dependent} simple
%regret and error bounds for this problem. Further, our solution
%explicitly accounts for possible cost constraints on using
%interventions. As a special case, we recover the gap-independent
%result in \cite{lattimore2016causal} (orderwise).







 \subsection{Main Contributions}
 
 Our main contributions are the following:
 
  {\noindent \bf (Successive Rejects Algorithm)} We provide an efficient \textit{successive rejects} multi-phase
 algorithm. The algorithm uses
 \textit{clipped importance sampling}. The clipper level is set \textit{adaptively} in each phase in order to trade-off \textit{bias and variance}. Our procedure yields a major improvement over the algorithm in~\cite{lattimore2016causal} (both in theoretical guarantees and in
 practice), which sets the clippers and allocates samples in a static
 manner. Please refer to Section~\ref{sec:detcontri} for more details.


{\noindent \bf (Gap Dependent Error Guarantees under Budget Constraints)}
Audibert et al. derive \textit{gap} dependent bounds for the classic best arm identification problem~\cite{audibert2010best}. It has been shown that the number of samples needed is (upto poly
log factors) $\max_i (i/\Delta_{(i)}^2)$ where $\Delta_{(i)}$ is the
$i$-th smallest \textit{gap} from the optimal (in terms expected reward of the arms).

A fundamental difference from the classical best arm setting~\cite{audibert2010best} is the \textit{information leakage} among the arms i.e sampling from one arm can inform us about the expected value of other arms because of  the shared causal graph. We show that leveraging this information leakage yields significant improvement both in theory and practice. We derive the first \textit{gap dependent} (gaps between the
 expectations of the target under different interventions unknown to
 our algorithm) bounds on the probability of error in
 terms of the number of samples $T$, cost budget $B$ on the relative
 fraction of times various arms are sampled and the divergences between soft intervention distributions of the arms.
 
In our result (upto poly log factors) the factor $i$ is replaced by the 'effective variance' of the estimator
for arm $(i)$, i.e. we obtain (with informal notation) $\max_i
\sigma_i^2/\Delta_{(i)}^2$. $\sigma_i$ can be much smaller than $\sqrt{i}$ (the corresponding term in the results of~\cite{audibert2010best}). Our theoretical guarantees quantify the improvement obtained by leveraging information leakage, which have been empirically observed in~\cite{bottou2013counterfactual}. We discuss in more detail in Sections~\ref{sec:guarantee} and~\ref{sec:appen_compare} (in the appendix), about how these guarantees can be exponentially better than the classical ones.
We derive simple regret (refer to Section~\ref{sec:def}) bounds analogous to
 the gap dependent error bounds.
 
 
% 
% A fundamental difference from the classical best arm setting~\cite{audibert2010best} is the \textit{information leakage} among the arms i.e sampling from one arm can inform us about the expected value of other arms because of  the shared causal graph. We show that leveraging this information leakage yields significant improvement both in theory and practice.
% 
% Our result generalizes that of \cite{audibert2010best} (the classic best arm
% identification problem)
% which derives that the number of samples needed is (upto poly
% log factors) $\max_i (i/\Delta_{(i)}^2)$ where $\Delta_{(i)}$ is the
% $i$-th smallest gap from the optimal . We obtain a similar result (upto poly log factors) where the the
%factor $i$ is replaced by the 'effective variance' of the estimator
%for arm $(i)$, i.e. we obtain (with informal notation) $\max_i
%\sigma_i^2/\Delta_{(i)}^2$. $\sigma_i$ can be much smaller than $\sqrt{i}$ (the corresponding term in the results of~\cite{audibert2010best}). Our theoretical guarantees quantify the improvement obtained by leveraging information leakage, which have been empirically observed in~\cite{bottou2013counterfactual}. We discuss in more detail in Sections~\ref{sec:guarantee} and~\ref{sec:detcontri} (in the appendix), about how these guarantees can be exponentially better than the classical ones.
%We derive simple regret (refer to Section~\ref{sec:def}) bounds analogous to
% the gap dependent bounds on the probability of misidentification.
 
{\noindent \bf (Novel $f$-divergence measure for analyzing Importance Sampling )} We provide a novel analysis of \textit{clipped importance sampling} estimators, where pairwise $f$-divergences between the distributions
 $\{\mathrm{P}_{k}(V \vert pa(V))\}$, for a carefully chosen function $f(.)$
 (see Section~\ref{sec:divergence}) act as the `effective variance'
 term in the analysis for the estimators (similar to Bernstein's bound~\cite{bennett1962probability}).
 

{\noindent \bf (Extensive Empirical Validation)} We demonstrate that our algorithm outperforms the prior works~\cite{lattimore2016causal,audibert2010best} on the Flow Cytometry data-set~\cite{sachs2005causal} (in Section~\ref{sec:cytometry}). We also exhibit an innovative application of our algorithm in the context of model interpretation of the Inception Deep Network~\cite{szegedy2015going} for classification of images (refer to Section~\ref{sec:inception}).

\begin{remark}
The techniques in this paper can be directly applied to more general settings like (i) the intervention source ($V$) can be a collection of nodes ($\mathcal{V}$) and the changes affect the distribution $P(\mathcal{V} \vert pa(\mathcal{V}))$, where  $pa(\mathcal{V})$ is the union of all the parents; (ii) the importance sampling can be applied at a directed cut separating the sources and the targets, provided the effect of the interventions, on the nodes forming the cut can be estimated. Moreover, our techniques can be applied without the complete knowledge of the source distributions. We explain the variations in more detail in Section~\ref{sec:variation} in the appendix.
\end{remark} 

 
%  \begin{figure}
%\centering
%\includegraphics[width=\linewidth]{Bottou_example.pdf}
%\caption{{\small Example of computational advertising borrowed from
%\cite{bottou2013counterfactual}. Various observable variables and
%hidden variables are shown. The topology of the causal graph is known;
%however the strengths of most interactions are unknown. A click-rate
%scoring algorithm predicts future user click-rates from users' search
%queries and the set of ads relevant to the user query chosen
%from an ad inventory. The algorithm's output determines the ads
%displayed (as well as the display style), and through a complex causal
%graph, finally determines actual revenue. The part of the network in
%bold -- distribution of user queries and matching ad keywords is known
%(including strengths), and the input output characteristics of several
%candidate (randomized) click-rate scoring algorithms are known. The
%objective is to choose the best algorithm that maximizes the revenue
%(target in bold red).}} \label{fig:Bottou}
%\end{figure}
 
% \subsection{An Example in Computational Advertising
%~\cite{bottou2013counterfactual}} 
%
%To illustrate our model, we revisit the computational advertisement example~\cite{bottou2013counterfactual} in more detail. In
%this example, the causal graph among various observable entities in a
%computational advertising system is known (however, the strengths of
%various interactions are not known). The corresponding causal graph is
%illustrated in Figure~\ref{fig:Bottou} (borrowed
%from~\cite{bottou2013counterfactual}).
%
%The overall goal of the system is to maximize the expected value of the \textit{target} variable \textit{revenue} (this is the target $Y$ in our causal system). In the advertisement system, a click-rate scoring algorithm is employed to predict future user
%\textit{click-through rate score} (an intermediate variable in the causal graph). This algorithm takes as input, the \textit{user query} word and the
%set of ad keywords (\textit{ads chosen}) that match the query word, and outputs a click-through rate
%score. This score in-turn influences the pricing and ad placement
%strategies, which in turn affects the revenue (see
%Figure~\ref{fig:Bottou}). In this example we are concerned with choosing the best scoring algorithm, that influences the causal relation between the predicted click-through rate score (equivalent to $V$ in our causal system) and its parents user query word and ad keywords in the causal graph (equivalent to $pa(V)$ in our causal system). 
%There are many candidate randomized scoring algorithms, and the input -
%output characteristics of each one are well studied. This means that
%for each of these algorithms, the conditionals
%$\mathrm{P}_k(\mathrm{Click-through~rate~score} |
%\mathrm{User~Query},\mathrm{Ads~chosen})$ are known. In the causal
%model, this is equivalent to knowing $\mathrm{P}_k (V | pa (V) ),$ where $V$ is
%identified with $\mathrm{click-through~rate~score}$. The task then is to find
%the best algorithm (arms or mechanisms determining $\mathrm{P}(V | pa (V) )$) that maximizes the revenue (target $Y$). This has a natural interpretation as a \textit{best arm identification} problem in bandits~\cite{audibert2010best}. Each of the mechanisms influencing the conditional $\mathrm{P}(V | pa(V))$ (eg. click rate prediction algorithms) can be thought of as the arms of the bandit. The expectation of the target $Y$ under arm/mechanism $i$ (revenue when algorithm $i$ is deployed) is considered to be the reward from arm $i$. The task is to identify the best arm with maximum certainty given a sample budget of $T$ interventions. The crucial difference from the classic best arm setting is that there is information leakage among the arms of the bandit through the shared causal graph.
%
%It should be noted that the level of difficulty to obtain samples from various algorithms can be very different in practice. For instance some of the algorithms above, may be default and easy to engineer and deploy, while others require a lot of engineering effort. Therefore, it is natural to expect a lot of samples from the default algorithms as compared to the more difficult ones. We model this is into our setting through a budget on the relative fractions of samples from different interventions (in addition to the total sample budget $T$). It is assumed that the cost associated with mechanism $i$ is $c_i$ ($c_i$ is high for an algorithm that is difficult to implement). Then we require that $\sum_{i \in [K]} c_i\nu_i \leq B$, where $\nu_i$ is the fraction of times arm $i$ is sampled and $B$ is the total fractional budget constraint.  Thus, it is evident that our causal setting is adequate in handling all the design issues in the optimization problem in the above example. In fact, it can be applied to a wide range of similar best arm identification settings with an underlying causal graph. 
 
 \subsection{Related Work}
    The problem lies at the intersection of causal inference and best
arm identification in bandits, similar in spirit
to~\cite{lattimore2016causal}. %We will review some of the relevant work in these areas and finally distinguish ourcontribution from that of \cite{lattimore2016causal}. 

The classical \textit{best arm identification} problem has been studied extensively in the bandit literature, both in the fixed confidence regime~\cite{gabillon2012best} and in the fixed budget setting~\cite{audibert2010best,chen2015optimal,jamieson2014lil,carpentier2016tight}. It was shown recently in
\cite{carpentier2016tight} that the results of \cite{audibert2010best}
are optimal.  The key difference from our work is that, in these
models, there is no information leakage among the arms.

There has been a lot of work \cite{mooij2016distinguishing,Hyttinen2013,Eberhardt2008X,Hauser2012b,Spirtes2001,Pearl2009}
on \textit{learning casual models} from data and/or experiments and using it to
\textit{estimate causal strength} questions of the \textit{counterfactual} nature. One
notable work that partially inspired our work is
\cite{bottou2013counterfactual} where the causal graph underlying a
computational advertising system (like in Bing, Google etc.) is known
and the primary interest is to find out how a change in the system
would affect some other variable.
  
At the intersection of \textit{causality and bandits}, \cite{lattimore2016causal} is perhaps most
relevant to our setting. The authors study the problem of identifying the best hard interventions on multiple variables (among many), provided the distribution of the parents of the target is known under those interventions. Simple regret bound of order $O(1/\sqrt{T})$ was derived. We assume soft interventions that affect the mechanism between
a 'source' node and its parents far away from the target (similar to
the case of computational advertising considered in
\cite{bottou2013counterfactual}). Further, we derive the first
\textit{gap dependent} bounds (that can be exponentially small in $T$),
generalizing the results of \cite{audibert2010best}. Our formulation can handle general budget constraints on the bandit arms and also recover the problem independent bounds of~\cite{lattimore2016causal} (orderwise).

In the context of machine learning, \textit{importance sampling} has been mostly used to recondition input data to adhere to conditions imposed by learning algorithms~\cite{sugiyama2007covariate,li2011unbiased,zhang2014stochastic}.


 
 
 




==> Introductionv9.tex <==
\label{sec:intro}


Causal graphs \cite{pearl2009causality} are useful for representing
causal relationships among interacting variables in large systems
\cite{bottou2013counterfactual}. Over the last few decades, causal
models have found use in computational
advertising~\cite{bottou2013counterfactual}, biological
systems~\cite{meinshausen2016methods},
sociology~\cite{blalock1985causal} and
agriculture~\cite{splawa1990application} and epidemiology
\cite{joffe2012causal}.
%
There are two important questions commonly studied with causal graphs: {\em
(i)} How to learn a directed causal graph that encodes that pattern of
interaction among components in a system (\textit{casual structure
learning})?~\cite{pearl2009causality}~, and {\em (ii)} Using
previously acquired (partial) knowledge about the causal graph
structure, how to estimate and/or to optimize the effect of a new
\textit{intervention} on other variables (\textit{optimization})~\cite{bottou2013counterfactual,joffe2012causal,kemmeren2014large,bonneau2007predictive,krouk2013gene}?
Here, an \textit{intervention} is a forcible change to the value of one of
the variables in a system. The change either alters the relationship
between the parental causes and the variable, or decouples it from the
parental causes entirely.
%Knowing the structure of the causal graph alone is not sufficient to
%answer questions about the quantitative effect of future
%interventional changes. For this, one needs to know the strength of
%various causal relationships in addition to the structure of the
%causal graph.
In this work, our focus is on optimizing over a set of given interventions.
 
 %
An illustrative example includes online advertising
\cite{bottou2013counterfactual}, where there is a collection of
click-through rate scoring algorithms that provide an estimate of the
probability that a user clicks on an ad displayed at a specific
position. The interventions occur through the choice of click-through
rate scoring algorithm; the algorithm choice directly impacts ad
placement and pricing, and through a complex network of interactions,
affects the revenue generated through advertisements. The revenue
%(downstream node in a causal
%graph)
 is used to determine the best scoring algorithm (optimize for the
best intervention); see Figure~\ref{fig:Bottou}. Another example is in
biological gene-regulatory networks \cite{bonneau2007predictive},
where a large number of genomes interact amongst each other and also
interact with environmental factors. The objective here is to
understand the best perturbation of some genomes in terms of its
effect on the expression of another subset of genomes (target) in
cellular systems. %(the downstream node).

This paper focuses on the following setting: We are given apriori
knowledge about the structure and strength of interactions over a
small part of the causal graph.  In addition, there is freedom to
intervene (from a set of allowable interventions) at a certain node in
the known part of the graph, and collect data under the chosen
intervention; further we can alter the inteventions over time and
observe the corresponding effects. Given a set of potential
interventions to optimize over, the key question of interest is: How
to choose the best sequence of $T$ allowable interventions in order to
discover which intervention maximizes the expectation of the
downstream target node.

Determining the best intervention in the above setting can be cast as
a best arm identification bandit problem, as noted in
\cite{lattimore2016causal}. In the classical setting, the objective is
to identify the best bounded random variable (called bandit arm) among
a finite collection that has the maximum mean. One is given the
freedom to observe the reward from any of the arms, i.e. one random
realization of the chosen variable at every time step. In our problem,
a bandit arm being played is equivalent to choosing one of the
allowable interventions and observing a reward. The reward from an
intervention (an arm) corresponds to a sample from the target node
that is observed under that intervention. As in the best arm setting,
one needs to allocate a total allowable budget of $T$ samples among
the set of interventions (arms), in order to maximize the certainty of
picking the best arm.

A key property we use is that these interventions are correlated,
i.e. there is information leakage that informs us about how good one
arm is by observing the performance of another. Classical best arm
identification~\cite{audibert2010best} does not model such information
leakage among arms; our goal is to extend the theory for this regime
and quantify the benefits of information leakage. Information leakage
effects are natural for various problems.  For example, Bonneau et
al.~\cite{bonneau2007predictive} study the causal interaction network
for gene expression under different environmental and genetic
perturbations.  There is information leakage in this problem since it
is possible to predict effects under unseen changes i.e. untested
interventions. Similarly, Bottou et
al.~\cite{bottou2013counterfactual} show that the performance of
untested ad scoring algorithms can be predicted from different scoring
models.  Recent work \cite{lattimore2016causal} has leveraged this
information leakage and developed algorithms for approximating the
best possible sequence of interventions for discovering the optimal
policy.

%A key property in this setting that we leverage, is that these
%interventions are correlated, and have predictive ability across
%interventions ({\em information leakage} across interventions). In
%contrast, the classical best arm identification
%problem~\cite{audibert2010best} has no information leakage among the
%arms. In our setting, sampling an arm provides additional information
%about other arms. For instance in \cite{bonneau2007predictive},
%experimental data under different environmental and genetic
%perturbations were collected, and a partial model (on $80\%$ of the
%nodes) of the network of causal interactions was built for
%\textit{Halo-bacterium salinarum NRC-1}. This model was then used to
%predict effects (inference) under new unseen changes (untested
%interventions). Similarly in \cite{bottou2013counterfactual}, the
%performance of new untested scoring algorithms could be predicted
%using the observed effects of a collection of previously tested
%algorithms. Indeed, recent work \cite{lattimore2016causal} has
%leveraged such information leakage, and developed algorithms for
%determining the sequence of interventions.  (with gap-independent
%bandit performance bounds, where the gap is the difference in the
%effect at the observed node across pairs of interventions).

More formally, suppose that $V$ is a node in a causal graph
$\mathcal{G}(\mathcal{V}, \mathcal{E})$, with the parents of $V$
denoted by $pa(V).$ This essentially means that $V$ is causally
determined by a function of $pa(V)$ and some exogenous random
noise. This dependence is characterized by the conditional
$\mathrm{P}(V | pa(V))$. Then a (soft) intervention mathematically
corresponds to changing this conditional probability distribution
i.e. probabilistically forcing $V$ to certain states given its
parents\footnote{These changes through the conditional distributions
are also called \textit{soft
interventions}~\cite{pearl2009causality}. Note that our algorithm is
also applicable to the more general case when the set of interventions
to optimize over is much larger than the set of interventions
available to sample from. This 'transfer of knowledge' to an unseen
but informationally related situation is also an important
motivation. Formally, it is possible to choose the best soft intervention in $\{0,1 \cdots , K-1 \}$ by only observing samples under interventions in the set $\mathcal{S}$, where $\mathcal{S} \subset [K]$.}. Further, suppose that the effect of an intervention is
observed at a node $Y$ which is downstream of $V$ in the topological
order (w.r.t $\mathcal{G}$).  Then, our key question is stated as
follows: \textit{Given a collection of interventions $\{\mathrm{P}_0
(V| pa(V)), \mathrm{P}_1 (V| pa(V))\ldots \mathrm{P}_{K-1}(V |
pa(V))\},$ find the best intervention among these $K$ possibilites
that maximizes $E[Y]$ under a fixed budget of $T$ (intervention,
observation) pairs.}

Our main result in this paper is a \textit{successive rejects bandit
algorithm} for selecting the sequence of interventions, to determine
the best one that has the maximum desired effect on a downstream
node. Our algorithm uses past observations along with information
leakage across interventions to sequentially eliminate sub-optimal
interventions. We provide the first \textit{gap-dependent} simple
regret and error bounds for this problem. Further, our solution
explicitly accounts for possible cost constraints on using
interventions. As a special case, we recover the gap-independent
result in \cite{lattimore2016causal} (orderwise).





% % {\bf Causal Model:} A causal model $\mathcal{G}(\mathcal{V},
% % \mathcal{E})$~ is an acyclic directed graph on the variables
% % $\mathcal{V}$ in a large system. Every directed edge represents a
% % direct causal link. In such a causal graph, a variable $V \in
% % \mathcal{V}$ is assumed to be a function of its parents $pa(V)$ and
% % some random noise external to the system. We focus on a particular
% % variable $V,$ and assume that the characteristics of the local
% % portion of the graph around $V$ is well-known from previously
% % collected data or domain knowledge (e.g. the input-output
% % characteristic of the algorithm in the advertisement
% % engine~\cite{bottou2013counterfactual}). Let $pa(V)$ denote the
% % parents of $V$ in the causal graph. Then, the conditional probability
% % distribution $P (V | pa(V) )$ between parents and the child captures
% % information about their causal interaction. 

% % A change or an intervention made on node $V$ is equivalent to altering
% % the conditional distribution\footnote{These changes through the
% % conditional distribution are also called \textit{soft}
% % interventions~\cite{pearl2009causality}.} $P (V | pa(V) ).$ Suppose
% % that we have prior knowledge of the marginal of $pa(V),$ and are given
% % $K$ possible choices of interventions $\{\mathrm{P}_0 (V| pa(V)), \mathrm{P}_1 (V|
% % pa(V))\ldots \mathrm{P}_{K-1}(V | pa(V))\}.$ The key question then is as
% % follows: \textit{Find the best interventions among the $K$
% % possibilites that maximizes the expectation of another target variable
% % $Y$ which is downstream of $V$ in the topological order (w.r.t
% % $\mathcal{G}$) under a fixed budget of $T$ samples.}


% {\bf Computational Advertising
% Example~\cite{bottou2013counterfactual}: } To illustrate, consider a
% real world example borrowed from \cite{bottou2013counterfactual} in
% Figure~\ref{fig:Bottou}. In this example, the causal graph among
% various observable entities in a computational advertising system is
% known (however, the strengths of various interactions are not known).
% A click-rate scoring algorithm is employed to predict future user
% click-rate. This algorithm takes as input, the user query word and the
% set of ad keywords that match the query word, and outputs a click-rate
% score. This score in-turn influences the pricing and ad placement
% strategies, which in turn affects the revenue (see
% Figure~\ref{fig:Bottou}). 

% There are many candidate randomized scoring algorithm, and the input -
% output characteristics of each one are well studied. This means that
% for each of these algorithms, the conditionals
% $\mathrm{P}_k(\mathrm{Click~rate~score} |
% \mathrm{User~Query},\mathrm{Ads~chosen})$ are known. In the causal
% model, this is equivalent to knowing $\mathrm{P}_k (V | pa (V) ),$ where $V$ is
% identified with $\mathrm{click-rate~score}$. The task then is to find
% the best algorithm that maximizes the revenue (target $Y$). Prior
% knowledge might give us reason to trust a subset the algorithms over
% the others; these trusts can then be encoded in terms of differential
% budgets for various interventions.


%  \begin{figure}
% \centering
% \includegraphics[width=11cm]{Bottou_example.pdf}
% \caption{Example of computational advertising borrowed from
% \cite{bottou2013counterfactual}. Various observable variables and
% hidden variables are shown. Basic information (topology) is
% known.There is an algorithm that is employed to predict future user
% click-rates from search queries users make and from the set of ads
% relevant to the user query chosen from an ad inventory. The output of
% the algorithm decides the style of ad display and through many more
% interactions finally determines actual revenue. The part of the
% network in bold - distribution of user queries and matching ad
% keywords is known and the input output characteristics of several
% candidate randomized prediction algorithms is known. One needs to
% choose the best algorithm that maximizes the revenue (target in bold
% red).    } \label{fig:Bottou} 
% \end{figure}

 
% %  {\bf Gene Network Example~\cite{meinshausen2016methods}: }Another
% % real word example, is gene regulatory networks, where different gene
% % perturbation experiments have been conducted in a specific sub-part of
% % the network and data has been collected. We would like to synthesize
% % these different changes and predict the best change that brings a
% % desired outcome elsewhere in the network
% % \cite{meinshausen2016methods}. Although \cite{meinshausen2016methods}
% % talks about first learning the casual graph, we are interested in
% % utilizing prior knowledge (in terms of marginals and conditional
% % distributions) in a known part of the graph, in order to infer the
% % causal effects of changes in this known portion, on some other
% % possibly unknown part of the causal network.
 
% % The above problem of identifying the best mechanism (soft
% % interventions) out of many possible ones in the known part of the
% % graph, in terms of its effect on a \textit{target} variable in a
% % larger causal network has strong similarities to the problem of best
% % arm identification in bandits, when the number of samples are
% % limited~\cite{lattimore2016causal}.

% {\bf Best Arm Identification Setting:} As noted in
% \cite{lattimore2016causal}, there is a strong connection between this
% problem of choosing the best intervention, and identifying the best
% arm in a multi-armed bandit problem.

% The problem of best arm identification in the context of the classic
% multi-armed bandit problem, has been well studied in the
% literature~\cite{audibert2010best, gabillon2012best}. Our problem can
% be cast as a best arm identification problem, with a few important
% twists. The $K$ candidate mechanisms that lead to the different
% conditional distributions $\{\mathrm{P}_{k}(V | pa(V)) \}_{k=0}^{K-1}$ can be
% thought of as the arms of the bandit. These conditionals can be
% assumed to be known from prior data (\textit{transfer of knowldege}).
% For instance in the computational advertising example, the algorithms
% affecting $(\mathrm{User~Query},\mathrm{Ads~chosen} \rightarrow
% \mathrm{click-rate~score})$ are the candidate mechanisms/arms. Their
% effects on the distribution $\mathrm{P}( \mathrm{click-rate~score} |$$
% \mathrm{User~Query},$$\mathrm{Ads~chosen})$ and the marginal
% distribution of $\mathrm{User~Query}$ and $\mathrm{Ads~chosen}$ seen
% by the system can be estimated from prior data and domain knowledge.
 
%  The quality of an arm is judged by its effect on a \textit{target}
% variable $Y$ (eg. user click-rate in advertising) which is further
% downstream in the less known portion of the causal graph. The task is
% to identify the mechanism that yields the highest expected reward
% $\EE[Y]$ given limited samples of $\{Y,pa(V),V \}$ from the various
% mechanism. Further, all mechanisms have a cost associated with it when
% they are used at $pa(V) \rightarrow V$ to collect samples about $Y$.
% So the problem also involves an additional cost budget that constrains
% the relative number of times different mechanisms are played. This is
% essential to capture real world restrictions; for instance, some of
% the candidate algorithms in the advertisement setting may be easier to
% deploy than others.
 
% The key difference between this and the naive best arm identification
% problem for bandits \cite{audibert2010best} is that any arm {\em leaks
% information} about any other arm due to the changes being propagated
% through a shared causal graph to the same target variable. Tracking
% and utilizing this information leakage is the key aspect of this
% problem. In this paper, we characterize the hardness of the problem in
% terms of various system parameters like the relationship between the
% candidate mechanisms and the gaps of the optimal mechanism from the
% rest in terms of the effect on \textit{target}. We list our main
% contributions in the following section.

 \subsection{Main Contributions}
 
 Our main contributions are the following:

 \begin{enumerate}
 \item {\bf (Gap Dependent Error Guarantees under budget constraints)}
 We derive the first \textit{gap dependent} (gaps between the
 expectations of the target under different interventions unknown to
 our algorithm) bounds on the probability of misidentification in
 terms of the number of samples $T$, cost budget $B$ on the relative
 fraction of times various arms are sampled and the divergences
 between different conditional probability distributions underlying
 the changes. Our result generalizes that of \cite{audibert2010best}
 which derives that the number of samples needed is (upto poly
 log factors) $\max_i (i/\Delta_{(i)}^2)$ where $\Delta_{(i)}$ is the
 $i$-th smallest gap from the optimal (for the classic best arm
 identification problem with no information leakage). This can be interpreted as the
 number of samples needed to eliminate arm $(i)$ from arms whose gaps
 are smaller than $\Delta_{(i)}$ in the case of no information
 leakage.
% Note that, it is easy to see that sum of the these terms is an
% achievable sample complexity. However, just the maximum number of
% samples required for any of these stages is sufficient. Thats the
% main contribution of \cite{audibert2010best}.
 
 We obtain a similar result (upto poly log factors) where the the
factor $i$ is replaced by the 'effective variance' of the estimator
for arm $(i)$, i.e. we obtain (with informal notation) $\max_i
\sigma_i^2/\Delta_{(i)}^2$. Here, $\sigma_i^2$ is the effective
variance of combining {\em clipped importance sampled estimates} of
various arms to eliminate $i$ from amongst those whose gap from
optimal is roughly less than $\Delta_i$. We also show that in general,
the effective variance term is lesser than $i$, as we leverage the
information leakage between the arms. In addition, we also note that
neither of the related prior works \cite{lattimore2016causal} (gap
independent bounds but with information leakage) nor
\cite{audibert2010best} (gap dependent bounds but with no information
leakage) deal with the budget constraints explicitly.
 
\item {\bf (Gap Dependent Guarantees on Simple Regret)} We derive
 simple regret (refer to Section~\ref{sec:def}) bounds analogous to
 the gap dependent bounds on the probability of misidentification.
 
 \item {\bf (Successive Rejects Algorithm leveraging Information
Leakage)} We provide an efficient \textit{successive rejects} multi-phase
algorithm that achieves these guarantees. The algorithm uses
\textit{clipped importance sampling} based estimators to leverage
information leakage. Clipping controls the variance by introducing a
mean bias in the estimates. Thus setting clipper levels becomes
crucial. At any phase, our algorithm \textit{adaptively} chooses the
clipper levels of the estimators and also allocates samples among the
arms to estimate those remaining after rejection in prior phases.
%These choices are based only on the divergences between the
%distributions ($\{\mathrm{P}_{k}(V | pa(V)) \}$) of the arms and the phase
%number.
Our procedure yields a major improvement over the algorithm in~\cite{lattimore2016causal} (both in theoretical guarantees and in
practice), which sets the clippers and allocates samples in a static
manner.
%Therefore, our algorithm effectively combines the successive rejects
%style of~\cite{audibert2010best} with the importance sampling
%techniques by leveraging a tighter analysis of the clipped importance
%sampled estimator (see Section~\ref{sec:divergence}).
We also demonstrate through synthetic
simulations that our algorithm outperforms the algorithms in
\cite{lattimore2016causal} and \cite{audibert2010best} - both of which
are suitably modified to take into account the additional cost budget
during comparison.
 
 \item {\bf (Analysis of Importance weighted Estimators)} 
%As mentioned before, our algorithm leverages information leakage
%among arms and combines samples from all arms through clipped
%importance sampling techniques, in order to estimate the reward under
%a particular arm.
 We show that pairwise $f$-divergences between the distributions
 $\{\mathrm{P}_{k}(V \vert pa(V))\}$, for a carefully chosen function $f(.)$
 (see Section~\ref{sec:divergence}) act as the `effective variance'
 terms in the analysis for the clipped importance sampling based
 estimators we employ. Much like standard Bernstein bounds, the
 clipper level controls the support, while the $f-$divergence
 controls the variance. This relationship may be of independent
 interest.
 \end{enumerate}
 
  \begin{figure}
\centering
\includegraphics[width=\linewidth]{Bottou_example.pdf}
\caption{{\small Example of computational advertising borrowed from
\cite{bottou2013counterfactual}. Various observable variables and
hidden variables are shown. The topology of the causal graph is known;
however the strengths of most interactions are unknown. A click-rate
scoring algorithm predicts future user click-rates from users' search
queries and the set of ads relevant to the user query chosen
from an ad inventory. The algorithm's output determines the ads
displayed (as well as the display style), and through a complex causal
graph, finally determines actual revenue. The part of the network in
bold -- distribution of user queries and matching ad keywords is known
(including strengths), and the input output characteristics of several
candidate (randomized) click-rate scoring algorithms are known. The
objective is to choose the best algorithm that maximizes the revenue
(target in bold red).}} \label{fig:Bottou}
\end{figure}
 
 \subsection{An Example in Computational Advertising
~\cite{bottou2013counterfactual}} 

To illustrate our model, we revisit the computational advertisement example~\cite{bottou2013counterfactual} in more detail. In
this example, the causal graph among various observable entities in a
computational advertising system is known (however, the strengths of
various interactions are not known). The corresponding causal graph is
illustrated in Figure~\ref{fig:Bottou} (borrowed
from~\cite{bottou2013counterfactual}).

The overall goal of the system is to maximize the expected value of the \textit{target} variable \textit{revenue} (this is the target $Y$ in our causal system). In the advertisement system, a click-rate scoring algorithm is employed to predict future user
\textit{click-through rate score} (an intermediate variable in the causal graph). This algorithm takes as input, the \textit{user query} word and the
set of ad keywords (\textit{ads chosen}) that match the query word, and outputs a click-through rate
score. This score in-turn influences the pricing and ad placement
strategies, which in turn affects the revenue (see
Figure~\ref{fig:Bottou}). In this example we are concerned with choosing the best scoring algorithm, that influences the causal relation between the predicted click-through rate score (equivalent to $V$ in our causal system) and its parents user query word and ad keywords in the causal graph (equivalent to $pa(V)$ in our causal system). 
There are many candidate randomized scoring algorithms, and the input -
output characteristics of each one are well studied. This means that
for each of these algorithms, the conditionals
$\mathrm{P}_k(\mathrm{Click-through~rate~score} |
\mathrm{User~Query},\mathrm{Ads~chosen})$ are known. In the causal
model, this is equivalent to knowing $\mathrm{P}_k (V | pa (V) ),$ where $V$ is
identified with $\mathrm{click-through~rate~score}$. The task then is to find
the best algorithm (arms or mechanisms determining $\mathrm{P}(V | pa (V) )$) that maximizes the revenue (target $Y$). This has a natural interpretation as a \textit{best arm identification} problem in bandits~\cite{audibert2010best}. Each of the mechanisms influencing the conditional $\mathrm{P}(V | pa(V))$ (eg. click rate prediction algorithms) can be thought of as the arms of the bandit. The expectation of the target $Y$ under arm/mechanism $i$ (revenue when algorithm $i$ is deployed) is considered to be the reward from arm $i$. The task is to identify the best arm with maximum certainty given a sample budget of $T$ interventions. The crucial difference from the classic best arm setting is that there is information leakage among the arms of the bandit through the shared causal graph.

It should be noted that the level of difficulty to obtain samples from various algorithms can be very different in practice. For instance some of the algorithms above, may be default and easy to engineer and deploy, while others require a lot of engineering effort. Therefore, it is natural to expect a lot of samples from the default algorithms as compared to the more difficult ones. We model this is into our setting through a budget on the relative fractions of samples from different interventions (in addition to the total sample budget $T$). It is assumed that the cost associated with mechanism $i$ is $c_i$ ($c_i$ is high for an algorithm that is difficult to implement). Then we require that $\sum_{i \in [K]} c_i\nu_i \leq B$, where $\nu_i$ is the fraction of times arm $i$ is sampled and $B$ is the total fractional budget constraint.  Thus, it is evident that our causal setting is adequate in handling all the design issues in the optimization problem in the above example. In fact, it can be applied to a wide range of similar best arm identification settings with an underlying causal graph. 
 
 \subsection{Related Work}
    The problem lies at the intersection of causal inference and best
arm identification in bandits, similar in spirit
to~\cite{lattimore2016causal}. There is a vast body of prior work in
related areas of casual inference, counterfactual estimation and best
arm identification in bandits. We will review some of the relevant
work in these areas and finally distinguish our
contribution from that of \cite{lattimore2016causal}.
    
  \textbf{Best arm Identification in Bandits:} The classical best arm
problem in bandits is to identify the best arm in terms of maximum
expected reward among $k$ independent arms. The problem has been
studied in two regimes (i) fixed confidence
regime~\cite{gabillon2012best} and (ii) fixed budget setting
\cite{audibert2010best}. The second regime is more relevant to our
work. Authors in \cite{audibert2010best} gave a successive rejects
based algorithm for this problem and guarantees on the error of
misidentification. This has been followed up in many subsequent works
\cite{chen2015optimal,jamieson2014lil}(see \cite{carpentier2016tight}
for more references). It was shown recently in
\cite{carpentier2016tight} that the results of \cite{audibert2010best}
are optimal. The key difference from our work is that, in these
models, there is no information leakage among the arms. When an arm is
pulled, it gives no information about the other arms.

  \textbf{Counterfactual Estimation and Causal Inference:} There has
been a lot of work
\cite{mooij2016distinguishing,Hyttinen2013,Eberhardt2008X,Hauser2012b,Spirtes2001,Pearl2009}
on learning casual models from data and/or experiments and using it to
estimate causal strength questions of the counterfactual nature. One
notable work that partially inspired our work is
\cite{bottou2013counterfactual} where the causal graph underlying a
computational advertising system (like in Bing, Google etc.) is known
and the primary interest is to find out how a change in the system
would affect some other variable when there is insufficient data
available for the change. Importance Sampling was used in this work as
an estimation tool to answer such counterfactual questions.
Essentially our work can be seen as a formal bandit modeling and analysis of this
counterfactual optimization question.
  
  \textbf{Causal Bandits:} \cite{lattimore2016causal} is perhaps most
relevant to our setting. The authors consider a causal graph ${\cal
G}$ and many possible hard interventions on multiple variables are
allowed. The objective is to choose the best intervention so as to
increase expected value of the target variable. They essentially
provide a $O(1/\sqrt{T})$ simple regret bound, which does not take
into account the parameters in the system, for instance the gaps from
the best arm. Further, it is assumed that the changes due to these
interventions on the parents of the target $Y$ are known(i.e.
marginals of the parents of the target under different changes are
known). We assume soft interventions that affect the mechanism between
a 'source' node and its parents far away from the target (similar to
the case of computational advertising considered in
\cite{bottou2013counterfactual}). Further, we derive the first
\textit{gap dependent} bounds where our sample complexity depends on
the gaps between expectations of the target under different changes
generalizing the results of \cite{audibert2010best}.
 
 \textbf{Importance Sampling in Machine Learning:} 
%In machine
%learning, for the classical problem of supervised learning used for
%classification, some times there is a covariate shift between the
%training and the test data. The authors in
%\cite{sugiyama2007covariate} propose an importance weighted cross
%validation procedure that avoids mis-estimation on the test data. One
%can see the mechanism changes in causal models as covariate shifts. It
%has also been used in offline policy evaluation in the bandit setting
%\cite{li2011unbiased}. In fact, we employ clipped importance sampling
%estimators as an important tool in our algorithm and further provide
%some confidence interval analysis relating it to $f$- divergence
%measures which may be of independent interest.
In the context of machine learning, importance sampling has been mostly used to recondition input data to adhere to conditions imposed by learning algorithms. For instance, in
\cite{sugiyama2007covariate} an importance weighted cross
validation procedure that avoids mis-estimation on the test data has
been proposed. Importance sampling has also been used in optimization
in order to reduce variance in stochastic descent methods
~\cite{zhang2014stochastic}. In connection to bandits, importance
sampling has been used for unbiased offline evaluations of bandit
algorithms~\cite{li2011unbiased}. 
% One can view these works as imposing causal changes in the data generation procedure through importance sampling. 

 
 
 




==> algorithm.tex <==
\label{sec:algo}
%We present two versions of \textit{successive rejects} style strategies, that attain the theoretical guarantees detailed in Section~\ref{sec:results}. Both the algorithms proceed in phases, successively rejecting arms at the end of each phase, until we are left with the optimal arm (provided $\Delta_{k} \geq 1/\sqrt{T}$ for all $k \in [K]$, otherwise it outputs a set of arms with $\Delta_k < 1/\sqrt{T}$). The only difference between Algorithms~\ref{algo:one} and \ref{algo:two} is that Algorithm~\ref{algo:one} only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while Algorithm~\ref{algo:two} reuses the past samples. 
Let us define some notation that is helpful in describing the main Algorithm:
\begin{enumerate}
\item $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $H_n = \sum_{i = 1}^{n}(1/i)$. 
\item We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set,
\begin{align}
\tau(l) &= \frac{T}{l H_{n(T)}} \label{taueq}\\
\end{align}
for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. Also, we have 
\begin{equation}\label{timeatphase}
T(l)= \frac{T H_l}{H_{n(T)}}.
\end{equation}
\item Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.
\end{enumerate}

Although, we assume that $P_k \left( V \lvert| PA(V) \right)$ and the marginal distribution $PA(V)$ are known, the algorithm we describe needs certain pairwise $f-$divergence values between these conditionals $P_k$. We describe the definition of $f-$ divergences we need. 

\subsection{Pairwise $f-$ divergences}\label{f-div}
\begin{definition}
Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
\begin{align*}
D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
\end{align*}
Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
\begin{align*}
D_{f}(p(X \vert Y) \Vert q(X \vert Y))= \sum_{y} q(Y = y) \left(\sum_{x} f \left( \frac{p(X = x \vert Y = y)}{q(X = x\vert Y = y)}\right)q(X = x\vert Y = y)\right)
\end{align*}
\end{definition}

 With some abuse of notation, we will denote $D_f(P_i(V \vert PA(V)) \Vert P_j(V \vert PA(V)))$ by the shorthand $D_f(P_i \Vert P_j)$. Consider the function $f_1(x) = x\exp(x-1) - 1$. We have the following relation,
\begin{align}
\label{eq:divergence}
 \mathbb{E}_{i} \left[ \exp \left( \frac{P_i(V \vert PA(V))}{P_j(V \vert PA(V))} \right) \right] = \left[ 1+D_{f_1}\left(P_i \lVert P_j\right) \right]e.
\end{align}

For notational convenience, let us define 
\begin{equation}
M_{ij} = 1 + \log (1 + D_{f_1} (P_i \lVert P_j))
\end{equation}

Now, we describe our main contribution - Algorithm \ref{alg:pickbest}.

\begin{algorithm*}
  \caption{PickBest - Given total budget $T$ and cost budget $B$ picks the best mechanism.}
  \begin{algorithmic}[1]
    \Function{PickBest}{$B,\{M_{kj} \},T$}
    \State ${\cal R} = [K]$.
    \State Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
    \For {$\ell=1$ to $n(T)$}      
        \State $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(B, \mathbf{A},{\cal R}, \tau(\ell) \right)$
        \State \label{linesamp} Use mechanism $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, PA(V) )$.
        \For {$k \in {\cal R}$}
    		\State Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator}) calculated with $\{M_kj \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\EndFor
	\State Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
	\State ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
	\If {$\lvert {\cal R}\rvert =1$}
	  	\State \textbf{return:} the arm in ${\cal R}$.
	\EndIf
    \EndFor
    \State \textbf{return:} A randomly chosen arm from ${\cal R}$.
   \EndFunction
      \end{algorithmic}
    \label{alg:pickbest}
\end{algorithm*}

\textbf{Remark:} The algorithm proceeds by having all the arms under consideration at the beginning. At the end of each phase some of the arms are possibly deemed sub-optimal and removed from consideration based on a phase specific criterion. 

==> inceptionv1.tex <==
\subsection{Interpretability of Inception Deep Network}
\label{sec:inception}
In this section we use our algorithm for \textit{model interpretation} of the pre-trained Inception-v3 network~\cite{szegedy2015going} for classifying images.  \textit{Model Interpretation} essentially answers: { \it 'why a learning model classifies in a certain way?'}, which is one of the most pertinent questions in the context of complicated learning models like deep nets~\cite{ribeiro2016should}.

When an RGB image is fed to Inception, it produces an ordered sequence of $1000$ labels (e.g 'drums', 'sunglasses') and generally the top-$10$ labels are an accurate description of the objects in the image. The task here is to segment the image into a number of \textit{superpixels}/segments (using segmentation algorithms like SLIC~\cite{achanta2010slic}) and infer which superpixel encourages the neural net to output a certain label (e.g 'drum') in top-$10$ and to what extent. This essentially means finding a mixture distribution over the superpixels where the mixture weights signify the amount by which the corresponding superpixels encourage Inception to produce the particular label as one of the top ones. 

We use our best arm identification algorithm to identify the best distribution over the superpixels of an image in terms of maximizing the probability of a particular label appearing in top-$k$ labels (for an appropriately chosen $k$). Sampling from an arm implies picking a few superpixels with replacement from the arm distribution, blurring out the rest of the pixels and feeding the resulting image into Inception. The reward is $1$ if the label being \textit{interpreted}  lies in the top-$k$ and $0$ otherwise. In our experiments in Figure~\ref{fig:cats}, the total number of superpixels is $43$ and each time $5$ superpixels are sampled from an arm distribution. 

We optimize over $3000$ arm distributions which lie in the $43$-dimensional simplex but have \textit{sparse} support (sparsity of $10$ in our examples). The support of these distributions are randomly generated by various techniques like markov random walk (encourages contiguity), random choice etc. as detailed in Section~\ref{sec:moreincep} in the appendix. However, we are only allowed to sample using $200$ arms that are dense distributions chosen uniformly at random from the $43$-dimensional simplex. The distributions are generated in a manner which is completely agnostic to the contents of an image. The total sample budget ($T$) is  $2500$. 

Figure~\ref{fig:cats} shows images in which the segments are weighted in proportion to the optimal distribution (obtained by SRISv2) for the interpretation of three different labels. This showcases the true counterfactual power of the algorithm, as the set of arms that can be optimized over are \textit{disjoint} from the arms that can be sampled from. Moreover the sample budget is \textit{less} than the number of arms. This is an extreme special case of budget setting \textbf{S2}. We see that our algorithm can generate meaningful interpretations for all the labels with relatively less number of runs of Inception. If information leakage is not leveraged, then even sampling $10$ times from each of the arms to be optimized over would require $30,000$ runs of Inception, while we need only $2500$. 
%In this section we demonstrate the use of our algorithm for \textit{model interpretation} of the pre-trained Inception-v3 network~\cite{szegedy2015going} for classifying images. \textit{Model Interpretation} essentially answers: { \it 'why a learning model classifies in a certain way?'}, which is one of the most pertinent questions in the context of complicated learning models like deep nets. LIME~\cite{ribeiro2016should} is a recent effort in this direction, where the authors use perturbed versions of images and LASSO to recover few \textit{superpixels} of an image that trigger a certain classifier label in Inception.
%
%
%We demonstrate that it is possible to use our algorithm to form a weighted version of an image, where the weight of each segment signifies the importance of that segment in triggering a particular label. We believe that this view can be much more informative that selecting a few segments alone. The methodology is as follows: (i) Segment the image into $n$ \textit{superpixels} using SLIC~\cite{achanta2010slic}. (ii) Generate \textit{pull} arms which are probability distributions over the segments, in a randomized fashion. (iii) Generate 'many' \textit{opt} arms which are again probability distributions over the segments. (iv) Suppose the objective is to \textit{explain} the occurrence of a particular label $l$. Then a sample reward for an arm is generated as follows: (a) select $m \ll n$ segments with replacement according to the distribution of the arm and blur out all the other segments (b) feed the resulting image into the network, and the reward is $1$ if label $l$ lies in top-$k$ (appropriately chosen $k$) of the predicted labels and $0$ otherwise. (v) Finally given a budget of $T$ samples, we use Algorithm~\ref{alg:pickbest2} to pick the best arm out of the \textit{opt} arms, while we are \textit{only} allowed to sample from the \textit{pull} arms (this is akin to setting $c_i = 1$ for if $i$ is a pull arm and $\infty$ if $i$ is an opt arm). The probability values in the optimal distribution are the weights of the segments for the label $l$.
%
%In Fig.~\ref{fig:cats}, we demonstrate the label explanations of a particular image (shown in Fig.~\ref{fig:cats1}). For this experiment. we (i) segment the image into $43$ superpixels (ii) use $200$ \textit{pull} arms (iii) use $3000$ \textit{opt} arms. (iv) use a budget of $T=2500$ samples. This shows the true \textit{counterfactual} nature of our algorithm as we are able to optimize over as many as $3000$ arms, while sampling from as few as $200$ arms, \textit{different} from the arms optimized over. Moreover, the total sample budget is \textit{less} than the number of arms. This allows us to optimize over a large set of arms and the optimal arm is indeed a meaningful interpretation. Note that the distributions of the arms are generated in a randomized manner, which is completely agnostic to the content of the images. We ellaborate more on this in Section~\ref{sec:moreincep} in the appendix.
\begin{figure}
	\centering
	\subfloat[][{\small Original Image}]{\includegraphics[width = 0.45\linewidth]{./figs/cats.JPEG}\label{fig:cats1}} \hfill
	\subfloat[][{\small Interpretation- \textit{Drums}}]{\includegraphics[width = 0.45\linewidth]{./figs/cats_drums_kk1_seg50.JPEG}\label{fig:cats2}} \\
	\subfloat[][{\small Interpretation- \textit{TigerCat}}]{\includegraphics[width = 0.45\linewidth]{./figs/cats_tigercat_kk200_seg50.JPEG}\label{fig:cats3}} \hfill
	\subfloat[][{\small Interpretation- \textit{Sunglasses}}]{\includegraphics[width = 0.45\linewidth]{./figs/cats_sunglasses_kk20_seg50.JPEG}\label{fig:cats4}}
	\caption{\small Interpretation for different top labels for the image in (a). The best arm algorithm can generate an image where the segments are weighted in proportion of their importance towards a particular label. For example, in (b) we see the drums highlighted more, while in (d) sunglasses are in the focus. We find that a part of the guitar is also highlighted when the chosen label is 'drums'. This can be attributed to the fact that drums and guitar appear together frequently on the imagenet data-set used to train Inception. In (c) both the cats are visible, however the cat with more tiger like fur has much more weightage. Such soft interpretations are not possible using the methods in~\cite{ribeiro2016should} }
	\label{fig:cats}
\end{figure}
\FloatBarrier

==> results.tex <==
\label{sec:results}
In this section we provide our main theoretical contributions. In Section~\ref{sec:algo}, we provide a successive rejects style algorithm, that leverages the information leakage between the arms, via importance sampling. Then, we provide theoretical guarantees on the probability of mis-identification $(e(T,B))$ and simple regret $(r(T,B))$ for our algorithm in Section~\ref{sec:guarantee}.
\subsection{An Efficient Algorithm}\label{sec:algo}
%We present two versions of \textit{successive rejects} style strategies, that attain the theoretical guarantees detailed in Section~\ref{sec:results}. Both the algorithms proceed in phases, successively rejecting arms at the end of each phase, until we are left with the optimal arm (provided $\Delta_{k} \geq 1/\sqrt{T}$ for all $k \in [K]$, otherwise it outputs a set of arms with $\Delta_k < 1/\sqrt{T}$). The only difference between Algorithms~\ref{algo:one} and \ref{algo:two} is that Algorithm~\ref{algo:one} only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while Algorithm~\ref{algo:two} reuses the past samples. 
We present a successive rejects style algorithm that leverages the information leakage among the arms, through importance sampling. The algorithm proceeds in phases. The algorithm starts with all the arms under consideration, and rejects zero or more arms at the end of each phase successively, until we are left with only the best arm or possibly a few arms which are \textit{very} close to the best arm.  Let us define some notation that is helpful in describing the main algorithm:
\begin{enumerate}
\item $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 
\item We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set,
\begin{align}
\tau(l) &= \frac{T}{\overline{\log}(n(T)) l} \label{taueq}\\
\end{align}
for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. Also, we have 
\begin{equation}\label{timeatphase}
T(l)= \frac{T \overline{\log}(l)}{\overline{\log}(n(T))}.
\end{equation}
\item Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.
\end{enumerate}

Although, we assume that $\mathrm{P}_k \left( V \vert pa(V) \right)$ and the marginal distribution $pa(V)$ are known, the algorithm we describe needs certain pairwise $f$-divergence values between these conditionals $\mathrm{P}_k$. The $f$-divergences can be calculated from the known distributions or estimated directly from data. Now we define the $f$- divergences that are required. 

\subsubsection{Pairwise $f$- divergences}\label{f-div}
\begin{definition}
Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
\begin{align*}
D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
\end{align*}
Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
\begin{align*}
&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
\end{align*}
\end{definition}

 With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by the shorthand $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. Consider the function $f_1(x) = x \exp (x-1) - 1$. We have the following relation,
\begin{align}
\label{eq:divergence}
 \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
\end{align}

For notational convenience, let us define log divergence to be:
\begin{equation}
\label{eq:mij}
M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))
\end{equation}

The divergence measure $M_{ij}$ between $\mathrm{P}_i$ and $\mathrm{P}_j$ can be related to the `effective standard deviation' of the estimator that estimates $\mathbb{E}[Y]$ under $\mathrm{P}_i$ using samples from $\mathrm{P}_j$. Larger the divergence, larger is the variance of the estimator.

\begin{definition}\label{effectivelogdivergence}
Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective variance} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ to be : 
    \begin{align}
\label{mainLP1}
&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
 &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
\end{align}
\end{definition}
$\sigma^*$ is the `effective standard deviation' when arms from $[K]$ are used to estimate the means of the arms in set ${\cal R}$, under relative fractional budget $B$. We will justify this by analyzing a heterogenous importance sampling estimator and deriving confidence intervals for it in later sections.

Now, we describe one of our main contributions - Algorithm \ref{alg:pickbest}.

\begin{algorithm}
  \caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $\nu_i$) picks the best arm.}
  \begin{algorithmic}[1]
    \STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
    \STATE ${\cal R} = [K]$.
    \STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
    \FOR {$\ell=1$ to $n(T)$}      
        \STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
        \STATE \label{linesamp} Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
        \FOR {$k \in {\cal R}$}
    		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\ENDFOR
	\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
	\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
	\IF {$\lvert {\cal R}\rvert =1$}
	  	\STATE \textbf{return:} the arm in ${\cal R}$.
	\ENDIF
    \ENDFOR
    \STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
      \end{algorithmic}
    \label{alg:pickbest}
\end{algorithm}
\textbf{Remark:} The algorithm proceeds by having all the arms under consideration at the beginning. At the end of each phase some of the arms are possibly deemed sub-optimal and removed from consideration based on a phase specific criterion. Note that Line \ref{linesamp} uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements. We will show our algorithms outperform all other algorithms in related prior work.

\begin{algorithm}
  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
  \begin{algorithmic}[1]
     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line \ref{samplestamp} where all samples acquired in all the phases till that Line is used.
    \end{algorithmic}
   \label{alg:pickbest2}
\end{algorithm}

\subsection{Theoretical Guarantees}
\label{sec:guarantee}
We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first problem dependent characterization of the problem.  
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%\begin{equation}
% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%  \end{equation}
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}

\begin{theorem}\label{mainresult}
(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) satisfies:
\begin{equation}
 e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
  \end{equation}
  when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
 Here, 
 \begin{align}
  \label{Hbar}
  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
  \end{align}
and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison to the result in \cite{audibert2010best}:}
Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result for the best arm identification with no information leakage in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}:
 \begin{equation}\label{noleakage}
   e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)
 \end{equation}

 One intuitive interpretation for $\tilde{H}$ is that it is the maximum among the number of samples (neglecting some log factors) required to conclude that arm $k$ is suboptimal from among the arms which are closer to the optimal than itself. Intuitively, this is because when there is no information leakage, one requires $1/\Delta_k^2$ samples to distinguish between the $k$-th optimal arm and the optimal arm. Further, the $k$th arm is played only $1/k$ fraction of the times since we do not know the identity of the $k$-th optimal arm. 
  
\textbf{Interpretation of our Result:}
Our main result in Theorem $\ref{mainresult}$ can be seen to be a generalization of the existing result in (\ref{noleakage}) for the case when there is information leakage between the arms (various changes in a causal graph).  

The term $\sigma^*(B,{\cal R}^*(\Delta_k))$ in our setting is the `effective standard deviation' due to information leakage.  There is a similar interpretation of our result (ignoring the log factors): Since there is information leakage, the expression $\frac{(\sigma^*)^2}{(\Delta_k)^2}$ characterizes the number of samples required to weed out arm $k$ out of contention from among competing arms (arms that are at a distance at most twice than that of arm $k$ from the optimal arm). The interpretation of 'effective variance' is justified using importance sampling which is detailed in Section \ref{sec:estimator}. Further, in our framework $\sigma^*$ also incorporates any budget constraint that comes with the problem, i.e. any \textit{apriori} constraint on the relative fraction of times different arms need to be pulled.

\textbf{Improvement over the no-information leakage case:}
For ease of exposition let $(k)$ denote the index of the $k$-th best arm (for $k = 1,..,K$) and $\Delta_{(k)}$ denotes the corresponding gap. In this setting, the terms $\tilde{H}$ (from the result in~\cite{audibert2010best}) and $\bar{H}$ can be written as:
\begin{align*}
\tilde{H} &= \max_{k \neq 1} \frac{k}{\Delta_{(k)}^2} \\
\bar{H} &= \max_{k \neq 1} \frac{\sigma^*(B,{\cal R}^*(\Delta_{(k)}))^2}{\Delta_{(k)}^2}.
\end{align*}
$ \sigma^*(B,{\cal R}^*(\Delta_{(k)}))$ can be smaller than $\sqrt{k}$ due to information leakage as every single arm pull contributes to another arm's estimate. Therefore, these provide better guarantees than ~\cite{audibert2010best}. 

To see the improvement over the previous result in \cite{audibert2010best}, we consider a special case when the cost budget $B$ is infinity and there is only the the sample budget $T$. In addition, let us assume that the log divergences are such that: $M_{ij} \leq \eta M_{ii} = \eta << \sqrt{\lvert {\cal R}  \rvert},~ \forall i \neq j$. Let ${\cal R} = {\cal R}^*(\Delta_{(k)})$. If $\eta > \sqrt{\lvert {\cal R}  \rvert}$, the optimal solution for (\ref{mainLP1}) is a bit complicated to interpret.  Consider the feasible allocation $\nu_i = \frac{1}{\lvert {\cal R}  \rvert}, ~ \forall i \in {\cal R}$ in (\ref{mainLP1}). Evaluating the objective function for this feasible allocation, it is possible to show that $\sigma^* \leq \frac{\eta}{1-1/\lvert {\cal R}  \rvert} <<  \sqrt{\lvert {\cal R}  \rvert}$. Hence, unless the variance due to information leakage is too bad, the effective variance is smaller than that of the case with no information leakage.

The improvement over the no information leakage setting, is even more pronounced under budget constraints. Consider the setting \textbf{S1}, and assume that the fractional budget of the \textit{difficult} arms, $B = o(1)$. This implies that the total number of samples available for difficult arms is $o(T)$. The budget constrained case has not been analyzed in~\cite{audibert2010best}, however in the absence of information leakage, one would expect that the arms with the least number of samples would be the most difficult to eliminate, and therefore the error guarantees would scale as $\exp(-O(BT)/\tilde{H}) \sim \exp(-o(T)/\tilde{H})$ (excluding $\log$ factors). On the other hand, our algorithm can leverage the information leakage and the error guarantee would scale as $\exp(-O(T)/\bar{H})$, which can be order-wise better if the \textit{effective standard deviations} are well-behaved. 

\textbf{Remark:} Although similar advantages can be shown for \cite{lattimore2016causal}, there are no gap dependent bounds in that work and our analysis indicates a gap dependent improvement term by term with respect to \cite{audibert2010best}.


 \begin{theorem}\label{mainresult2}
(Proved formally as Theorem \ref{thm:detailed})  Let $v^*$ be the effective inverse log divergence as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
\ \begin{align}
\label{eq:SRmain}
&r(T,B) \leq  \\
&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
 \end{align}
 Here, 
 \begin{align}
  \label{HK}
 \bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
  \end{align}
and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison to the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 

On the contrary, we provide problem dependent bounds, which differentiates the arms according to its gap from the optimal arm and its \textit{effective standard deviation} parameter. The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$. 

We defer the theoretical analysis to Section~\ref{sec:proofs}. In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we introduce the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 








==> resultsv2.tex <==
\label{sec:results}
In this section we provide our main theoretical contributions. In Section~\ref{sec:algo}, we provide a successive rejects style algorithm, that leverages the information leakage between the arms, via importance sampling. Then, we provide theoretical guarantees on the probability of mis-identification $(e(T,B))$ and simple regret $(r(T,B))$ for our algorithm in Section~\ref{sec:guarantee}. In order to explain our algorithm in more detail, we first provide some key definitions in Section~\ref{sec:def}.


\subsection{Definitions}
\label{sec:def}
%The algorithm starts by having all the $K$ arms under consideration and then proceeds in phases. At the beginning of each phase, a budget for samples is allocated to each arm. Thereafter, samples are collected according to the allocated budgets, and using these samples, importance sampling based estimators for the means of all the \textit{remaining} arms are formed. Then at the end of each phase, one or more arms are rejected based on some phase specific criterion on the estimated values. 
The structure of the algorithm and the estimation technique for the means of the arms,  both rely on a specific $f$-divergence between the arm distributions. These $f$-divergences can be calculated analytically or estimated directly from empirical data (without the knowledge of the full distributions) using techniques like that of~\cite{perez2008kullback}. We now define the specific divergences.

\begin{definition}
Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
\begin{align*}
D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
\end{align*}
Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
\begin{align*}
&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
\end{align*}
\end{definition}

 With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by the shorthand $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. Consider the function $f_1(x) = x \exp (x-1) - 1$. 
% We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
Let us define log divergences to be:
\begin{equation}
\label{eq:mij}
M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))
\end{equation}

%One way to view the information leakage among arms is through the following expression relating the mean under arm $i$ to samples collected under arm $j$,
%\begin{align}
%\label{eq:basic_main}
%\EE_{i}\left[Y\right] = \EE_{j}\left[Y\frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))}\right]
%\end{align}
%which is trivially true as the only change in the joint distribution of all variables is at $\mathrm{P}(V \vert pa(V))$. However, directly using this expression to form an estimator, can lead to arbitrarily bad concentration as the ratio in the expression can be unbounded. Therefore, it is essential to clip the importance weighted samples at a carefully chosen value, such that we balance the trade-off between the variance of the samples and the bias incurred by the clipping. 
In Theorem~\ref{lem:clippedmain} we show that the quantities $M_{ij}$'s are crucial in the analysis of clipped importance sampled estimators. It is possible to obtain information about the target mean under the $k^{th}$ arm ($\mu_k = \EE_{k}[Y]$) from the samples of all the other arms (refer to Section~\ref{sec:divergence}). We design an efficient estimator of $\EE_{k}[Y]$ ($\forall k \in [K]$) that seamlessly uses the samples from all arms, possibly with variable weights depending on the relative divergences between the distributions. The estimator is given by (\ref{eq:uniestimator_main}).

Suppose we obtain $\tau_{i}$ samples from arm $i \in [K]$. Let the total number of samples from all arms put together be $\tau$. Let us index all the samples by $s \in \{1,2,..,\tau \}$. Let $\mathcal{T}_{k} \subset \{1,2,..,\tau \}$ be the indices of all the samples collected from arm $k$. Further, let $Z_k = \sum_{j \in [K]}\tau_j/M_{kj}$. Now, we are at the position to introduce the estimator for $\mu_k$, which we will denoted by $\hat{Y}_{k}^{\epsilon}$ ($\epsilon$ is an indicator of the level of confidence desired):
\begin{align*}
\label{eq:uniestimator_main}
&\hat{Y}_{k}^{\epsilon}  = \frac{1}{Z_{k}}\sum_{j = 0}^{K} \sum_{s \in \mathcal{T}_j} \frac{1}{M_{kj}}Y_j(s)\frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \times
\\
&\mathds{1}\left\{ \frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \leq 2\log(2/\epsilon)M_{kj}\right\}. \numberthis
\end{align*}
In other words, $\hat{Y}_{k}^{\epsilon}$ is the weighted average of the clipped samples, where the samples from arm $j$ are weighted by $1/M_{kj}$ and clipped at $ 2\log(2/\epsilon)M_{kj}$. The choice of $\epsilon$ will be clearly specified when we present our algorithm. 

The log-divergences $M_{ij}$'s are also central in allocating the phase-wise budget of samples for the arms. We design the sub-method Algorithm~\ref{alg:allocate} (in the appendix) that allocates the samples adhering to budget restrictions, such that the estimators (\ref{eq:uniestimator_main}) of all the remaining arms are \textit{good} (quantified in Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the appendix). One key quantity that is closely related to this allocation and also crucial in the theoretical analysis, is the \textbf{effective standard deviation} $\sigma^*(B,{\cal R})$ for budget $B$ and the of set of arms  ${\cal R}$ remaining at the beginning of a phase. 
\begin{definition}\label{effectivelogdivergence}
Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective standard deviation} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ to be : 
    \begin{align}
\label{mainLP1}
&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
 &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
\end{align}
\end{definition}


\subsection{Algorithm}
Now, we describe our main algorithmic contributions - Algorithm \ref{alg:pickbest} and \ref{alg:pickbest2}.  Algorithm \ref{alg:pickbest}  starts by having all the $K$ arms (Step 1) under consideration and then proceeds in phases. At the beginning of each phase, a budget for samples is allocated to each arm (Step 5). Thereafter, samples are collected according to the allocated budgets, and using these samples, importance sampling based estimators for the means of all the \textit{remaining} arms are formed (Step 8). Then at the end of each phase, one or more arms are rejected based on some phase specific criterion on the estimated values (Step 11). The only difference between Algorithms~\ref{alg:pickbest} and \ref{alg:pickbest2} is that the former only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while the latter reuses the past samples. Let us define some notation that is helpful in describing the main algorithm:

\begin{algorithm}
	\caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $\nu_i$) picks the best arm.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
		\STATE ${\cal R} = [K]$.
		\STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
		\FOR {$\ell=1$ to $n(T)$}      
		\STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
		\STATE \label{linesamp} Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
		\FOR {$k \in {\cal R}$}
		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator_main}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\ENDFOR
		\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
		\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
		\IF {$\lvert {\cal R}\rvert =1$}
		\STATE \textbf{return:} the arm in ${\cal R}$.
		\ENDIF
		\ENDFOR
		\STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
	\end{algorithmic}
	\label{alg:pickbest}
\end{algorithm}

 $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 


 We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set $\tau(l) = T/(l\overline{\log}(n(T)))$ for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. So, we have $T(l)= (T \overline{\log}(l))/(\overline{\log}(n(T)))$.

Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.


\begin{remark}  Note that Line \ref{linesamp} uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements.
\end{remark}
\begin{algorithm}
  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
  \begin{algorithmic}[1]
     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line \ref{samplestamp} where all samples acquired in all the phases till that Line is used.
    \end{algorithmic}
   \label{alg:pickbest2}
\end{algorithm}
\label{sec:algo}
\subsection{Theoretical Guarantees}
\label{sec:guarantee}
We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first gap dependent characterization of the problem.  
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%\begin{equation}
% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%  \end{equation}
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}

\begin{theorem}\label{mainresult}
	(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The probability of error for  Algorithm \ref{alg:pickbest} satisfies:
	\begin{equation}
	e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
	\end{equation}
	when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
	Here, 
	\begin{align}
	\label{Hbar}
	\bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison to the result in \cite{audibert2010best}:}
Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result for the best arm identification with no information leakage in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}:
\begin{equation}\label{noleakage}
e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)
\end{equation}

%One intuitive interpretation for $\tilde{H}$ is that it is the maximum among the number of samples (neglecting some log factors) required to conclude that arm $k$ is suboptimal from among the arms which are closer to the optimal than itself. Intuitively, this is because when there is no information leakage, one requires $1/\Delta_k^2$ samples to distinguish between the $k$-th optimal arm and the optimal arm. Further, the $k$th arm is played only $1/k$ fraction of the times since we do not know the identity of the $k$-th optimal arm. 


Our main result in Theorem $\ref{mainresult}$ can be seen to be a generalization of the existing result in (\ref{noleakage}) for the case when there is information leakage between the arms (various changes in a causal graph).  

The term $\sigma^*(B,{\cal R}^*(\Delta_k))$ in our setting is the `effective standard deviation' due to information leakage.  %There is a similar interpretation of our result (ignoring the log factors): Since there is information leakage, the expression $\frac{(\sigma^*)^2}{(\Delta_k)^2}$ characterizes the number of samples required to weed out arm $k$ out of contention from among competing arms (arms that are at a distance at most twice than that of arm $k$ from the optimal arm). 
The interpretation  is justified using importance sampling which is detailed in Section \ref{sec:estimator}. Further, in our framework $\sigma^*$ also incorporates any budget constraint that comes with the problem, i.e. any \textit{apriori} constraint on the relative fraction of times different arms need to be pulled. In Section~\ref{sec:compare1} (in the appendix), we demonstrate through simple examples that $\sigma^*(B,{\cal R}^*(\Delta_k))$ can be significantly smaller than $\sqrt{\tilde{\mathcal{R}}(\Delta_k)}$ (the corresponding term in (\ref{noleakage})) even when there are no average budget constraints. Moreover, our results can be exponentially better in the presence of average budget constraints (examples in Section~\ref{sec:compare1}).

Now we present our bounds on simple regret in Theorem~\ref{mainresult2}.
%\textbf{Remark:} Although similar advantages can be shown for \cite{lattimore2016causal}, there are no gap dependent bounds in that work and our analysis indicates a gap dependent improvement term by term with respect to \cite{audibert2010best}.
\begin{theorem}\label{mainresult2}
	(Proved formally as Theorem \ref{thm:detailed})  Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
	\ \begin{align}
	\label{eq:SRmain}
	&r(T,B) \leq   \nonumber\\
	&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
	& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
	\end{align}
	Here, 
	\begin{align}
	\label{HK}
	\bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison to the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 

On the contrary, we provide problem dependent bounds. %The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. 
It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$ and can handle general constraints on average budgets. Further details are provided in Section~\ref{sec:compare2}. 

We defer the theoretical analysis to Section~\ref{sec:proofs}. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we analyze the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 




























%\subsection{An Efficient Algorithm}\label{sec:algo}
%%We present two versions of \textit{successive rejects} style strategies, that attain the theoretical guarantees detailed in Section~\ref{sec:results}. Both the algorithms proceed in phases, successively rejecting arms at the end of each phase, until we are left with the optimal arm (provided $\Delta_{k} \geq 1/\sqrt{T}$ for all $k \in [K]$, otherwise it outputs a set of arms with $\Delta_k < 1/\sqrt{T}$). The only difference between Algorithms~\ref{algo:one} and \ref{algo:two} is that Algorithm~\ref{algo:one} only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while Algorithm~\ref{algo:two} reuses the past samples. 
%We present a successive rejects style algorithm that leverages the information leakage among the arms, through importance sampling. The algorithm proceeds in phases. The algorithm starts with all the arms under consideration, and rejects zero or more arms at the end of each phase successively, until we are left with only the best arm or possibly a few arms which are \textit{very} close to the best arm.  Let us define some notation that is helpful in describing the main algorithm:
%\begin{enumerate}
%\item $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 
%\item We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set,
%\begin{align}
%\tau(l) &= \frac{T}{\overline{\log}(n(T)) l} \label{taueq}\\
%\end{align}
%for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. Also, we have 
%\begin{equation}\label{timeatphase}
%T(l)= \frac{T \overline{\log}(l)}{\overline{\log}(n(T))}.
%\end{equation}
%\item Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.
%\end{enumerate}
%
%Although, we assume that $\mathrm{P}_k \left( V \vert pa(V) \right)$ and the marginal distribution $pa(V)$ are known, the algorithm we describe needs certain pairwise $f$-divergence values between these conditionals $\mathrm{P}_k$. The $f$-divergences can be calculated from the known distributions or estimated directly from data. Now we define the $f$- divergences that are required. 
%
%\subsubsection{Pairwise $f$- divergences}\label{f-div}
%\begin{definition}
%Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
%\begin{align*}
%D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
%\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
%\end{definition}
%
% With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by the shorthand $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. Consider the function $f_1(x) = x \exp (x-1) - 1$. We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
%
%For notational convenience, let us define log divergence to be:
%\begin{equation}
%\label{eq:mij}
%M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))
%\end{equation}
%
%The divergence measure $M_{ij}$ between $\mathrm{P}_i$ and $\mathrm{P}_j$ can be related to the `effective standard deviation' of the estimator that estimates $\mathbb{E}[Y]$ under $\mathrm{P}_i$ using samples from $\mathrm{P}_j$. Larger the divergence, larger is the variance of the estimator.
%
%\begin{definition}\label{effectivelogdivergence}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective variance} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ to be : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}
%$\sigma^*$ is the `effective standard deviation' when arms from $[K]$ are used to estimate the means of the arms in set ${\cal R}$, under relative fractional budget $B$. We will justify this by analyzing a heterogenous importance sampling estimator and deriving confidence intervals for it in later sections.
%
%Now, we describe one of our main contributions - Algorithm \ref{alg:pickbest}.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $\nu_i$) picks the best arm.}
%  \begin{algorithmic}[1]
%    \STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
%    \STATE ${\cal R} = [K]$.
%    \STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
%    \FOR {$\ell=1$ to $n(T)$}      
%        \STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
%        \STATE \label{linesamp} Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
%        \FOR {$k \in {\cal R}$}
%    		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\ENDFOR
%	\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
%	\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
%	\IF {$\lvert {\cal R}\rvert =1$}
%	  	\STATE \textbf{return:} the arm in ${\cal R}$.
%	\ENDIF
%    \ENDFOR
%    \STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
%      \end{algorithmic}
%    \label{alg:pickbest}
%\end{algorithm}
%\textbf{Remark:}  Note that Line \ref{linesamp} uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements. We will show our algorithms outperform all other algorithms in related prior work.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
%  \begin{algorithmic}[1]
%     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line \ref{samplestamp} where all samples acquired in all the phases till that Line is used.
%    \end{algorithmic}
%   \label{alg:pickbest2}
%\end{algorithm}
%
%\subsection{Theoretical Guarantees}
%\label{sec:guarantee}
%We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first problem dependent characterization of the problem.  
%%\begin{theorem}\label{mainresult}
%%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%%\begin{equation}
%% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%%  \end{equation}
%% Here, 
%% \begin{align}
%%  \label{Hbar}
%%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%%  \end{align}
%%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%%\end{theorem}
%
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) satisfies:
%\begin{equation}
% e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
%  \end{equation}
%  when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{audibert2010best}:}
%Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result for the best arm identification with no information leakage in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}:
% \begin{equation}\label{noleakage}
%   e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)
% \end{equation}
%
% One intuitive interpretation for $\tilde{H}$ is that it is the maximum among the number of samples (neglecting some log factors) required to conclude that arm $k$ is suboptimal from among the arms which are closer to the optimal than itself. Intuitively, this is because when there is no information leakage, one requires $1/\Delta_k^2$ samples to distinguish between the $k$-th optimal arm and the optimal arm. Further, the $k$th arm is played only $1/k$ fraction of the times since we do not know the identity of the $k$-th optimal arm. 
%  
%\textbf{Interpretation of our Result:}
%Our main result in Theorem $\ref{mainresult}$ can be seen to be a generalization of the existing result in (\ref{noleakage}) for the case when there is information leakage between the arms (various changes in a causal graph).  
%
%The term $\sigma^*(B,{\cal R}^*(\Delta_k))$ in our setting is the `effective standard deviation' due to information leakage.  There is a similar interpretation of our result (ignoring the log factors): Since there is information leakage, the expression $\frac{(\sigma^*)^2}{(\Delta_k)^2}$ characterizes the number of samples required to weed out arm $k$ out of contention from among competing arms (arms that are at a distance at most twice than that of arm $k$ from the optimal arm). The interpretation of 'effective variance' is justified using importance sampling which is detailed in Section \ref{sec:estimator}. Further, in our framework $\sigma^*$ also incorporates any budget constraint that comes with the problem, i.e. any \textit{apriori} constraint on the relative fraction of times different arms need to be pulled.
%
%\textbf{Improvement over the no-information leakage case:}
%For ease of exposition let $(k)$ denote the index of the $k$-th best arm (for $k = 1,..,K$) and $\Delta_{(k)}$ denotes the corresponding gap. In this setting, the terms $\tilde{H}$ (from the result in~\cite{audibert2010best}) and $\bar{H}$ can be written as:
%\begin{align*}
%\tilde{H} &= \max_{k \neq 1} \frac{k}{\Delta_{(k)}^2} \\
%\bar{H} &= \max_{k \neq 1} \frac{\sigma^*(B,{\cal R}^*(\Delta_{(k)}))^2}{\Delta_{(k)}^2}.
%\end{align*}
%$ \sigma^*(B,{\cal R}^*(\Delta_{(k)}))$ can be smaller than $\sqrt{k}$ due to information leakage as every single arm pull contributes to another arm's estimate. Therefore, these provide better guarantees than ~\cite{audibert2010best}. 
%
%To see the improvement over the previous result in \cite{audibert2010best}, we consider a special case when the cost budget $B$ is infinity and there is only the the sample budget $T$. In addition, let us assume that the log divergences are such that: $M_{ij} \leq \eta M_{ii} = \eta << \sqrt{\lvert {\cal R}  \rvert},~ \forall i \neq j$. Let ${\cal R} = {\cal R}^*(\Delta_{(k)})$. If $\eta > \sqrt{\lvert {\cal R}  \rvert}$, the optimal solution for (\ref{mainLP1}) is a bit complicated to interpret.  Consider the feasible allocation $\nu_i = \frac{1}{\lvert {\cal R}  \rvert}, ~ \forall i \in {\cal R}$ in (\ref{mainLP1}). Evaluating the objective function for this feasible allocation, it is possible to show that $\sigma^* \leq \frac{\eta}{1-1/\lvert {\cal R}  \rvert} <<  \sqrt{\lvert {\cal R}  \rvert}$. Hence, unless the variance due to information leakage is too bad, the effective variance is smaller than that of the case with no information leakage.
%
%The improvement over the no information leakage setting, is even more pronounced under budget constraints. Consider the setting \textbf{S1}, and assume that the fractional budget of the \textit{difficult} arms, $B = o(1)$. This implies that the total number of samples available for difficult arms is $o(T)$. The budget constrained case has not been analyzed in~\cite{audibert2010best}, however in the absence of information leakage, one would expect that the arms with the least number of samples would be the most difficult to eliminate, and therefore the error guarantees would scale as $\exp(-O(BT)/\tilde{H}) \sim \exp(-o(T)/\tilde{H})$ (excluding $\log$ factors). On the other hand, our algorithm can leverage the information leakage and the error guarantee would scale as $\exp(-O(T)/\bar{H})$, which can be order-wise better if the \textit{effective standard deviations} are well-behaved. 
%
%\textbf{Remark:} Although similar advantages can be shown for \cite{lattimore2016causal}, there are no gap dependent bounds in that work and our analysis indicates a gap dependent improvement term by term with respect to \cite{audibert2010best}.
%
%
% \begin{theorem}\label{mainresult2}
%(Proved formally as Theorem \ref{thm:detailed})  Let $v^*$ be the effective inverse log divergence as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
%\ \begin{align}
%\label{eq:SRmain}
%&r(T,B) \leq  \\
%&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
%& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
% \end{align}
% Here, 
% \begin{align}
%  \label{HK}
% \bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds, which differentiates the arms according to its gap from the optimal arm and its \textit{effective standard deviation} parameter. The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$. 
%
%We defer the theoretical analysis to Section~\ref{sec:proofs}. In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we introduce the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%







==> resultsv3.tex <==
\label{sec:results}
In this section we provide our main theoretical contributions. In Section~\ref{sec:algo}, we provide a successive rejects style algorithm, that leverages the information leakage between the arms, via importance sampling. Then, we provide theoretical guarantees on the probability of mis-identification $(e(T,B))$ and simple regret $(r(T,B))$ for our algorithm in Section~\ref{sec:guarantee}. In order to explain our algorithm and our results formally, we first describe several key ideas in our algorithm and introduce definitions in Section~\ref{sec:def} that are relevant to these ideas.

\subsection{Definitions}
\label{sec:def}
%The algorithm starts by having all the $K$ arms under consideration and then proceeds in phases. At the beginning of each phase, a budget for samples is allocated to each arm. Thereafter, samples are collected according to the allocated budgets, and using these samples, importance sampling based estimators for the means of all the \textit{remaining} arms are formed. Then at the end of each phase, one or more arms are rejected based on some phase specific criterion on the estimated values. The structure of the algorithm and the estimation technique for the means of the arms,  both rely on a specific $f$-divergence between the arm distributions. 

\textbf{Quantifying Information Leakage:} We observe that
 \[\mu_k = \mathbb{E}_k[Y] = \mathbb{E}_{k'}\left[Y \frac{\mathrm{P}_k\left(V|pa(V) \right)}{\mathrm{P}_{k'}\left(V|pa(V)\right)}\right]. \] By weighing samples with the correct ratio of conditional probabilities $\mathrm{P}_k(\cdot)$ and $\mathrm{P}_{k'}(\cdot)$, it is possible to use samples under intervention $k'$ to estimate the mean under intervention $k$. However, the variance of this estimator depends on how different $\mathrm{P}_k(\cdot)$ is from $\mathrm{P}_{k}'(\cdot)$. We use a specific $f$-divergence measure between $\mathrm{P}_k(\cdot)$ is from $\mathrm{P}_{k}'(\cdot)$ to measure the difference. This $f$-divergence measure can be calculated analytically or estimated directly from empirical data (without the knowledge of the full distributions) using techniques like that of~\cite{perez2008kullback}. 

\begin{definition}
Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
\begin{align*}
D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
\end{definition}

 With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. 
 % We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
\begin{definition}
($M_{ij}$ measure)  Consider the function $f_1(x) = x \exp (x-1) - 1$. We define the following log-divergence measure:  $M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))$
%\begin{equation}
%\label{eq:mij}
%
%\end{equation}
\end{definition}
%\textbf{Remark:} We will call this log-divergence measure as the `$M_{ij}$ measure' for lack of a better descriptive name.

%One way to view the information leakage among arms is through the following expression relating the mean under arm $i$ to samples collected under arm $j$,
%\begin{align}
%\label{eq:basic_main}
%\EE_{i}\left[Y\right] = \EE_{j}\left[Y\frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))}\right]
%\end{align}
%which is trivially true as the only change in the joint distribution of all variables is at $\mathrm{P}(V \vert pa(V))$. However, directly using this expression to form an estimator, can lead to arbitrarily bad concentration as the ratio in the expression can be unbounded. Therefore, it is essential to clip the importance weighted samples at a carefully chosen value, such that we balance the trade-off between the variance of the samples and the bias incurred by the clipping. 
The quantities $M_{ij}$'s are crucial in the our analysis. 

\textbf{Aggregating Interventional Data:} Now, we describe an efficient estimator of $\EE_{k}[Y]$ ($\forall k \in [K]$) that seamlessly combines available samples from different arms. This estimator uses variable weights depending on the relative $M_{ij}$ measures and also  uses clipping to control variance by introducing bias. The estimator is given by (\ref{eq:uniestimator_main}).

Suppose we obtain $\tau_{i}$ samples from arm $i \in [K]$. Let the total number of samples from all arms put together be $\tau$. Let us index all the samples by $s \in \{1,2,..,\tau \}$. Let $\mathcal{T}_{k} \subset \{1,2,..,\tau \}$ be the indices of all the samples collected from arm $k$. Further, let $Z_k = \sum_{j \in [K]}\tau_j/M_{kj}$. Now, we are at the position to introduce the estimator for $\mu_k$, which we will denoted by $\hat{Y}_{k}^{\epsilon}$ ($\epsilon$ is an indicator of the level of confidence desired):
\begin{align*}
\label{eq:uniestimator_main}
&\hat{Y}_{k}^{\epsilon}  = \frac{1}{Z_{k}}\sum_{j = 0}^{K} \sum_{s \in \mathcal{T}_j} \frac{1}{M_{kj}}Y_j(s)\frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \times
\\
&\mathds{1}\left\{ \frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \leq 2\log(2/\epsilon)M_{kj}\right\}. \numberthis
\end{align*}
In other words, $\hat{Y}_{k}^{\epsilon}$ is the weighted average of the clipped samples, where the samples from arm $j$ are weighted by $1/M_{kj}$ and clipped at $ 2\log(2/\epsilon)M_{kj}$. The \textbf{choice of $\epsilon$} controls the \textit{bias-variance tradeoff} which we will adaptively change in our full algorithm.

\textbf{Effective Deviation:} Consider the following estimation problem - With a budget of $\tau$ samples, estimate $\mathbb{E}_k[Y]$ for all $k \in {\cal R}$ (set of arms not rejected). We first characterize the variance of estimators based on (\ref{eq:uniestimator_main}). Suppose a budget of $\tau$ samples has been allocated among arms in $[K]$ to estimate arms in a subset ${\cal R}$. Let the fraction of samples allocated to arm $k$ be $\nu_k$. Then, $\tau_i=\nu_i\times\tau$. Let $\pmb{\nu}=\left[\nu_1 \ldots \nu_K \right]^T$. Then, we define the effective standard deviation of the allocation as:

\begin{definition}\label{effectiveallocation}
Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective standard deviation} $\sigma^*(\pmb{\nu},{\cal R})$ for {\bf allocation $\pmb{\nu}$}  and arm set ${\cal R} \subseteq [K] $ to be : 
    %\begin{align}
%\label{mainLP2}
$\frac{1}{\sigma^*(\pmb{\nu},{\cal R})} = v^*(\pmb{\nu},{\cal R}) =\min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k}$ 
%\end{align}
\end{definition}
\textbf{Remark:} Formally the minimum standard deviation of the set of estimators of the form (\ref{eq:uniestimator_main}) applied to estimating the means of arm-set ${\cal R}$ is given by Definition \ref{effectiveallocation} (Lemma \ref{allocation} in the appendix).

\textbf{Allocation of Budget:} The above definition provides a handle on the effective variance on estimators of the form~(\ref{eq:uniestimator_main}) given an allocation of budget $\pmb{\nu}$. However, the choice of the allocation (while adhering to budget constraints) is in the hands of the algorithm designer. We design a sub-routine Algorithm~\ref{alg:allocate} (in the appendix) that allocates the samples, such that the worst estimator in (\ref{eq:uniestimator_main}) for arms amongst ${\cal R}$ is as  \textit{good} (quantified in Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the appendix) as possible. The target effective deviation of the worst estimator is:
\begin{definition}\label{effectivelogdivergence}
The \textbf{effective standard deviation} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ is defined as : 
    \begin{align}
\label{mainLP1}
&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} v^*(\pmb{\nu},{\cal R})   \\
 &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
\end{align}
\end{definition}


\subsection{Algorithm}
Now, we describe our main algorithmic contributions - Algorithm \ref{alg:pickbest} and \ref{alg:pickbest2}.  Algorithm \ref{alg:pickbest}  starts by having all the $K$ arms under consideration and then proceeds in phases. The total number of phases is fixed apriori. At every phase, the algorithm chooses the $\epsilon$ parameter (i.e. the bias variance trade-off) and the allocates the phase budget to optimize the effective deviation ( Definition \ref{effectivelogdivergence}). Estimator $(\ref{eq:uniestimator_main})$ is applied to every arm under consideration with these parameters. Using a phase specific threshold, some arms are rejected on the basis of these estimates. Any one of the remaining arms is randomly declared to be the optimal at the end. The only difference between Algorithms~\ref{alg:pickbest} and \ref{alg:pickbest2} is that the former only uses the samples obtained in the current phase while the latter reuses the past samples. After defining the phase budgets and the number of phases, we formally describe the main algorithms:

\begin{algorithm}
	\caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $c_i$'s) picks the best arm.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
		\STATE ${\cal R} = [K]$.
		\STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
		\FOR {$\ell=1$ to $n(T)$}      
		\STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
		\STATE Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
		\FOR {$k \in {\cal R}$}
		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator_main}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line 6.	\ENDFOR
		\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
		\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
		\IF {$\lvert {\cal R}\rvert =1$}
		\STATE \textbf{return:} the arm in ${\cal R}$.
		\ENDIF
		\ENDFOR
		\STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
	\end{algorithmic}
	\label{alg:pickbest}
\end{algorithm}

 $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 


 We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set $\tau(l) = T/(l\overline{\log}(n(T)))$ for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. So, we have $T(l)= (T \overline{\log}(l))/(\overline{\log}(n(T)))$. Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.


\begin{remark}  Note that Line 6 uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements.
\end{remark}
\begin{algorithm}
  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
  \begin{algorithmic}[1]
     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line 6 where all samples acquired in all the phases till that Line is used.
    \end{algorithmic}
   \label{alg:pickbest2}
\end{algorithm}
\label{sec:algo}
\subsection{Theoretical Guarantees}
\label{sec:guarantee}
We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first gap dependent characterization.  
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%\begin{equation}
% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%  \end{equation}
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}

\begin{theorem}\label{mainresult}
	(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The probability of error for  Algorithm \ref{alg:pickbest} satisfies:
	\begin{equation}
	e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
	\end{equation}
	when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
	Here, 
	\begin{align}
	\label{Hbar}
	\bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison with the result in \cite{audibert2010best}:}
Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}: $e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)$. 

Our work is analogous to the above result (upto poly log factors) except that $\bar{H}$ appears instead of $\tilde{H}$. In Section~\ref{sec:compare1} (in the appendix), we demonstrate through simple examples that $\sigma^*(B,{\cal R}^*(\Delta_k))$ can be significantly smaller than $\sqrt{\tilde{\mathcal{R}}(\Delta_k)}$ (the corresponding term in $e(T)$ above) even when there are no average budget constraints. Moreover, our results can be exponentially better in the presence of average budget constraints (examples in Section~\ref{sec:compare1}). Now we present our bounds on simple regret in Theorem~\ref{mainresult2}.

\begin{theorem}\label{mainresult2}
	(Proved formally as Theorem \ref{thm:detailed})  Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
	\ \begin{align}
	\label{eq:SRmain}
	&r(T,B) \leq   \nonumber\\
	&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
	& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
	\end{align}
	Here, 
	\begin{align}
	\label{HK}
	\bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison with the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the simple regret scales as $O(1/\sqrt{T})$ and do not adapt to the gaps. We provide gap dependent bounds that can be exponentially better than that of~\cite{lattimore2016causal}. More over our bounds generalize to gap independent bounds that match $O(1/\sqrt{T})$. Further details are provided in Section~\ref{sec:compare2} (in the appendix).

%In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds. %The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. 
%It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$ and can handle general constraints on average budgets. Further details are provided in Section~\ref{sec:compare2}. 

We defer the theoretical analysis to Section~\ref{sec:proofs}. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we analyze the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 




























%\subsection{An Efficient Algorithm}\label{sec:algo}
%%We present two versions of \textit{successive rejects} style strategies, that attain the theoretical guarantees detailed in Section~\ref{sec:results}. Both the algorithms proceed in phases, successively rejecting arms at the end of each phase, until we are left with the optimal arm (provided $\Delta_{k} \geq 1/\sqrt{T}$ for all $k \in [K]$, otherwise it outputs a set of arms with $\Delta_k < 1/\sqrt{T}$). The only difference between Algorithms~\ref{algo:one} and \ref{algo:two} is that Algorithm~\ref{algo:one} only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while Algorithm~\ref{algo:two} reuses the past samples. 
%We present a successive rejects style algorithm that leverages the information leakage among the arms, through importance sampling. The algorithm proceeds in phases. The algorithm starts with all the arms under consideration, and rejects zero or more arms at the end of each phase successively, until we are left with only the best arm or possibly a few arms which are \textit{very} close to the best arm.  Let us define some notation that is helpful in describing the main algorithm:
%\begin{enumerate}
%\item $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 
%\item We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set,
%\begin{align}
%\tau(l) &= \frac{T}{\overline{\log}(n(T)) l} \label{taueq}\\
%\end{align}
%for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. Also, we have 
%\begin{equation}\label{timeatphase}
%T(l)= \frac{T \overline{\log}(l)}{\overline{\log}(n(T))}.
%\end{equation}
%\item Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.
%\end{enumerate}
%
%Although, we assume that $\mathrm{P}_k \left( V \vert pa(V) \right)$ and the marginal distribution $pa(V)$ are known, the algorithm we describe needs certain pairwise $f$-divergence values between these conditionals $\mathrm{P}_k$. The $f$-divergences can be calculated from the known distributions or estimated directly from data. Now we define the $f$- divergences that are required. 
%
%\subsubsection{Pairwise $f$- divergences}\label{f-div}
%\begin{definition}
%Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
%\begin{align*}
%D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
%\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
%\end{definition}
%
% With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by the shorthand $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. Consider the function $f_1(x) = x \exp (x-1) - 1$. We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
%
%For notational convenience, let us define log divergence to be:
%\begin{equation}
%\label{eq:mij}
%M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))
%\end{equation}
%
%The divergence measure $M_{ij}$ between $\mathrm{P}_i$ and $\mathrm{P}_j$ can be related to the `effective standard deviation' of the estimator that estimates $\mathbb{E}[Y]$ under $\mathrm{P}_i$ using samples from $\mathrm{P}_j$. Larger the divergence, larger is the variance of the estimator.
%
%\begin{definition}\label{effectivelogdivergence}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective variance} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ to be : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}
%$\sigma^*$ is the `effective standard deviation' when arms from $[K]$ are used to estimate the means of the arms in set ${\cal R}$, under relative fractional budget $B$. We will justify this by analyzing a heterogenous importance sampling estimator and deriving confidence intervals for it in later sections.
%
%Now, we describe one of our main contributions - Algorithm \ref{alg:pickbest}.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $\nu_i$) picks the best arm.}
%  \begin{algorithmic}[1]
%    \STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
%    \STATE ${\cal R} = [K]$.
%    \STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
%    \FOR {$\ell=1$ to $n(T)$}      
%        \STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
%        \STATE \label{linesamp} Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
%        \FOR {$k \in {\cal R}$}
%    		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\ENDFOR
%	\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
%	\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
%	\IF {$\lvert {\cal R}\rvert =1$}
%	  	\STATE \textbf{return:} the arm in ${\cal R}$.
%	\ENDIF
%    \ENDFOR
%    \STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
%      \end{algorithmic}
%    \label{alg:pickbest}
%\end{algorithm}
%\textbf{Remark:}  Note that Line \ref{linesamp} uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements. We will show our algorithms outperform all other algorithms in related prior work.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
%  \begin{algorithmic}[1]
%     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line \ref{samplestamp} where all samples acquired in all the phases till that Line is used.
%    \end{algorithmic}
%   \label{alg:pickbest2}
%\end{algorithm}
%
%\subsection{Theoretical Guarantees}
%\label{sec:guarantee}
%We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first problem dependent characterization of the problem.  
%%\begin{theorem}\label{mainresult}
%%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%%\begin{equation}
%% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%%  \end{equation}
%% Here, 
%% \begin{align}
%%  \label{Hbar}
%%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%%  \end{align}
%%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%%\end{theorem}
%
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) satisfies:
%\begin{equation}
% e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
%  \end{equation}
%  when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{audibert2010best}:}
%Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result for the best arm identification with no information leakage in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}:
% \begin{equation}\label{noleakage}
%   e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)
% \end{equation}
%
% One intuitive interpretation for $\tilde{H}$ is that it is the maximum among the number of samples (neglecting some log factors) required to conclude that arm $k$ is suboptimal from among the arms which are closer to the optimal than itself. Intuitively, this is because when there is no information leakage, one requires $1/\Delta_k^2$ samples to distinguish between the $k$-th optimal arm and the optimal arm. Further, the $k$th arm is played only $1/k$ fraction of the times since we do not know the identity of the $k$-th optimal arm. 
%  
%\textbf{Interpretation of our Result:}
%Our main result in Theorem $\ref{mainresult}$ can be seen to be a generalization of the existing result in (\ref{noleakage}) for the case when there is information leakage between the arms (various changes in a causal graph).  
%
%The term $\sigma^*(B,{\cal R}^*(\Delta_k))$ in our setting is the `effective standard deviation' due to information leakage.  There is a similar interpretation of our result (ignoring the log factors): Since there is information leakage, the expression $\frac{(\sigma^*)^2}{(\Delta_k)^2}$ characterizes the number of samples required to weed out arm $k$ out of contention from among competing arms (arms that are at a distance at most twice than that of arm $k$ from the optimal arm). The interpretation of 'effective variance' is justified using importance sampling which is detailed in Section \ref{sec:estimator}. Further, in our framework $\sigma^*$ also incorporates any budget constraint that comes with the problem, i.e. any \textit{apriori} constraint on the relative fraction of times different arms need to be pulled.
%
%\textbf{Improvement over the no-information leakage case:}
%For ease of exposition let $(k)$ denote the index of the $k$-th best arm (for $k = 1,..,K$) and $\Delta_{(k)}$ denotes the corresponding gap. In this setting, the terms $\tilde{H}$ (from the result in~\cite{audibert2010best}) and $\bar{H}$ can be written as:
%\begin{align*}
%\tilde{H} &= \max_{k \neq 1} \frac{k}{\Delta_{(k)}^2} \\
%\bar{H} &= \max_{k \neq 1} \frac{\sigma^*(B,{\cal R}^*(\Delta_{(k)}))^2}{\Delta_{(k)}^2}.
%\end{align*}
%$ \sigma^*(B,{\cal R}^*(\Delta_{(k)}))$ can be smaller than $\sqrt{k}$ due to information leakage as every single arm pull contributes to another arm's estimate. Therefore, these provide better guarantees than ~\cite{audibert2010best}. 
%
%To see the improvement over the previous result in \cite{audibert2010best}, we consider a special case when the cost budget $B$ is infinity and there is only the the sample budget $T$. In addition, let us assume that the log divergences are such that: $M_{ij} \leq \eta M_{ii} = \eta << \sqrt{\lvert {\cal R}  \rvert},~ \forall i \neq j$. Let ${\cal R} = {\cal R}^*(\Delta_{(k)})$. If $\eta > \sqrt{\lvert {\cal R}  \rvert}$, the optimal solution for (\ref{mainLP1}) is a bit complicated to interpret.  Consider the feasible allocation $\nu_i = \frac{1}{\lvert {\cal R}  \rvert}, ~ \forall i \in {\cal R}$ in (\ref{mainLP1}). Evaluating the objective function for this feasible allocation, it is possible to show that $\sigma^* \leq \frac{\eta}{1-1/\lvert {\cal R}  \rvert} <<  \sqrt{\lvert {\cal R}  \rvert}$. Hence, unless the variance due to information leakage is too bad, the effective variance is smaller than that of the case with no information leakage.
%
%The improvement over the no information leakage setting, is even more pronounced under budget constraints. Consider the setting \textbf{S1}, and assume that the fractional budget of the \textit{difficult} arms, $B = o(1)$. This implies that the total number of samples available for difficult arms is $o(T)$. The budget constrained case has not been analyzed in~\cite{audibert2010best}, however in the absence of information leakage, one would expect that the arms with the least number of samples would be the most difficult to eliminate, and therefore the error guarantees would scale as $\exp(-O(BT)/\tilde{H}) \sim \exp(-o(T)/\tilde{H})$ (excluding $\log$ factors). On the other hand, our algorithm can leverage the information leakage and the error guarantee would scale as $\exp(-O(T)/\bar{H})$, which can be order-wise better if the \textit{effective standard deviations} are well-behaved. 
%
%\textbf{Remark:} Although similar advantages can be shown for \cite{lattimore2016causal}, there are no gap dependent bounds in that work and our analysis indicates a gap dependent improvement term by term with respect to \cite{audibert2010best}.
%
%
% \begin{theorem}\label{mainresult2}
%(Proved formally as Theorem \ref{thm:detailed})  Let $v^*$ be the effective inverse log divergence as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
%\ \begin{align}
%\label{eq:SRmain}
%&r(T,B) \leq  \\
%&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
%& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
% \end{align}
% Here, 
% \begin{align}
%  \label{HK}
% \bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds, which differentiates the arms according to its gap from the optimal arm and its \textit{effective standard deviation} parameter. The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$. 
%
%We defer the theoretical analysis to Section~\ref{sec:proofs}. In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we introduce the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%







==> resultsv4.tex <==
\label{sec:results}
In this section we provide our main theoretical contributions. In Section~\ref{sec:algo}, we provide a successive rejects style algorithm, that leverages the information leakage between the arms, via importance sampling. Then, we provide theoretical guarantees on the probability of mis-identification $(e(T,B))$ and simple regret $(r(T,B))$ for our algorithm in Section~\ref{sec:guarantee}. In order to explain our algorithm and our results formally, we first describe several key ideas in our algorithm and introduce definitions in Section~\ref{sec:def} that are relevant to these ideas.

\subsection{Definitions}
\label{sec:def}
%The algorithm starts by having all the $K$ arms under consideration and then proceeds in phases. At the beginning of each phase, a budget for samples is allocated to each arm. Thereafter, samples are collected according to the allocated budgets, and using these samples, importance sampling based estimators for the means of all the \textit{remaining} arms are formed. Then at the end of each phase, one or more arms are rejected based on some phase specific criterion on the estimated values. The structure of the algorithm and the estimation technique for the means of the arms,  both rely on a specific $f$-divergence between the arm distributions. 

\textbf{Quantifying Information Leakage:} We observe that
 \[\mu_k = \mathbb{E}_k[Y] = \mathbb{E}_{k'}\left[Y \frac{\mathrm{P}_k\left(V|pa(V) \right)}{\mathrm{P}_{k'}\left(V|pa(V)\right)}\right]. \] By weighing samples with the correct ratio of conditional probabilities $\mathrm{P}_k(\cdot)$ and $\mathrm{P}_{k'}(\cdot)$, it is possible to use samples under intervention $k'$ to estimate the mean under intervention $k$. However, the variance of this estimator depends on how different $\mathrm{P}_k(\cdot)$ is from $\mathrm{P}_{k}'(\cdot)$. We use a specific $f$-divergence measure between $\mathrm{P}_k(\cdot)$ is from $\mathrm{P}_{k}'(\cdot)$ to measure the difference. This $f$-divergence measure can be calculated analytically or estimated directly from empirical data (without the knowledge of the full distributions) using techniques like that of~\cite{perez2008kullback}. 

\begin{definition}
Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
\begin{align*}
D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
\end{definition}

 With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. 
 % We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
\begin{definition}
	\label{def:mij}
($M_{ij}$ measure)  Consider the function $f_1(x) = x \exp (x-1) - 1$. We define the following log-divergence measure:  $M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))$
%\begin{equation}
%\label{eq:mij}
%
%\end{equation}
\end{definition}
%\textbf{Remark:} We will call this log-divergence measure as the `$M_{ij}$ measure' for lack of a better descriptive name.

%One way to view the information leakage among arms is through the following expression relating the mean under arm $i$ to samples collected under arm $j$,
%\begin{align}
%\label{eq:basic_main}
%\EE_{i}\left[Y\right] = \EE_{j}\left[Y\frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))}\right]
%\end{align}
%which is trivially true as the only change in the joint distribution of all variables is at $\mathrm{P}(V \vert pa(V))$. However, directly using this expression to form an estimator, can lead to arbitrarily bad concentration as the ratio in the expression can be unbounded. Therefore, it is essential to clip the importance weighted samples at a carefully chosen value, such that we balance the trade-off between the variance of the samples and the bias incurred by the clipping. 
The quantities $M_{ij}$'s are crucial in the our analysis. 

\textbf{Aggregating Interventional Data:} Now, we describe an efficient estimator of $\EE_{k}[Y]$ ($\forall k \in [K]$) that seamlessly combines available samples from different arms. This estimator uses variable weights depending on the relative $M_{ij}$ measures and also  uses clipping to control variance by introducing bias. The estimator is given by (\ref{eq:uniestimator_main}).

Suppose we obtain $\tau_{i}$ samples from arm $i \in [K]$. Let the total number of samples from all arms put together be $\tau$. Let us index all the samples by $s \in \{1,2,..,\tau \}$. Let $\mathcal{T}_{k} \subset \{1,2,..,\tau \}$ be the indices of all the samples collected from arm $k$. Further, let $Z_k = \sum_{j \in [K]}\tau_j/M_{kj}$. Now, we are at the position to introduce the estimator for $\mu_k$, which we will denoted by $\hat{Y}_{k}^{\epsilon}$ ($\epsilon$ is an indicator of the level of confidence desired):
\begin{align*}
\label{eq:uniestimator_main}
&\hat{Y}_{k}^{\epsilon}  = \frac{1}{Z_{k}}\sum_{j = 0}^{K} \sum_{s \in \mathcal{T}_j} \frac{1}{M_{kj}}Y_j(s)\frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \times
\\
&\mathds{1}\left\{ \frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \leq 2\log(2/\epsilon)M_{kj}\right\}. \numberthis
\end{align*}
In other words, $\hat{Y}_{k}^{\epsilon}$ is the weighted average of the clipped samples, where the samples from arm $j$ are weighted by $1/M_{kj}$ and clipped at $ 2\log(2/\epsilon)M_{kj}$. The \textbf{choice of $\epsilon$} controls the \textit{bias-variance tradeoff} which we will adaptively change in our full algorithm. 

%\textbf{Effective Deviation:} Consider the following estimation problem - With a budget of $\tau$ samples, estimate $\mathbb{E}_k[Y]$ for all $k \in {\cal R}$ (set of arms not rejected). We first characterize the variance of estimators based on (\ref{eq:uniestimator_main}). Suppose a budget of $\tau$ samples has been allocated among arms in $[K]$ to estimate arms in a subset ${\cal R}$. Let the fraction of samples allocated to arm $k$ be $\nu_k$. Then, $\tau_i=\nu_i\times\tau$. Let $\pmb{\nu}=\left[\nu_1 \ldots \nu_K \right]^T$. Then, we define the effective standard deviation of the allocation as:
%
%\begin{definition}\label{effectiveallocation}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective standard deviation} $\sigma^*(\pmb{\nu},{\cal R})$ for {\bf allocation $\pmb{\nu}$}  and arm set ${\cal R} \subseteq [K] $ to be : 
%    %\begin{align}
%%\label{mainLP2}
%$\frac{1}{\sigma^*(\pmb{\nu},{\cal R})} = v^*(\pmb{\nu},{\cal R}) =\min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k}$ 
%%\end{align}
%\end{definition}
%\textbf{Remark:} Formally the minimum standard deviation of the set of estimators of the form (\ref{eq:uniestimator_main}) applied to estimating the means of arm-set ${\cal R}$ is given by Definition \ref{effectiveallocation} (Lemma \ref{allocation} in the appendix).
%
%\textbf{Allocation of Budget:} The above definition provides a handle on the effective variance on estimators of the form~(\ref{eq:uniestimator_main}) given an allocation of budget $\pmb{\nu}$. However, the choice of the allocation (while adhering to budget constraints) is in the hands of the algorithm designer. We design a sub-routine Algorithm~\ref{alg:allocate} (in the appendix) that allocates the samples, such that the worst estimator in (\ref{eq:uniestimator_main}) for arms amongst ${\cal R}$ is as  \textit{good} (quantified in Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the appendix) as possible. The target effective deviation of the worst estimator is:
%\begin{definition}\label{effectivelogdivergence}
%The \textbf{effective standard deviation} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ is defined as : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} v^*(\pmb{\nu},{\cal R})   \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}


\subsection{Algorithm}
Now, we describe our main algorithmic contributions - Algorithm \ref{alg:pickbest} and \ref{alg:pickbest2}.  Algorithm \ref{alg:pickbest}  starts by having all the $K$ arms under consideration and then proceeds in phases, rejecting one or more arms at the end of each phase. 

Recall the parameters $T$ -  Total sample budget available and $B$ - average cost budget constraint. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$.  We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$. We set $\tau(l) = T/(l\overline{\log}(n(T)))$ for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.

Let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$. The vector $\pmb{\tau(\ell)}$ which encodes the sample budget for each arm in a phase is decided by Algorithm~\ref{alg:allocate}. The allocation is crucial for improving the performance of the estimators. For example an arm that provides sufficient information about all the remaining arms needs to be given more budget than another arm which has high divergences from the remaining arms. This allocation depends on the average budget constraints and the relative log divergences between the arms (Definition~\ref{def:mij}). Algorithm~\ref{alg:allocate} ensures that the worst estimator (of the form (\ref{eq:uniestimator_main})) for the arms in $\mathcal{R}$ is as \textit{good} as possible (quantified in Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the appendix). 

Estimator $(\ref{eq:uniestimator_main})$ with a phase specific choice of  the $\epsilon$ parameter (i.e. the bias variance trade-off), is applied to every arm under consideration . Using a phase specific threshold, some arms are rejected on the basis of these estimates, at the end of each phase. Any one of the arms surviving at the end of \textit{all} phases is randomly declared to be the optimal.

\begin{algorithm}
	\caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $c_i$'s) picks the best arm.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
		\STATE ${\cal R} = [K]$.
		\STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
		\FOR {$\ell=1$ to $n(T)$}      
		\STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
		\STATE Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
		\FOR {$k \in {\cal R}$}
		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator_main}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line 6.	\ENDFOR
		\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
		\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
		\IF {$\lvert {\cal R}\rvert =1$}
		\STATE \textbf{return:} the arm in ${\cal R}$.
		\ENDIF
		\ENDFOR
		\STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
	\end{algorithmic}
	\label{alg:pickbest}
\end{algorithm}


\begin{remark}  Note that Line 6 uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements.
\end{remark}

\begin{algorithm}
  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
  \begin{algorithmic}[1]
     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line 6 where all samples acquired in all the phases till that Line is used.
    \end{algorithmic}
   \label{alg:pickbest2}
\end{algorithm}
\label{sec:algo}

The inverse of the maximal objective of the LP in Algorithm~\ref{alg:allocate} acts as \textit{effective standard deviation} terms for the estimators for the remaining arms in $\mathcal{R}$. It is analogous to the variance terms appearing in the confidence bounds of these estimators similar to Bernstien's bound (refer to Lemma~\ref{allocation} in the appendix).

\begin{definition}\label{effectivelogdivergence}
The \textbf{effective standard deviation} for budget $B$ and arm set ${\cal R} \subseteq [K] $ is defined as ${\sigma^*(B,{\cal R})} = 1/v^*(B,{\cal R})$ from Algorithm~\ref{alg:allocate} with input $B$ and arm set ${\cal R}$.
\end{definition}

\begin{algorithm}
	\caption{Allocate - Allocates a given budget $\tau$ among the arms to reduce variance.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{Allocate}(\mathbf{c},B,\mathbf{A},{\cal R},\tau)$
		\STATE Solve the following LP: 
		\begin{align}
		\label{mainLP1}
		\frac{1}{\sigma^*(B,{\cal R})} &= v^*(B,{\cal R}) =  \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
		&\text{s.t.~} \sum_{i=0}^K c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K} \nu_j = 1, ~\nu_i \geq 0. \nonumber
		\end{align}
		\STATE Assign $\tau_j = \nu_j^*(B,{\cal R})\tau $
	\end{algorithmic}
	\label{alg:allocate}
\end{algorithm}
\subsection{Theoretical Guarantees}
\label{sec:guarantee}
We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first gap dependent characterization.  
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%\begin{equation}
% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%  \end{equation}
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}

\begin{theorem}\label{mainresult}
	(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The probability of error for  Algorithm \ref{alg:pickbest} satisfies:
	\begin{equation}
	e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
	\end{equation}
	when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
	Here, 
	\begin{align}
	\label{Hbar}
	\bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison with the result in \cite{audibert2010best}:}
Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}: $e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)$. 

Our work is analogous to the above result (upto poly log factors) except that $\bar{H}$ appears instead of $\tilde{H}$. In Section~\ref{sec:compare1} (in the appendix), we demonstrate through simple examples that $\sigma^*(B,{\cal R}^*(\Delta_k))$ can be significantly smaller than $\sqrt{\tilde{\mathcal{R}}(\Delta_k)}$ (the corresponding term in $e(T)$ above) even when there are no average budget constraints. Moreover, our results can be exponentially better in the presence of average budget constraints (examples in Section~\ref{sec:compare1}). Now we present our bounds on simple regret in Theorem~\ref{mainresult2}.

\begin{theorem}\label{mainresult2}
	(Proved formally as Theorem \ref{thm:detailed})  Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
	\ \begin{align}
	\label{eq:SRmain}
	&r(T,B) \leq   \nonumber\\
	&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
	& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
	\end{align}
	Here, 
	\begin{align}
	\label{HK}
	\bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison with the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the simple regret scales as $O(1/\sqrt{T})$ and do not adapt to the gaps. We provide gap dependent bounds that can be exponentially better than that of~\cite{lattimore2016causal}. More over our bounds generalize to gap independent bounds that match $O(1/\sqrt{T})$. Further details are provided in Section~\ref{sec:compare2} (in the appendix).

%In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds. %The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. 
%It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$ and can handle general constraints on average budgets. Further details are provided in Section~\ref{sec:compare2}. 

We defer the theoretical analysis to Section~\ref{sec:proofs}. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we analyze the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 




























%\subsection{An Efficient Algorithm}\label{sec:algo}
%%We present two versions of \textit{successive rejects} style strategies, that attain the theoretical guarantees detailed in Section~\ref{sec:results}. Both the algorithms proceed in phases, successively rejecting arms at the end of each phase, until we are left with the optimal arm (provided $\Delta_{k} \geq 1/\sqrt{T}$ for all $k \in [K]$, otherwise it outputs a set of arms with $\Delta_k < 1/\sqrt{T}$). The only difference between Algorithms~\ref{algo:one} and \ref{algo:two} is that Algorithm~\ref{algo:one} only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while Algorithm~\ref{algo:two} reuses the past samples. 
%We present a successive rejects style algorithm that leverages the information leakage among the arms, through importance sampling. The algorithm proceeds in phases. The algorithm starts with all the arms under consideration, and rejects zero or more arms at the end of each phase successively, until we are left with only the best arm or possibly a few arms which are \textit{very} close to the best arm.  Let us define some notation that is helpful in describing the main algorithm:
%\begin{enumerate}
%\item $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 
%\item We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set,
%\begin{align}
%\tau(l) &= \frac{T}{\overline{\log}(n(T)) l} \label{taueq}\\
%\end{align}
%for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. Also, we have 
%\begin{equation}\label{timeatphase}
%T(l)= \frac{T \overline{\log}(l)}{\overline{\log}(n(T))}.
%\end{equation}
%\item Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.
%\end{enumerate}
%
%Although, we assume that $\mathrm{P}_k \left( V \vert pa(V) \right)$ and the marginal distribution $pa(V)$ are known, the algorithm we describe needs certain pairwise $f$-divergence values between these conditionals $\mathrm{P}_k$. The $f$-divergences can be calculated from the known distributions or estimated directly from data. Now we define the $f$- divergences that are required. 
%
%\subsubsection{Pairwise $f$- divergences}\label{f-div}
%\begin{definition}
%Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
%\begin{align*}
%D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
%\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
%\end{definition}
%
% With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by the shorthand $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. Consider the function $f_1(x) = x \exp (x-1) - 1$. We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
%
%For notational convenience, let us define log divergence to be:
%\begin{equation}
%\label{eq:mij}
%M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))
%\end{equation}
%
%The divergence measure $M_{ij}$ between $\mathrm{P}_i$ and $\mathrm{P}_j$ can be related to the `effective standard deviation' of the estimator that estimates $\mathbb{E}[Y]$ under $\mathrm{P}_i$ using samples from $\mathrm{P}_j$. Larger the divergence, larger is the variance of the estimator.
%
%\begin{definition}\label{effectivelogdivergence}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective variance} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ to be : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}
%$\sigma^*$ is the `effective standard deviation' when arms from $[K]$ are used to estimate the means of the arms in set ${\cal R}$, under relative fractional budget $B$. We will justify this by analyzing a heterogenous importance sampling estimator and deriving confidence intervals for it in later sections.
%
%Now, we describe one of our main contributions - Algorithm \ref{alg:pickbest}.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $\nu_i$) picks the best arm.}
%  \begin{algorithmic}[1]
%    \STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
%    \STATE ${\cal R} = [K]$.
%    \STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
%    \FOR {$\ell=1$ to $n(T)$}      
%        \STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
%        \STATE \label{linesamp} Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
%        \FOR {$k \in {\cal R}$}
%    		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\ENDFOR
%	\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
%	\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
%	\IF {$\lvert {\cal R}\rvert =1$}
%	  	\STATE \textbf{return:} the arm in ${\cal R}$.
%	\ENDIF
%    \ENDFOR
%    \STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
%      \end{algorithmic}
%    \label{alg:pickbest}
%\end{algorithm}
%\textbf{Remark:}  Note that Line \ref{linesamp} uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements. We will show our algorithms outperform all other algorithms in related prior work.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
%  \begin{algorithmic}[1]
%     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line \ref{samplestamp} where all samples acquired in all the phases till that Line is used.
%    \end{algorithmic}
%   \label{alg:pickbest2}
%\end{algorithm}
%
%\subsection{Theoretical Guarantees}
%\label{sec:guarantee}
%We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first problem dependent characterization of the problem.  
%%\begin{theorem}\label{mainresult}
%%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%%\begin{equation}
%% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%%  \end{equation}
%% Here, 
%% \begin{align}
%%  \label{Hbar}
%%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%%  \end{align}
%%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%%\end{theorem}
%
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) satisfies:
%\begin{equation}
% e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
%  \end{equation}
%  when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{audibert2010best}:}
%Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result for the best arm identification with no information leakage in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}:
% \begin{equation}\label{noleakage}
%   e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)
% \end{equation}
%
% One intuitive interpretation for $\tilde{H}$ is that it is the maximum among the number of samples (neglecting some log factors) required to conclude that arm $k$ is suboptimal from among the arms which are closer to the optimal than itself. Intuitively, this is because when there is no information leakage, one requires $1/\Delta_k^2$ samples to distinguish between the $k$-th optimal arm and the optimal arm. Further, the $k$th arm is played only $1/k$ fraction of the times since we do not know the identity of the $k$-th optimal arm. 
%  
%\textbf{Interpretation of our Result:}
%Our main result in Theorem $\ref{mainresult}$ can be seen to be a generalization of the existing result in (\ref{noleakage}) for the case when there is information leakage between the arms (various changes in a causal graph).  
%
%The term $\sigma^*(B,{\cal R}^*(\Delta_k))$ in our setting is the `effective standard deviation' due to information leakage.  There is a similar interpretation of our result (ignoring the log factors): Since there is information leakage, the expression $\frac{(\sigma^*)^2}{(\Delta_k)^2}$ characterizes the number of samples required to weed out arm $k$ out of contention from among competing arms (arms that are at a distance at most twice than that of arm $k$ from the optimal arm). The interpretation of 'effective variance' is justified using importance sampling which is detailed in Section \ref{sec:estimator}. Further, in our framework $\sigma^*$ also incorporates any budget constraint that comes with the problem, i.e. any \textit{apriori} constraint on the relative fraction of times different arms need to be pulled.
%
%\textbf{Improvement over the no-information leakage case:}
%For ease of exposition let $(k)$ denote the index of the $k$-th best arm (for $k = 1,..,K$) and $\Delta_{(k)}$ denotes the corresponding gap. In this setting, the terms $\tilde{H}$ (from the result in~\cite{audibert2010best}) and $\bar{H}$ can be written as:
%\begin{align*}
%\tilde{H} &= \max_{k \neq 1} \frac{k}{\Delta_{(k)}^2} \\
%\bar{H} &= \max_{k \neq 1} \frac{\sigma^*(B,{\cal R}^*(\Delta_{(k)}))^2}{\Delta_{(k)}^2}.
%\end{align*}
%$ \sigma^*(B,{\cal R}^*(\Delta_{(k)}))$ can be smaller than $\sqrt{k}$ due to information leakage as every single arm pull contributes to another arm's estimate. Therefore, these provide better guarantees than ~\cite{audibert2010best}. 
%
%To see the improvement over the previous result in \cite{audibert2010best}, we consider a special case when the cost budget $B$ is infinity and there is only the the sample budget $T$. In addition, let us assume that the log divergences are such that: $M_{ij} \leq \eta M_{ii} = \eta << \sqrt{\lvert {\cal R}  \rvert},~ \forall i \neq j$. Let ${\cal R} = {\cal R}^*(\Delta_{(k)})$. If $\eta > \sqrt{\lvert {\cal R}  \rvert}$, the optimal solution for (\ref{mainLP1}) is a bit complicated to interpret.  Consider the feasible allocation $\nu_i = \frac{1}{\lvert {\cal R}  \rvert}, ~ \forall i \in {\cal R}$ in (\ref{mainLP1}). Evaluating the objective function for this feasible allocation, it is possible to show that $\sigma^* \leq \frac{\eta}{1-1/\lvert {\cal R}  \rvert} <<  \sqrt{\lvert {\cal R}  \rvert}$. Hence, unless the variance due to information leakage is too bad, the effective variance is smaller than that of the case with no information leakage.
%
%The improvement over the no information leakage setting, is even more pronounced under budget constraints. Consider the setting \textbf{S1}, and assume that the fractional budget of the \textit{difficult} arms, $B = o(1)$. This implies that the total number of samples available for difficult arms is $o(T)$. The budget constrained case has not been analyzed in~\cite{audibert2010best}, however in the absence of information leakage, one would expect that the arms with the least number of samples would be the most difficult to eliminate, and therefore the error guarantees would scale as $\exp(-O(BT)/\tilde{H}) \sim \exp(-o(T)/\tilde{H})$ (excluding $\log$ factors). On the other hand, our algorithm can leverage the information leakage and the error guarantee would scale as $\exp(-O(T)/\bar{H})$, which can be order-wise better if the \textit{effective standard deviations} are well-behaved. 
%
%\textbf{Remark:} Although similar advantages can be shown for \cite{lattimore2016causal}, there are no gap dependent bounds in that work and our analysis indicates a gap dependent improvement term by term with respect to \cite{audibert2010best}.
%
%
% \begin{theorem}\label{mainresult2}
%(Proved formally as Theorem \ref{thm:detailed})  Let $v^*$ be the effective inverse log divergence as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
%\ \begin{align}
%\label{eq:SRmain}
%&r(T,B) \leq  \\
%&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
%& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
% \end{align}
% Here, 
% \begin{align}
%  \label{HK}
% \bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds, which differentiates the arms according to its gap from the optimal arm and its \textit{effective standard deviation} parameter. The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$. 
%
%We defer the theoretical analysis to Section~\ref{sec:proofs}. In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we introduce the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%







==> resultsv5.tex <==
\label{sec:results}
In this section we provide our main theoretical contributions. In Section~\ref{sec:algo}, we provide a successive rejects style algorithm, that leverages the information leakage between the arms, via importance sampling. Then, we provide theoretical guarantees on the probability of mis-identification $(e(T,B))$ and simple regret $(r(T,B))$ for our algorithm in Section~\ref{sec:guarantee}. In order to explain our algorithm and our results formally, we first describe several key ideas in our algorithm and introduce definitions in Section~\ref{sec:def} that are relevant to these ideas.

\subsection{Definitions}
\label{sec:def}
%The algorithm starts by having all the $K$ arms under consideration and then proceeds in phases. At the beginning of each phase, a budget for samples is allocated to each arm. Thereafter, samples are collected according to the allocated budgets, and using these samples, importance sampling based estimators for the means of all the \textit{remaining} arms are formed. Then at the end of each phase, one or more arms are rejected based on some phase specific criterion on the estimated values. The structure of the algorithm and the estimation technique for the means of the arms,  both rely on a specific $f$-divergence between the arm distributions. 

\textbf{Quantifying Information Leakage:} We observe that
 \[\mu_k = \mathbb{E}_k[Y] = \mathbb{E}_{k'}\left[Y \frac{\mathrm{P}_k\left(V|pa(V) \right)}{\mathrm{P}_{k'}\left(V|pa(V)\right)}\right]. \] By weighing samples with the correct ratio of conditional probabilities $\mathrm{P}_k(\cdot)$ and $\mathrm{P}_{k'}(\cdot)$, it is possible to use samples under intervention $k'$ to estimate the mean under intervention $k$. However, the variance of this estimator depends on how different $\mathrm{P}_k(\cdot)$ is from $\mathrm{P}_{k}'(\cdot)$. We use a specific $f$-divergence measure between $\mathrm{P}_k(\cdot)$ is from $\mathrm{P}_{k}'(\cdot)$ to measure the difference. This $f$-divergence measure can be calculated analytically or estimated directly from empirical data (without the knowledge of the full distributions) using techniques like that of~\cite{perez2008kullback}. 

\begin{definition}
Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two joint distributions $p_{X,Y}(x,y)$ and $q_{X,Y}(x,y)$ (and the associated conditionals), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
\begin{align*}
D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q_{X,Y}} \left[f \left( \frac{p_{X \vert Y}(X \vert Y)}{q_{X \vert Y}(X \vert Y)} \right)\right].
\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
\end{definition}

 With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. 
 % We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
\begin{definition}
	\label{def:mij}
($M_{ij}$ measure)  Consider the function $f_1(x) = x \exp (x-1) - 1$. We define the following log-divergence measure:  $M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))$
%\begin{equation}
%\label{eq:mij}
%
%\end{equation}
\end{definition}
%\textbf{Remark:} We will call this log-divergence measure as the `$M_{ij}$ measure' for lack of a better descriptive name.

%One way to view the information leakage among arms is through the following expression relating the mean under arm $i$ to samples collected under arm $j$,
%\begin{align}
%\label{eq:basic_main}
%\EE_{i}\left[Y\right] = \EE_{j}\left[Y\frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))}\right]
%\end{align}
%which is trivially true as the only change in the joint distribution of all variables is at $\mathrm{P}(V \vert pa(V))$. However, directly using this expression to form an estimator, can lead to arbitrarily bad concentration as the ratio in the expression can be unbounded. Therefore, it is essential to clip the importance weighted samples at a carefully chosen value, such that we balance the trade-off between the variance of the samples and the bias incurred by the clipping. 
The quantities $M_{ij}$'s are crucial in the our analysis. 

\textbf{Aggregating Interventional Data:} Now, we describe an efficient estimator of $\EE_{k}[Y]$ ($\forall k \in [K]$) that seamlessly combines available samples from different arms. This estimator uses variable weights depending on the relative $M_{ij}$ measures and also  uses clipping to control variance by introducing bias. The estimator is given by (\ref{eq:uniestimator_main}).

Suppose we obtain $\tau_{i}$ samples from arm $i \in [K]$. Let the total number of samples from all arms put together be $\tau$. Let us index all the samples by $s \in \{1,2,..,\tau \}$. Let $\mathcal{T}_{k} \subset \{1,2,..,\tau \}$ be the indices of all the samples collected from arm $k$. Further, let $Z_k = \sum_{j \in [K]}\tau_j/M_{kj}$. Now, we are at the position to introduce the estimator for $\mu_k$, which we will denote by $\hat{Y}_{k}^{\epsilon}$ ($\epsilon$ is an indicator of the level of confidence desired):
\begin{align*}
\label{eq:uniestimator_main}
&\hat{Y}_{k}^{\epsilon}  = \frac{1}{Z_{k}}\sum_{j = 0}^{K} \sum_{s \in \mathcal{T}_j} \frac{1}{M_{kj}}Y_j(s)\frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \times
\\
&\mathds{1}\left\{ \frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \leq 2\log(2/\epsilon)M_{kj}\right\}. \numberthis
\end{align*}
In other words, $\hat{Y}_{k}^{\epsilon}$ is the weighted average of the clipped samples, where the samples from arm $j$ are weighted by $1/M_{kj}$ and clipped at $ 2\log(2/\epsilon)M_{kj}$. The \textbf{choice of $\epsilon$} controls the \textit{bias-variance tradeoff} which we will adaptively change in our algorithm. 

%\textbf{Effective Deviation:} Consider the following estimation problem - With a budget of $\tau$ samples, estimate $\mathbb{E}_k[Y]$ for all $k \in {\cal R}$ (set of arms not rejected). We first characterize the variance of estimators based on (\ref{eq:uniestimator_main}). Suppose a budget of $\tau$ samples has been allocated among arms in $[K]$ to estimate arms in a subset ${\cal R}$. Let the fraction of samples allocated to arm $k$ be $\nu_k$. Then, $\tau_i=\nu_i\times\tau$. Let $\pmb{\nu}=\left[\nu_1 \ldots \nu_K \right]^T$. Then, we define the effective standard deviation of the allocation as:
%
%\begin{definition}\label{effectiveallocation}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective standard deviation} $\sigma^*(\pmb{\nu},{\cal R})$ for {\bf allocation $\pmb{\nu}$}  and arm set ${\cal R} \subseteq [K] $ to be : 
%    %\begin{align}
%%\label{mainLP2}
%$\frac{1}{\sigma^*(\pmb{\nu},{\cal R})} = v^*(\pmb{\nu},{\cal R}) =\min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k}$ 
%%\end{align}
%\end{definition}
%\textbf{Remark:} Formally the minimum standard deviation of the set of estimators of the form (\ref{eq:uniestimator_main}) applied to estimating the means of arm-set ${\cal R}$ is given by Definition \ref{effectiveallocation} (Lemma \ref{allocation} in the appendix).
%
%\textbf{Allocation of Budget:} The above definition provides a handle on the effective variance on estimators of the form~(\ref{eq:uniestimator_main}) given an allocation of budget $\pmb{\nu}$. However, the choice of the allocation (while adhering to budget constraints) is in the hands of the algorithm designer. We design a sub-routine Algorithm~\ref{alg:allocate} (in the appendix) that allocates the samples, such that the worst estimator in (\ref{eq:uniestimator_main}) for arms amongst ${\cal R}$ is as  \textit{good} (quantified in Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the appendix) as possible. The target effective deviation of the worst estimator is:
%\begin{definition}\label{effectivelogdivergence}
%The \textbf{effective standard deviation} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ is defined as : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} v^*(\pmb{\nu},{\cal R})   \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}


\subsection{Algorithm}
Now, we describe our main algorithmic contribution - Algorithm \ref{alg:pickbest} and \ref{alg:pickbest2}.  Algorithm \ref{alg:pickbest}  starts by having all the $K$ arms under consideration and then proceeds in phases, rejecting one or more arms at the end of each phase. 

At every phase, Estimator $(\ref{eq:uniestimator_main})$ with a phase specific choice of  the $\epsilon$ parameter (i.e. controlling bias variance trade-off), is applied to all arms under consideration . Using a phase specific threshold on these estimates, some arms are rejected at the end of each phase. A random arm among the ones surviving at the end of \textit{all} phases is declared to be the optimal. We now describe the duration of various phases.

Recall the parameters $T$ -  Total sample budget available and $B$ - average cost budget constraint. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$.  We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$. We set $\tau(l) = T/(l\overline{\log}(n(T)))$ for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.

Let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$. The vector of allocated samples, i.e. $\pmb{\tau(\ell)}$ is decided by Algorithm~\ref{alg:allocate}. The performance depends crucially on the allocation. Intuitively, an arm that provides sufficient information about all the remaining arms needs to be given more budget than other less informative arms. This allocation depends on the average budget constraints and the relative log divergences between the arms (Definition~\ref{def:mij}). Algorithm~\ref{alg:allocate} ensures that variance of the worst estimator (of the form (\ref{eq:uniestimator_main})) for the arms in $\mathcal{R}$ is as \textit{good} as possible (quantified in Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the appendix). 



\begin{algorithm}
	\caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $c_i$'s) picks the best arm.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
		\STATE ${\cal R} = [K]$.
		\STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
		\FOR {$\ell=1$ to $n(T)$}      
		\STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
		\STATE Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
		\FOR {$k \in {\cal R}$}
		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator_main}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line 6.	\ENDFOR
		\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
		\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
		\IF {$\lvert {\cal R}\rvert =1$}
		\STATE \textbf{return:} the arm in ${\cal R}$.
		\ENDIF
		\ENDFOR
		\STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
	\end{algorithmic}
	\label{alg:pickbest}
\end{algorithm}


\begin{remark}  Note that Line 6 uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements.
\end{remark}

\begin{algorithm}
  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
  \begin{algorithmic}[1]
     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line 6 where all samples acquired in all the phases till that Line is used.
    \end{algorithmic}
   \label{alg:pickbest2}
\end{algorithm}
\label{sec:algo}

The inverse of the maximal objective of the LP in Algorithm~\ref{alg:allocate} acts as \textit{effective standard deviation} uniformly for all the estimators for the remaining arms in $\mathcal{R}$. It is analogous to the variance terms appearing in Bernstien-type concentration bounds (refer to Lemma~\ref{allocation} in the appendix).

\begin{definition}\label{effectivelogdivergence}
The \textbf{effective standard deviation} for budget $B$ and arm set ${\cal R} \subseteq [K] $ is defined as ${\sigma^*(B,{\cal R})} = 1/v^*(B,{\cal R})$ from Algorithm~\ref{alg:allocate} with input $B$ and arm set ${\cal R}$.
\end{definition}

\begin{algorithm}
	\caption{Allocate - Allocates a given budget $\tau$ among the arms to reduce variance.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{Allocate}(\mathbf{c},B,\mathbf{A},{\cal R},\tau)$
		\STATE Solve the following LP: 
		\begin{align}
		\label{mainLP1}
		\frac{1}{\sigma^*(B,{\cal R})} &= v^*(B,{\cal R}) =  \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
		&\text{s.t.~} \sum_{i=0}^K c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K} \nu_j = 1, ~\nu_i \geq 0. \nonumber
		\end{align}
		\STATE Assign $\tau_j = \nu_j^*(B,{\cal R})\tau $
	\end{algorithmic}
	\label{alg:allocate}
\end{algorithm}
\subsection{Theoretical Guarantees}
\label{sec:guarantee}
We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first gap dependent characterization.  
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%\begin{equation}
% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%  \end{equation}
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}

\begin{theorem}\label{mainresult}
	(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The probability of error for  Algorithm \ref{alg:pickbest} satisfies:
	\begin{equation}
	e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
	\end{equation}
	when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
	Here, 
	\begin{align}
	\label{Hbar}
	\bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison with the result in \cite{audibert2010best}:}
Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}: $e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)$. 

Our work is analogous to the above result (upto poly log factors) except that $\bar{H}$ appears instead of $\tilde{H}$. In Section~\ref{sec:compare1} (in the appendix), we demonstrate through simple examples that $\sigma^*(B,{\cal R}^*(\Delta_k))$ can be significantly smaller than $\sqrt{\tilde{\mathcal{R}}(\Delta_k)}$ (the corresponding term in $e(T)$ above) even when there are no average budget constraints. Moreover, our results can be exponentially better in the presence of average budget constraints (examples in Section~\ref{sec:compare1}). Now we present our bounds on simple regret in Theorem~\ref{mainresult2}.

\begin{theorem}\label{mainresult2}
	(Proved formally as Theorem \ref{thm:detailed})  Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
	\ \begin{align}
	\label{eq:SRmain}
	&r(T,B) \leq   \nonumber\\
	&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
	& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
	\end{align}
	Here, 
	\begin{align}
	\label{HK}
	\bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison with the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the simple regret scales as $O(1/\sqrt{T})$ and do not adapt to the gaps. We provide gap dependent bounds that can be exponentially better than that of~\cite{lattimore2016causal}. More over our bounds generalize to gap independent bounds that match $O(1/\sqrt{T})$. Further details are provided in Section~\ref{sec:compare2} (in the appendix).

%In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds. %The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. 
%It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$ and can handle general constraints on average budgets. Further details are provided in Section~\ref{sec:compare2}. 

We defer the theoretical analysis to Section~\ref{sec:proofs}. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we analyze the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 




























%\subsection{An Efficient Algorithm}\label{sec:algo}
%%We present two versions of \textit{successive rejects} style strategies, that attain the theoretical guarantees detailed in Section~\ref{sec:results}. Both the algorithms proceed in phases, successively rejecting arms at the end of each phase, until we are left with the optimal arm (provided $\Delta_{k} \geq 1/\sqrt{T}$ for all $k \in [K]$, otherwise it outputs a set of arms with $\Delta_k < 1/\sqrt{T}$). The only difference between Algorithms~\ref{algo:one} and \ref{algo:two} is that Algorithm~\ref{algo:one} only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while Algorithm~\ref{algo:two} reuses the past samples. 
%We present a successive rejects style algorithm that leverages the information leakage among the arms, through importance sampling. The algorithm proceeds in phases. The algorithm starts with all the arms under consideration, and rejects zero or more arms at the end of each phase successively, until we are left with only the best arm or possibly a few arms which are \textit{very} close to the best arm.  Let us define some notation that is helpful in describing the main algorithm:
%\begin{enumerate}
%\item $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 
%\item We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set,
%\begin{align}
%\tau(l) &= \frac{T}{\overline{\log}(n(T)) l} \label{taueq}\\
%\end{align}
%for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. Also, we have 
%\begin{equation}\label{timeatphase}
%T(l)= \frac{T \overline{\log}(l)}{\overline{\log}(n(T))}.
%\end{equation}
%\item Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.
%\end{enumerate}
%
%Although, we assume that $\mathrm{P}_k \left( V \vert pa(V) \right)$ and the marginal distribution $pa(V)$ are known, the algorithm we describe needs certain pairwise $f$-divergence values between these conditionals $\mathrm{P}_k$. The $f$-divergences can be calculated from the known distributions or estimated directly from data. Now we define the $f$- divergences that are required. 
%
%\subsubsection{Pairwise $f$- divergences}\label{f-div}
%\begin{definition}
%Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
%\begin{align*}
%D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
%\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
%\end{definition}
%
% With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by the shorthand $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. Consider the function $f_1(x) = x \exp (x-1) - 1$. We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
%
%For notational convenience, let us define log divergence to be:
%\begin{equation}
%\label{eq:mij}
%M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))
%\end{equation}
%
%The divergence measure $M_{ij}$ between $\mathrm{P}_i$ and $\mathrm{P}_j$ can be related to the `effective standard deviation' of the estimator that estimates $\mathbb{E}[Y]$ under $\mathrm{P}_i$ using samples from $\mathrm{P}_j$. Larger the divergence, larger is the variance of the estimator.
%
%\begin{definition}\label{effectivelogdivergence}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective variance} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ to be : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}
%$\sigma^*$ is the `effective standard deviation' when arms from $[K]$ are used to estimate the means of the arms in set ${\cal R}$, under relative fractional budget $B$. We will justify this by analyzing a heterogenous importance sampling estimator and deriving confidence intervals for it in later sections.
%
%Now, we describe one of our main contributions - Algorithm \ref{alg:pickbest}.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $\nu_i$) picks the best arm.}
%  \begin{algorithmic}[1]
%    \STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
%    \STATE ${\cal R} = [K]$.
%    \STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
%    \FOR {$\ell=1$ to $n(T)$}      
%        \STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
%        \STATE \label{linesamp} Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
%        \FOR {$k \in {\cal R}$}
%    		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\ENDFOR
%	\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
%	\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
%	\IF {$\lvert {\cal R}\rvert =1$}
%	  	\STATE \textbf{return:} the arm in ${\cal R}$.
%	\ENDIF
%    \ENDFOR
%    \STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
%      \end{algorithmic}
%    \label{alg:pickbest}
%\end{algorithm}
%\textbf{Remark:}  Note that Line \ref{linesamp} uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements. We will show our algorithms outperform all other algorithms in related prior work.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
%  \begin{algorithmic}[1]
%     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line \ref{samplestamp} where all samples acquired in all the phases till that Line is used.
%    \end{algorithmic}
%   \label{alg:pickbest2}
%\end{algorithm}
%
%\subsection{Theoretical Guarantees}
%\label{sec:guarantee}
%We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first problem dependent characterization of the problem.  
%%\begin{theorem}\label{mainresult}
%%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%%\begin{equation}
%% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%%  \end{equation}
%% Here, 
%% \begin{align}
%%  \label{Hbar}
%%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%%  \end{align}
%%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%%\end{theorem}
%
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) satisfies:
%\begin{equation}
% e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
%  \end{equation}
%  when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{audibert2010best}:}
%Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result for the best arm identification with no information leakage in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}:
% \begin{equation}\label{noleakage}
%   e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)
% \end{equation}
%
% One intuitive interpretation for $\tilde{H}$ is that it is the maximum among the number of samples (neglecting some log factors) required to conclude that arm $k$ is suboptimal from among the arms which are closer to the optimal than itself. Intuitively, this is because when there is no information leakage, one requires $1/\Delta_k^2$ samples to distinguish between the $k$-th optimal arm and the optimal arm. Further, the $k$th arm is played only $1/k$ fraction of the times since we do not know the identity of the $k$-th optimal arm. 
%  
%\textbf{Interpretation of our Result:}
%Our main result in Theorem $\ref{mainresult}$ can be seen to be a generalization of the existing result in (\ref{noleakage}) for the case when there is information leakage between the arms (various changes in a causal graph).  
%
%The term $\sigma^*(B,{\cal R}^*(\Delta_k))$ in our setting is the `effective standard deviation' due to information leakage.  There is a similar interpretation of our result (ignoring the log factors): Since there is information leakage, the expression $\frac{(\sigma^*)^2}{(\Delta_k)^2}$ characterizes the number of samples required to weed out arm $k$ out of contention from among competing arms (arms that are at a distance at most twice than that of arm $k$ from the optimal arm). The interpretation of 'effective variance' is justified using importance sampling which is detailed in Section \ref{sec:estimator}. Further, in our framework $\sigma^*$ also incorporates any budget constraint that comes with the problem, i.e. any \textit{apriori} constraint on the relative fraction of times different arms need to be pulled.
%
%\textbf{Improvement over the no-information leakage case:}
%For ease of exposition let $(k)$ denote the index of the $k$-th best arm (for $k = 1,..,K$) and $\Delta_{(k)}$ denotes the corresponding gap. In this setting, the terms $\tilde{H}$ (from the result in~\cite{audibert2010best}) and $\bar{H}$ can be written as:
%\begin{align*}
%\tilde{H} &= \max_{k \neq 1} \frac{k}{\Delta_{(k)}^2} \\
%\bar{H} &= \max_{k \neq 1} \frac{\sigma^*(B,{\cal R}^*(\Delta_{(k)}))^2}{\Delta_{(k)}^2}.
%\end{align*}
%$ \sigma^*(B,{\cal R}^*(\Delta_{(k)}))$ can be smaller than $\sqrt{k}$ due to information leakage as every single arm pull contributes to another arm's estimate. Therefore, these provide better guarantees than ~\cite{audibert2010best}. 
%
%To see the improvement over the previous result in \cite{audibert2010best}, we consider a special case when the cost budget $B$ is infinity and there is only the the sample budget $T$. In addition, let us assume that the log divergences are such that: $M_{ij} \leq \eta M_{ii} = \eta << \sqrt{\lvert {\cal R}  \rvert},~ \forall i \neq j$. Let ${\cal R} = {\cal R}^*(\Delta_{(k)})$. If $\eta > \sqrt{\lvert {\cal R}  \rvert}$, the optimal solution for (\ref{mainLP1}) is a bit complicated to interpret.  Consider the feasible allocation $\nu_i = \frac{1}{\lvert {\cal R}  \rvert}, ~ \forall i \in {\cal R}$ in (\ref{mainLP1}). Evaluating the objective function for this feasible allocation, it is possible to show that $\sigma^* \leq \frac{\eta}{1-1/\lvert {\cal R}  \rvert} <<  \sqrt{\lvert {\cal R}  \rvert}$. Hence, unless the variance due to information leakage is too bad, the effective variance is smaller than that of the case with no information leakage.
%
%The improvement over the no information leakage setting, is even more pronounced under budget constraints. Consider the setting \textbf{S1}, and assume that the fractional budget of the \textit{difficult} arms, $B = o(1)$. This implies that the total number of samples available for difficult arms is $o(T)$. The budget constrained case has not been analyzed in~\cite{audibert2010best}, however in the absence of information leakage, one would expect that the arms with the least number of samples would be the most difficult to eliminate, and therefore the error guarantees would scale as $\exp(-O(BT)/\tilde{H}) \sim \exp(-o(T)/\tilde{H})$ (excluding $\log$ factors). On the other hand, our algorithm can leverage the information leakage and the error guarantee would scale as $\exp(-O(T)/\bar{H})$, which can be order-wise better if the \textit{effective standard deviations} are well-behaved. 
%
%\textbf{Remark:} Although similar advantages can be shown for \cite{lattimore2016causal}, there are no gap dependent bounds in that work and our analysis indicates a gap dependent improvement term by term with respect to \cite{audibert2010best}.
%
%
% \begin{theorem}\label{mainresult2}
%(Proved formally as Theorem \ref{thm:detailed})  Let $v^*$ be the effective inverse log divergence as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
%\ \begin{align}
%\label{eq:SRmain}
%&r(T,B) \leq  \\
%&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
%& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
% \end{align}
% Here, 
% \begin{align}
%  \label{HK}
% \bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds, which differentiates the arms according to its gap from the optimal arm and its \textit{effective standard deviation} parameter. The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$. 
%
%We defer the theoretical analysis to Section~\ref{sec:proofs}. In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we introduce the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%







==> resultsv6.tex <==
\label{sec:results}
In this section we provide our main theoretical contributions. In
Section~\ref{sec:algo}, we provide a successive rejects style
algorithm that leverages the information leakage between the arms via
importance sampling. Then, we provide theoretical guarantees on the
probability of mis-identification $(e(T,B))$ and simple regret
$(r(T,B))$ for our algorithm in Section~\ref{sec:guarantee}. In order
to explain our algorithm and our results formally, we first describe
several key ideas in our algorithm and introduce important definitions in
Section~\ref{sec:def}.

\subsection{Definitions}
\label{sec:def}
%The algorithm starts by having all the $K$ arms under consideration and then proceeds in phases. At the beginning of each phase, a budget for samples is allocated to each arm. Thereafter, samples are collected according to the allocated budgets, and using these samples, importance sampling based estimators for the means of all the \textit{remaining} arms are formed. Then at the end of each phase, one or more arms are rejected based on some phase specific criterion on the estimated values. The structure of the algorithm and the estimation technique for the means of the arms,  both rely on a specific $f$-divergence between the arm distributions. 

\textbf{Quantifying Information Leakage:} %We observe that
% \[\mu_k = \mathbb{E}_k[Y] = \mathbb{E}_{k'}\left[Y
%     \frac{\mathrm{P}_k\left(V|pa(V)
%       \right)}{\mathrm{P}_{k'}\left(V|pa(V)\right)}\right]. \] By
% weighting samples with the correct ratio of conditional probabilities
% $\mathrm{P}_k(\cdot)$ and $\mathrm{P}_{k'}(\cdot)$, it is possible to
% use samples under intervention $k'$ to estimate the mean under
% intervention $k$. However, the variance of this estimator depends on
% the ratio of $\mathrm{P}_k(\cdot)$ to $\mathrm{P}_{k}'(\cdot)$.
% We use a specific $f$-divergence measure between
% $\mathrm{P}_k(\cdot)$ and $\mathrm{P}_{k}'(\cdot)$ to quantify
% the variance. This $f$-divergence measure can be calculated
% analytically or estimated directly from empirical data (without the
% knowledge of the full distributions) using techniques like that
% of~\cite{perez2008kullback}. 
One of the salient features of this problem is that there is information leakage among the $K$ arms of the bandit. The different arms that are being tested only differ in the conditional distribution of $V$ given its parents $pa(V)$, while the rest of the relationships in the causal graph $\mathcal{G}$ remain unchanged. Since the different candidate conditional distributions $\mathrm{P}_{k}(V \vert pa(V))$ are known from prior knowledge, it is possible to utilize samples obtained under an arm $j$ to obtain an estimate for the expectation under arm $i$ (i.e $\EE_{i} \left[ Y\right]$). A popular method for utilizing this information leakage among different distributions is \textit{importance sampling}. Importance sampling has been used before in counterfactual analysis in a similar causal setting~\cite{lattimore2016causal, bottou2013counterfactual}.

{\bf \noindent Importance Sampling:} Now we introduce the concept of importance sampling which is one of the key tools we use to leverage the information leakage between the candidate arms. Suppose we get samples from arm $j \in [K]$ and we are interested in estimating $\EE_i[Y]$. In this context it helpful to express $\EE_i[Y]$ in the following manner:
\begin{align}
\label{eq:basic}
\EE_{i}\left[Y\right] = \EE_{j}\left[Y\frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))}\right]
\end{align}
(\ref{eq:basic}) is trivially true because the only change to the joint distribution of all the variables in the causal graph $\mathcal{G}$ under arm $i$ and $j$ is at the factor $\mathrm{P}(V \vert pa(V))$. Suppose we observe $t$ samples of $\{Y, V, pa(V) \}$ from the arm $j$, denoted by $\{Y_j(s),V_j(s),pa(V)_j(s)\}_{s=1}^{t}$. Here $X_j(s)$ denotes the sample from random variable $X$ at time step $s$, while the sub-script $j$ just denotes that the samples are collected under arm $j$. Under the observation of  Equation (\ref{eq:basic}), one might assume that the naive estimator, 
\begin{align}
\label{eq:naive}
\hat{Y}'_i(j) = \frac{1}{t}\sum_{s = 1}^{t} Y_j(s)\frac{\mathrm{P}_i(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))}
\end{align} 
provides a good estimate for $\mu_i = \EE_{i} \left[ Y\right]$. However, the confidence guarantees on such an estimate can be arbitrarily bad even though $Y$ is bounded. This is because the factor $\mathrm{P}_i(V \vert pa(V))/\mathrm{P}_j(V \vert pa(V))$ can be very large for several values of $V, pa(V)$. Therefore, usual confidence inequalities like Azuma-Hoeffding's, Berstein's would not yield good confidence intervals. This has been noted in~\cite{lattimore2016causal} in a similar setting, where a \textit{static} clipper has been used to control the variance. This static clipper introduces bias which is not suitable for obtaining gap dependent simple regret bounds. In our algorithm we use dynamic clipping to carefully control the bias variance trade-off in a phase dependent manner. This leads to significantly better gap dependent bounds that also generalize to a gap independent bounds. We now define some key quantities.

\begin{definition}
Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$.
For two joint distributions $p_{X,Y}(x,y)$ and $q_{X,Y}(x,y)$ (and the
associated  conditionals), the conditional $f$-divergence $D_{f}(p_{X
  \vert Y} \Vert q_{X \vert Y})$ is given by: 
\begin{align*}
D_{f}(p_{X \vert Y} \Vert q_{X \vert Y}) = \EE_{q_{X,Y}} \left[f \left( \frac{p_{X \vert Y}(X \vert Y)}{q_{X \vert Y}(X \vert Y)} \right)\right].
\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
\end{definition}
 % With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert
 % pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by $D_f(\mathrm{P}_i \Vert
 % \mathrm{P}_j)$. 
Recall that $\mathrm{P}_i$ is the conditional distribution of node $V$
given the state of its parents $pa(V).$ Thus, $D_f(\mathrm{P}_i \Vert
\mathrm{P}_j)$ is the conditional $f$-divergence between the conditional
distributions $P_i$ and $P_j.$ Now we define some \textit{log-divergences} that are are crucial in the our analysis.
% We have the following relation,
% \begin{align} \label{eq:divergence} \mathbb{E}_{i} \left[ \exp
%     \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert
%       pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i
%       \lVert \mathrm{P}_j\right) \right]e. \end{align}
\begin{definition}
	\label{def:mij}
($M_{ij}$ measure)  Consider the function $f_1(x) = x \exp (x-1) - 1$. We define the following log-divergence measure:  $M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j)),$ $\forall i,j \in [K].$
%\begin{equation}
%\label{eq:mij}
%
%\end{equation}
\end{definition}
\noindent These log divergences help us in controlling the bias variance trade-off in importance sampling as shown in Section~\ref{sec:relation} in the appendix.
%\textbf{Remark:} We will call this log-divergence measure as the `$M_{ij}$ measure' for lack of a better descriptive name.

%One way to view the information leakage among arms is through the following expression relating the mean under arm $i$ to samples collected under arm $j$,
%\begin{align}
%\label{eq:basic_main}
%\EE_{i}\left[Y\right] = \EE_{j}\left[Y\frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))}\right]
%\end{align}
%which is trivially true as the only change in the joint distribution of all variables is at $\mathrm{P}(V \vert pa(V))$. However, directly using this expression to form an estimator, can lead to arbitrarily bad concentration as the ratio in the expression can be unbounded. Therefore, it is essential to clip the importance weighted samples at a carefully chosen value, such that we balance the trade-off between the variance of the samples and the bias incurred by the clipping. 
 

\noindent \textbf{Aggregating Interventional Data:} We describe an efficient
estimator of $\EE_{k}[Y]$ ($\forall k \in [K]$) that combines
available samples from different arms. This estimator adaptively
weights samples depending on the relative $M_{ij}$ measures, and also
uses clipping to control variance by introducing bias. The estimator
is given by (\ref{eq:uniestimator_main}).

Suppose we obtain $\tau_{i}$ samples from arm $i \in [K]$. Let the
total number of samples from all arms be denoted by $\tau$. Further,
let us index all the samples by $s \in \{1,2,..,\tau \},$ and
$\mathcal{T}_{k} \subset \{1,2,..,\tau \}$ be the indices of all the
samples collected from arm $k$. Let $X_j(s)$ denotes the sample collected for random variable $X$ under intervention $j$, at time instant $s$. Finally, let $Z_k = \sum_{j \in
  [K]}\tau_j/M_{kj}$. 
We denote the estimate of  $\mu_k$ by $\hat{Y}_{k}^{\epsilon}$
($\epsilon$ is an indicator of the level of confidence desired).
Our estimator is:  
\begin{align*}
\label{eq:uniestimator_main}
&\hat{Y}_{k}^{\epsilon}  = \frac{1}{Z_{k}}\sum_{j = 0}^{K} \sum_{s \in
  \mathcal{T}_j} \frac{1}{M_{kj}}Y_j(s)\frac{\mathrm{P}_k(V_j(s) \vert
  pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \times \mathds{1}\left\{ \frac{\mathrm{P}_k(V_j(s) \vert pa(V)_j(s))}{\mathrm{P}_j(V_j(s) \vert pa(V)_j(s))} \leq 2\log(2/\epsilon)M_{kj}\right\}. \numberthis
\end{align*}
In other words, $\hat{Y}_{k}^{\epsilon}$ is the weighted average of
the clipped samples, where the samples from arm $j$ are weighted by
$1/M_{kj}$ and clipped at $ 2\log(2/\epsilon)M_{kj}$. The
\textbf{choice of $\epsilon$} controls the \textit{bias-variance
  tradeoff} which we will adaptively change in our algorithm.

%\textbf{Effective Deviation:} Consider the following estimation problem - With a budget of $\tau$ samples, estimate $\mathbb{E}_k[Y]$ for all $k \in {\cal R}$ (set of arms not rejected). We first characterize the variance of estimators based on (\ref{eq:uniestimator_main}). Suppose a budget of $\tau$ samples has been allocated among arms in $[K]$ to estimate arms in a subset ${\cal R}$. Let the fraction of samples allocated to arm $k$ be $\nu_k$. Then, $\tau_i=\nu_i\times\tau$. Let $\pmb{\nu}=\left[\nu_1 \ldots \nu_K \right]^T$. Then, we define the effective standard deviation of the allocation as:
%
%\begin{definition}\label{effectiveallocation}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective standard deviation} $\sigma^*(\pmb{\nu},{\cal R})$ for {\bf allocation $\pmb{\nu}$}  and arm set ${\cal R} \subseteq [K] $ to be : 
%    %\begin{align}
%%\label{mainLP2}
%$\frac{1}{\sigma^*(\pmb{\nu},{\cal R})} = v^*(\pmb{\nu},{\cal R}) =\min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k}$ 
%%\end{align}
%\end{definition}
%\textbf{Remark:} Formally the minimum standard deviation of the set of estimators of the form (\ref{eq:uniestimator_main}) applied to estimating the means of arm-set ${\cal R}$ is given by Definition \ref{effectiveallocation} (Lemma \ref{allocation} in the appendix).
%
%\textbf{Allocation of Budget:} The above definition provides a handle on the effective variance on estimators of the form~(\ref{eq:uniestimator_main}) given an allocation of budget $\pmb{\nu}$. However, the choice of the allocation (while adhering to budget constraints) is in the hands of the algorithm designer. We design a sub-routine Algorithm~\ref{alg:allocate} (in the appendix) that allocates the samples, such that the worst estimator in (\ref{eq:uniestimator_main}) for arms amongst ${\cal R}$ is as  \textit{good} (quantified in Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the appendix) as possible. The target effective deviation of the worst estimator is:
%\begin{definition}\label{effectivelogdivergence}
%The \textbf{effective standard deviation} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ is defined as : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} v^*(\pmb{\nu},{\cal R})   \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}


\subsection{Algorithm}
Now, we describe our main algorithmic contribution - Algorithm
\ref{alg:pickbest} and \ref{alg:pickbest2}.  Algorithm
\ref{alg:pickbest}  starts by having all the $K$ arms under
consideration and then proceeds in phases, possibly rejecting one or more arms
at the end of each phase.  

At every phase, Estimator $(\ref{eq:uniestimator_main})$ with a phase
specific choice of  the $\epsilon$ parameter (i.e. controlling bias
variance trade-off), is applied to all arms under consideration. Using
a phase specific threshold on these estimates, some arms are rejected
at the end of each phase. A random arm among the ones surviving at the
end of \textit{all} phases is declared to be the optimal. We now
describe the duration of various phases. 

Recall the parameters $T$ -  Total sample budget available and $B$ -
average cost budget constraint. Let $n(T) = \lceil \log 2 \times \log
10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$.
We will have an algorithm with $n(T)$ phases numbered by $\ell =
1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase
$\ell$. We set $\tau(l) = T/(l\overline{\log}(n(T)))$ for $l \in
\{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let ${\cal R}$ be the
set of arms remaining to compete with the optimal arm at the beginning
of phase $\ell$ which is continuously updated. 

Let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase
$\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{
\tau_k\left(\ell \right) \}$. The vector of allocated samples, i.e.
$\pmb{\tau(\ell)}$ is decided by Algorithm~\ref{alg:allocate}. 
%
%% The performance depends crucially on the allocation. 
%
Intuitively, an arm that provides sufficient information about all the
remaining arms needs to be given more budget than other less
informative arms. This allocation depends on the average budget
constraints and the relative log divergences between the arms
(Definition~\ref{def:mij}). Algorithm~\ref{alg:allocate} formalizes
this intuition, and ensures that variance of the worst estimator (of
the form (\ref{eq:uniestimator_main})) for the arms in $\mathcal{R}$
is as \textit{good} as possible (quantified in
Theorem~\ref{thm:uniestimator} and Lemma~\ref{allocation} in the
appendix).



\begin{algorithm}
	\caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $c_i$'s) picks the best arm.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
		\STATE ${\cal R} = [K]$.
		\STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
		\FOR {$\ell=1$ to $n(T)$}      
		\STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
		\STATE Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
		\FOR {$k \in {\cal R}$}
		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator_main}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line 6.	\ENDFOR
		\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
		\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
		\IF {$\lvert {\cal R}\rvert =1$}
		\STATE \textbf{return:} the arm in ${\cal R}$.
		\ENDIF
		\ENDFOR
		\STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
	\end{algorithmic}
	\label{alg:pickbest}
\end{algorithm}

\begin{remark} Note that Line 6 uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm~\ref{alg:pickbest}. We conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements.
\end{remark}
\begin{algorithm}
	\caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
	\begin{algorithmic}[1]
		\STATE Identical to Algorithm \ref{alg:pickbest} except for Line 6 where all samples acquired in all the phases till that Line is used.
	\end{algorithmic}
	\label{alg:pickbest2}
\end{algorithm}
\label{sec:algo}

The inverse of the maximal objective of the LP in Algorithm~\ref{alg:allocate} acts as \textit{effective standard deviation} uniformly for all the estimators for the remaining arms in $\mathcal{R}$. It is analogous to the variance terms appearing in Bernstien-type concentration bounds (refer to Lemma~\ref{allocation} in the appendix).

\begin{definition}\label{effectivelogdivergence}
The \textbf{effective standard deviation} for budget $B$ and arm set ${\cal R} \subseteq [K] $ is defined as ${\sigma^*(B,{\cal R})} = 1/v^*(B,{\cal R})$ from Algorithm~\ref{alg:allocate} with input $B$ and arm set ${\cal R}$.
\end{definition}

\begin{algorithm}
	\caption{Allocate - Allocates a given budget $\tau$ among the arms to reduce variance.}
	\begin{algorithmic}[1]
		\STATE $\mathrm{ALLOCATE}(\mathbf{c},B,\mathbf{A},{\cal R},\tau)$
		\STATE Solve the following LP: 
		\begin{align}
		\label{mainLP1}
		\frac{1}{\sigma^*(B,{\cal R})} &= v^*(B,{\cal R}) =  \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
		&\text{s.t.~} \sum_{i=0}^K c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K} \nu_j = 1, ~\nu_i \geq 0. \nonumber
		\end{align}
		where $[\mathbf{A}\pmb{\nu}]_{k}$ denotes the $k^{th}$ element in the vector $\mathbf{A}\pmb{\nu}$.
		\STATE Assign $\tau_j = \nu_j^*(B,{\cal R})\tau $
	\end{algorithmic}
	\label{alg:allocate}
\end{algorithm}
\subsection{Theoretical Guarantees}
\label{sec:guarantee}
We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first gap dependent characterization.  
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%\begin{equation}
% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%  \end{equation}
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}

\begin{theorem}\label{mainresult}
	(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The probability of error for  Algorithm \ref{alg:pickbest} satisfies:
	\begin{equation}
	e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
	\end{equation}
	when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
	Here, 
	\begin{align}
	\label{Hbar}
	\bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
\end{theorem}

\textbf{Comparison with the result in \cite{audibert2010best}:}
Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}: $e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)$. 

Our work is analogous to the above result (upto poly log factors) except that $\bar{H}$ appears instead of $\tilde{H}$. In Section~\ref{sec:compare1} (in the appendix), we demonstrate through simple examples that $\sigma^*(B,{\cal R}^*(\Delta_k))$ can be significantly smaller than $\sqrt{\tilde{\mathcal{R}}(\Delta_k)}$ (the corresponding term in $e(T)$ above) even when there are no average budget constraints. Moreover, our results can be exponentially better in the presence of average budget constraints (examples in Section~\ref{sec:compare1}). Now we present our bounds on simple regret in Theorem~\ref{mainresult2}.

\begin{theorem}\label{mainresult2}
	(Proved formally as Theorem \ref{thm:detailed})  Let $\sigma^*(.)$ be the effective standard deviation as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
	\ \begin{align}
	&r(T,B) \leq  
	 \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} +2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) 	\label{eq:SRmain}
	\end{align}
	Here, 
%	\begin{align}
%	\label{HK}
	$\bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}$
%	\end{align}
	and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \}. $ 
\end{theorem}

\textbf{Comparison with the result in \cite{lattimore2016causal}:}
In~\cite{lattimore2016causal}, the simple regret scales as
$O(1/\sqrt{T})$ and does not adapt to the gaps. We provide gap
dependent bounds that can be exponentially better than that
of~\cite{lattimore2016causal} (when $\Delta_k$'s are not too small and the first term in (\ref{eq:SRmain}) is zero). More over our bounds generalize to gap
independent bounds that match $O(1/\sqrt{T})$. Further details are
provided in Section~\ref{sec:compare2} (in the appendix).

%In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds. %The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. 
%It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$ and can handle general constraints on average budgets. Further details are provided in Section~\ref{sec:compare2}. 

We defer the theoretical analysis to Section~\ref{sec:proofs}. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we analyze the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 




























%\subsection{An Efficient Algorithm}\label{sec:algo}
%%We present two versions of \textit{successive rejects} style strategies, that attain the theoretical guarantees detailed in Section~\ref{sec:results}. Both the algorithms proceed in phases, successively rejecting arms at the end of each phase, until we are left with the optimal arm (provided $\Delta_{k} \geq 1/\sqrt{T}$ for all $k \in [K]$, otherwise it outputs a set of arms with $\Delta_k < 1/\sqrt{T}$). The only difference between Algorithms~\ref{algo:one} and \ref{algo:two} is that Algorithm~\ref{algo:one} only uses the samples obtained in the current phase, to take the decisions at the end of the phase, while Algorithm~\ref{algo:two} reuses the past samples. 
%We present a successive rejects style algorithm that leverages the information leakage among the arms, through importance sampling. The algorithm proceeds in phases. The algorithm starts with all the arms under consideration, and rejects zero or more arms at the end of each phase successively, until we are left with only the best arm or possibly a few arms which are \textit{very} close to the best arm.  Let us define some notation that is helpful in describing the main algorithm:
%\begin{enumerate}
%\item $T$ -  Total sample budget available. $B$ - average cost budget. Let $n(T) = \lceil \log 2 \times \log 10\sqrt{T} \rceil$. Let $\overline{\log}(n) = \sum_{i = 1}^{n}(1/i)$. 
%\item We will have an algorithm with $n(T)$ phases numbered by $\ell = 1,2.,,n(T)$. Let $\tau(\ell)$ be the total number of samples in phase $\ell$ and let $\tau_k(\ell)$ be the samples allocated to arm $k$ in phase $\ell$. Let $\pmb{\tau(\ell)}$ be the vector consisting of entries $\{ \tau_k\left(\ell \right) \}$ We set,
%\begin{align}
%\tau(l) &= \frac{T}{\overline{\log}(n(T)) l} \label{taueq}\\
%\end{align}
%for $l \in \{1,..,n(T) \}$. Note that $\sum_{l}\tau(l)= T$. Let $T(l) = \sum_{s = 1}^{l}\tau(s)$. Also, we have 
%\begin{equation}\label{timeatphase}
%T(l)= \frac{T \overline{\log}(l)}{\overline{\log}(n(T))}.
%\end{equation}
%\item Let ${\cal R}$ be the set of arms remaining to compete with the optimal arm at the beginning of phase $\ell$ which is continuously updated.
%\end{enumerate}
%
%Although, we assume that $\mathrm{P}_k \left( V \vert pa(V) \right)$ and the marginal distribution $pa(V)$ are known, the algorithm we describe needs certain pairwise $f$-divergence values between these conditionals $\mathrm{P}_k$. The $f$-divergences can be calculated from the known distributions or estimated directly from data. Now we define the $f$- divergences that are required. 
%
%\subsubsection{Pairwise $f$- divergences}\label{f-div}
%\begin{definition}
%Let $f(\cdot)$ be a non-negative convex function such that $f(1) = 0$. For two conditional distributions $p(X \vert Y)$ and $q(X \vert Y)$ (and the associated joint distributions), the conditional $f$-divergence $D_{f}(p(X \vert Y) \Vert q(X \vert Y))$ is given by:
%\begin{align*}
%D_{f}(p(X \vert Y) \Vert q(X \vert Y)) = \EE_{q} \left[f \left( \frac{p(X \vert Y)}{q(X \vert Y)} \right)\right].
%\end{align*}
%Further for two discrete conditional distributions $p$ and $q$, $D_{f}(p \Vert q)$ can be expressed as the summation:
%\begin{align*}
%&D_{f}(p(X \vert Y) \Vert q(X \vert Y))\\
%&= \sum_{y} q(y) \left(\sum_{x} f \left( \frac{p( x \vert  y)}{q( x\vert  y)}\right)q(x\vert  y)\right)
%\end{align*}
%\end{definition}
%
% With some abuse of notation, we will denote $D_f(\mathrm{P}_i(V \vert pa(V)) \Vert \mathrm{P}_j(V \vert pa(V)))$ by the shorthand $D_f(\mathrm{P}_i \Vert \mathrm{P}_j)$. Consider the function $f_1(x) = x \exp (x-1) - 1$. We have the following relation,
%\begin{align}
%\label{eq:divergence}
% \mathbb{E}_{i} \left[ \exp \left( \frac{\mathrm{P}_i(V \vert pa(V))}{\mathrm{P}_j(V \vert pa(V))} \right) \right] = \left[ 1+D_{f_1}\left(\mathrm{P}_i \lVert \mathrm{P}_j\right) \right]e.
%\end{align}
%
%For notational convenience, let us define log divergence to be:
%\begin{equation}
%\label{eq:mij}
%M_{ij} = 1 + \log (1 + D_{f_1} (\mathrm{P}_i \lVert \mathrm{P}_j))
%\end{equation}
%
%The divergence measure $M_{ij}$ between $\mathrm{P}_i$ and $\mathrm{P}_j$ can be related to the `effective standard deviation' of the estimator that estimates $\mathbb{E}[Y]$ under $\mathrm{P}_i$ using samples from $\mathrm{P}_j$. Larger the divergence, larger is the variance of the estimator.
%
%\begin{definition}\label{effectivelogdivergence}
%Consider the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $\mathbf{A}_{kj} = 1/M_{kj}$ for all $k,j \in [K]$.  We define the \textbf{effective variance} $\sigma^*(B,{\cal R})$ for budget $B$ and arm set ${\cal R} \subseteq [K] $ to be : 
%    \begin{align}
%\label{mainLP1}
%&\frac{1}{\sigma^*(B,{\cal R})} = v^*(B,{\cal R}) = \max_{\pmb{\nu}} \min_{k \in {\cal R}} [\mathbf{A}\pmb{\nu}]_{k} \\
% &\text{s.t.~} \sum_{i=0}^{K-1} c_i \nu_{i} \leq B  \text{ and } \sum_{j = 0}^{K-1} \nu_j = 1, ~\nu_i \geq 0. \nonumber
%\end{align}
%\end{definition}
%$\sigma^*$ is the `effective standard deviation' when arms from $[K]$ are used to estimate the means of the arms in set ${\cal R}$, under relative fractional budget $B$. We will justify this by analyzing a heterogenous importance sampling estimator and deriving confidence intervals for it in later sections.
%
%Now, we describe one of our main contributions - Algorithm \ref{alg:pickbest}.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v1 (SRISv1) - Given total budget $T$ and the cost budget $B$ (along with $\nu_i$) picks the best arm.}
%  \begin{algorithmic}[1]
%    \STATE $\mathrm{SRIS}(B,\{M_{kj} \},T)$
%    \STATE ${\cal R} = [K]$.
%    \STATE Form the matrix $\mathbf{A} \in \mathbb{R}^{K \times K}$ such that $A_{kj} = \frac{1}{M_{kj}}$.
%    \FOR {$\ell=1$ to $n(T)$}      
%        \STATE $\pmb{\tau(\ell)} = \mathrm{ALLOCATE} \left(\mathbf{c}, B, \mathbf{A},{\cal R}, \tau(\ell) \right)$ (Algorithm~\ref{alg:allocate})
%        \STATE \label{linesamp} Use arm $k$, $\tau_k(\ell)$ times and collect samples $(Y,V, pa(V) )$.
%        \FOR {$k \in {\cal R}$}
%    		\STATE \label{samplestamp}Let $\hat{Y}_k$ be the estimator for arm $k$ as in (\ref{eq:uniestimator}) calculated with $\{M_{kj} \}$, $\epsilon = 2^{-(\ell-1)}$ and the samples obtained in Line \ref{linesamp}.	\ENDFOR
%	\STATE Let $\hat{Y}_H  = \argmax _{k \in {\cal R}} \hat{Y}_k$. 
%	\STATE ${\cal R}= {\cal R} - \{k \in {\cal R} : \hat{Y}_H > \hat{Y}_k + 5/2^{l} \}$.
%	\IF {$\lvert {\cal R}\rvert =1$}
%	  	\STATE \textbf{return:} the arm in ${\cal R}$.
%	\ENDIF
%    \ENDFOR
%    \STATE \textbf{return:} A randomly chosen arm from ${\cal R}$.
%      \end{algorithmic}
%    \label{alg:pickbest}
%\end{algorithm}
%\textbf{Remark:}  Note that Line \ref{linesamp} uses only the samples acquired in that phase. Clearly, a natural extension is to modify the algorithm to re-use all the samples acquired prior to that step. We give that variation in Algorithm \ref{alg:pickbest2}. We prove all our guarantees for Algorithm \ref{alg:pickbest} and we conjecture that the second variation has tighter guarantees (dropping a multiplicative log factor) in the sample complexity requirements. We will show our algorithms outperform all other algorithms in related prior work.
%
%\begin{algorithm}
%  \caption{Successive Rejects with Importance Sampling -v2 (SRISv2) - Given total budget $T$ and the cost budget $B$ (along with $\mathbf{c}$) picks the best arm.}
%  \begin{algorithmic}[1]
%     \STATE Identical to Algorithm \ref{alg:pickbest} except for Line \ref{samplestamp} where all samples acquired in all the phases till that Line is used.
%    \end{algorithmic}
%   \label{alg:pickbest2}
%\end{algorithm}
%
%\subsection{Theoretical Guarantees}
%\label{sec:guarantee}
%We state our main results as Theorem~\ref{mainresult} and Theorem~\ref{mainresult2}, which provide guarantees on probability of error and simple regret respectively. Our results can be interpreted as a natural generalization of the results in~\cite{audibert2010best}, when there is information leakage among the arms. This is the first problem dependent characterization of the problem.  
%%\begin{theorem}\label{mainresult}
%%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) is at most $\delta$, whenever the following relation involving total number of samples $T$  is satisfied:
%%\begin{equation}
%% \frac{T}{\overline{\log}(n(T))} \geq  100\left[\log \log(20/\Delta) + \log (2K^2/\delta ) \right]  \bar{H}
%%  \end{equation}
%% Here, 
%% \begin{align}
%%  \label{Hbar}
%%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%%  \end{align}
%%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%%\end{theorem}
%
%\begin{theorem}\label{mainresult}
%(Proved formally as Theorem \ref{thm:detailed}) Let $\Delta= \min \limits_{k \neq k*} \Delta_k$. Let $\sigma^*$ be the effective variance as in Definition \ref{effectivelogdivergence}. The probability that Algorithm \ref{alg:pickbest} identifies the wrong optimal arm ($e(T,B)$) satisfies:
%\begin{equation}
% e(T,B) \leq 2K^2 \log_2 (20/\Delta) \exp \left( - \frac{T}{ 2\bar{H} \overline{\log}(n(T))} \right)
%  \end{equation}
%  when the budget for the total number of samples is $T$ and $\Delta \geq 10/\sqrt{T}$. 
% Here, 
% \begin{align}
%  \label{Hbar}
%  \bar{H} = \max_{k \neq k^*} \log_2(10/\Delta_k)^3  \left(\frac{\sigma^*(B,{\cal R}^*(\Delta_k))}{\Delta_k }\right)^2
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{audibert2010best}:}
%Let $\tilde{{\cal R}}(\Delta_k)= \{s: \Delta_s \leq \Delta_k \}$, i.e. the set of arms which are closer to the optimal than arm $k$. Let $\tilde{H} = \max \limits_{k \neq k*} \frac{\lvert \tilde{{\cal R}}(\Delta_k) \rvert}{\Delta_k^2}$. The result for the best arm identification with no information leakage in \cite{audibert2010best} can be stated as: \textit{The error in finding the optimal arm is bounded as}:
% \begin{equation}\label{noleakage}
%   e(T) \leq O\left(K^2 \exp \left(- \frac{T - K}{\overline{\log}(K)\tilde{H}} \right) \right)
% \end{equation}
%
% One intuitive interpretation for $\tilde{H}$ is that it is the maximum among the number of samples (neglecting some log factors) required to conclude that arm $k$ is suboptimal from among the arms which are closer to the optimal than itself. Intuitively, this is because when there is no information leakage, one requires $1/\Delta_k^2$ samples to distinguish between the $k$-th optimal arm and the optimal arm. Further, the $k$th arm is played only $1/k$ fraction of the times since we do not know the identity of the $k$-th optimal arm. 
%  
%\textbf{Interpretation of our Result:}
%Our main result in Theorem $\ref{mainresult}$ can be seen to be a generalization of the existing result in (\ref{noleakage}) for the case when there is information leakage between the arms (various changes in a causal graph).  
%
%The term $\sigma^*(B,{\cal R}^*(\Delta_k))$ in our setting is the `effective standard deviation' due to information leakage.  There is a similar interpretation of our result (ignoring the log factors): Since there is information leakage, the expression $\frac{(\sigma^*)^2}{(\Delta_k)^2}$ characterizes the number of samples required to weed out arm $k$ out of contention from among competing arms (arms that are at a distance at most twice than that of arm $k$ from the optimal arm). The interpretation of 'effective variance' is justified using importance sampling which is detailed in Section \ref{sec:estimator}. Further, in our framework $\sigma^*$ also incorporates any budget constraint that comes with the problem, i.e. any \textit{apriori} constraint on the relative fraction of times different arms need to be pulled.
%
%\textbf{Improvement over the no-information leakage case:}
%For ease of exposition let $(k)$ denote the index of the $k$-th best arm (for $k = 1,..,K$) and $\Delta_{(k)}$ denotes the corresponding gap. In this setting, the terms $\tilde{H}$ (from the result in~\cite{audibert2010best}) and $\bar{H}$ can be written as:
%\begin{align*}
%\tilde{H} &= \max_{k \neq 1} \frac{k}{\Delta_{(k)}^2} \\
%\bar{H} &= \max_{k \neq 1} \frac{\sigma^*(B,{\cal R}^*(\Delta_{(k)}))^2}{\Delta_{(k)}^2}.
%\end{align*}
%$ \sigma^*(B,{\cal R}^*(\Delta_{(k)}))$ can be smaller than $\sqrt{k}$ due to information leakage as every single arm pull contributes to another arm's estimate. Therefore, these provide better guarantees than ~\cite{audibert2010best}. 
%
%To see the improvement over the previous result in \cite{audibert2010best}, we consider a special case when the cost budget $B$ is infinity and there is only the the sample budget $T$. In addition, let us assume that the log divergences are such that: $M_{ij} \leq \eta M_{ii} = \eta << \sqrt{\lvert {\cal R}  \rvert},~ \forall i \neq j$. Let ${\cal R} = {\cal R}^*(\Delta_{(k)})$. If $\eta > \sqrt{\lvert {\cal R}  \rvert}$, the optimal solution for (\ref{mainLP1}) is a bit complicated to interpret.  Consider the feasible allocation $\nu_i = \frac{1}{\lvert {\cal R}  \rvert}, ~ \forall i \in {\cal R}$ in (\ref{mainLP1}). Evaluating the objective function for this feasible allocation, it is possible to show that $\sigma^* \leq \frac{\eta}{1-1/\lvert {\cal R}  \rvert} <<  \sqrt{\lvert {\cal R}  \rvert}$. Hence, unless the variance due to information leakage is too bad, the effective variance is smaller than that of the case with no information leakage.
%
%The improvement over the no information leakage setting, is even more pronounced under budget constraints. Consider the setting \textbf{S1}, and assume that the fractional budget of the \textit{difficult} arms, $B = o(1)$. This implies that the total number of samples available for difficult arms is $o(T)$. The budget constrained case has not been analyzed in~\cite{audibert2010best}, however in the absence of information leakage, one would expect that the arms with the least number of samples would be the most difficult to eliminate, and therefore the error guarantees would scale as $\exp(-O(BT)/\tilde{H}) \sim \exp(-o(T)/\tilde{H})$ (excluding $\log$ factors). On the other hand, our algorithm can leverage the information leakage and the error guarantee would scale as $\exp(-O(T)/\bar{H})$, which can be order-wise better if the \textit{effective standard deviations} are well-behaved. 
%
%\textbf{Remark:} Although similar advantages can be shown for \cite{lattimore2016causal}, there are no gap dependent bounds in that work and our analysis indicates a gap dependent improvement term by term with respect to \cite{audibert2010best}.
%
%
% \begin{theorem}\label{mainresult2}
%(Proved formally as Theorem \ref{thm:detailed})  Let $v^*$ be the effective inverse log divergence as in Definition \ref{effectivelogdivergence}. The simple regret of Algorithm \ref{alg:pickbest} when the number of samples is $T$ satisfies:
%\ \begin{align}
%\label{eq:SRmain}
%&r(T,B) \leq  \\
%&2K^2\sum_{\substack{k \neq k^*:\\ \Delta_k \geq 10/\sqrt{T} }} \Delta_k \log_2\left(\frac{20}{\Delta_k}\right) \exp \left( - \frac{T}{ 2\bar{H}_{k} \overline{\log}(n(T))} \right) \\ \nonumber
%& + \frac{10}{\sqrt{T}}\mathds{1} \left\{\exists k\neq k^* \text{ s.t } \Delta_k < 10/\sqrt{T} \right\} 
% \end{align}
% Here, 
% \begin{align}
%  \label{HK}
% \bar{H}_{k} = \max_{\{l : \Delta_l \geq \Delta_k\}} \frac{\log_2(10/\Delta_l)^3}{(\Delta_l/10)^2 v^*(B,{\cal R}^*(\Delta_l))^2}
%  \end{align}
%and ${\cal R}^*(\Delta_k) = \{ s: \log_2 \left(\frac{10}{\Delta_s} \right) \geq \lfloor  \log_2 \left(\frac{10}{\Delta_k }\right) \rfloor  \} $ is the set of arms whose distance from the optimal arm is roughly at most twice that of arm $k$.
%\end{theorem}
%
%\textbf{Comparison to the result in \cite{lattimore2016causal}:} In~\cite{lattimore2016causal}, the algorithm is based on clipped importance samples, where the clipper is always set at a static level of $O(\sqrt{T})$ (excluding $\log$ factors). The simple regret guarantee in~\cite{lattimore2016causal} scales as $O(\sqrt{(m(\eta)/T)\log T})$, where $m(\eta)$ is a global hardness parameter. The guarantees do not adapt to the problem parameters, specifically the gaps $\{\Delta_k \}_{k \in [K]}$. 
%
%On the contrary, we provide problem dependent bounds, which differentiates the arms according to its gap from the optimal arm and its \textit{effective standard deviation} parameter. The terms $\bar{H}_{k}$ can be interpreted as the hardness parameter for rejecting arm $k$. Note that $\bar{H}_k$ depends only on the  arms that are at least as \textit{bad} in terms of their gap from the optimal arm. Moreover the guarantees are adapted to our general budget constraints, which is absent in~\cite{lattimore2016causal}. It can be seen that when $\Delta_k$'s do not scale in $T$, then our simple regret is exponentially small in $T$ (dependent on $\bar{H}_k$'s) and can be much less than $O(1/\sqrt{T})$. The guarantee also generalizes to the problem independent setting when $\Delta_k$'s scale as $O(1/\sqrt{T})$. 
%
%We defer the theoretical analysis to Section~\ref{sec:proofs}. In Section~\ref{sec:divergence} we discuss importance sampling with clipped estimators. We demonstrate a novel way to analyze these clipped estimators by relating them to a particular $f$-divergence in Section~\ref{sec:relation}. One of our main results is Theorem~\ref{lem:clippedmain}, that provides concentration guarantees for the clipped estimators by relating the bias of the estimator to certain pairwise $f$-divergences among the candidate distributions  $\{\mathrm{P}_k(V|pa(V))\}$. In Section~\ref{sec:estimator}, we introduce the main estimator used in Algorithm~\ref{alg:pickbest}, and demonstrate how we can seamlessly use the samples from all arms to estimate the mean reward from a particular arm. The confidence bounds for this estimator are provided as Theorem~\ref{thm:uniestimator}.  Finally, in Section~\ref{sec:analysis} we analyze our algorithm, thereby shedding more light on the key design decisions. Theorem~\ref{mainresult} and Theorem~\ref{mainresult2} are subparts of our main technical theorem (Theorem~\ref{thm:detailed}), which is proved in Section~\ref{sec:analysis}. 
%






